Energy-energy correlators within $Z$-tagged jets in proton-proton collisions at $\sqrt{s}$ = 13 TeV

Energy-energy correlators probe perturbative and nonperturbative QCD regimes of jet formation through momentum-weighted angular correlations between hadrons. First measurements in light-quark-enriched jets are presented for inclusive, like-sign, and opposite-sign charged-hadron pairs, using proton-proton collisions at LHCb. The results support universality of the confinement scale for light-quark-initiated jets across collision systems and the reported transverse momentum scale of the jet. In the charge-dependent measurements, opposite-sign correlations are enhanced as angular separation decreases down to the confinement-scale region, a behavior that is well described by simulations.

==> LHCb/Authorship_LHCb-PAPER-20YY-nnn.tex <==
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}




==> LHCbInternal/README-acknowledgements <==
J. Walsh
21-Apr-2023

Unfortunately, I am forced to maintain two different acknowledgements files. This is because the a recent request
to add to it is only valid from 2023 on, but we have many old papers in the pipeline. There is no way to generate 
a time-dependent acknowledgements list, although there is work going on by the FENCE team to implement something. 

For now we have two files:

acknowledgements.tex -- to be used on papers before 2023. 
acknowledgements_2023_01_01.tex -- to be used on papers from 2023 on. 

When modifying the acknowledgments, if it should be retroactive to older papers, then both of these files must
be edited. If it's only for recent papers, then only the 2023 version should be modified. 

MacBook [512]> diff acknowledgements.tex acknowledgements_2023_01_01.tex 
36c36
< EPLANET, Marie Sk\l{}odowska-Curie Actions and ERC (European Union);
---
> EPLANET, Marie Sk\l{}odowska-Curie Actions, ERC and NextGenerationEU (European Union);
44c44
< GVA, XuntaGal and GENCAT (Spain);
---
> GVA, XuntaGal, GENCAT, Inditex and InTalent (Spain);

Note that both of these are "new" in the sense that mention of Russian agencies is removed. The version with the
Russian agencies present still exists: acknowledgements_full.tex. It has not been updated for 2023. 

5-Jun-2023

I'm renaming these two acknowledgements files:

acknowledgements.tex -> acknowledgements_2022.tex
acknolwedgements_2023_01_01.tex -> acknowledgements.tex




==> LHCbInternal/Scripts/trunk/python/LHCbPapers.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% All LHCb papers in one command
% Use as
% \newboolean{articletitles}
% \setboolean{articletitles}{false}
% \input{LHCbPapers}
% 
% \LHCbCitation{LHCb-PAPER-2014-001}
% \LHCbShortCitation{LHCb-PAPER-2014-001}
% 
% optionally (this is the default):
% 
% \LHCbCitation[\tiny\blue]{LHCb-PAPER-2014-001}
% \LHCbShortCitation{LHCb-PAPER-2014-001}
% 
% @author P. Koppenburg
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\DefaultLHCbCitationStyle{\tiny\blue}

\newcommand{\LHCbCitation}[2][\DefaultLHCbCitationStyle]{{%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-050}}{\ifthenelse{\boolean{articletitles}}{``\textsl TBC'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-050}{LHCb-PAPER-2017-050}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-049}}{\ifthenelse{\boolean{articletitles}}{``\textsl Evidence for the rare decay $\Sigma^+ \to p \mu\mu$'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-049}{LHCb-PAPER-2017-049}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-048}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $C\!P$-violating phase $\phi_s^{d\bar{d}}$ in quasi-two-body $B^0_s \to (K^+\pi^-)(K^-\pi^+)$ decays'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-048}{LHCb-PAPER-2017-048}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-047}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $C\!P$ asymmetry in $B^0_s \to D_s^\mp K^\pm$ decays'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-047}{LHCb-PAPER-2017-047}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-046}}{\ifthenelse{\boolean{articletitles}}{``\textsl Updated determination of $D^0$-$\overline{D}^0$ mixing parameters and $C\!P$ violation in $D^0 \to K^+\pi^-$ decays'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-046}{LHCb-PAPER-2017-046}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-045}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the decays of charmed beauty mesons to two charm mesons'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-045}{LHCb-PAPER-2017-045}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-044}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for direct $C\!P$ violation in $\Lc\to p K ^-K^+$ and $\Lc \to p\pi^-\pi^+$ decays using semileptonic $\Lb$ decays'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-044}{LHCb-PAPER-2017-044}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-043}}{\ifthenelse{\boolean{articletitles}}{``\textsl Weakly decaying $b$-flavored pentaquarks in final states containing $J/\psi$ mesons and hadrons'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-043}{LHCb-PAPER-2017-043}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-042}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for excited $B_{c}^{+}$ states'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-042}{LHCb-PAPER-2017-042}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-041}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the relative branching ratio $\mathcal{B}(\Lb \to \psi(2S)\Lz / \mathcal{B}(\Lb \to J/\psi\Lz)$'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-041}{LHCb-PAPER-2017-041}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-040}}{\ifthenelse{\boolean{articletitles}}{``\textsl Studies of the resonance structure in $D^0 \to K^{\mp}\pi^{\pm}\pi^+\pi^-$ decays'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-040}{LHCb-PAPER-2017-040}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-039}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the suppressed $\Lc\to p\mu^+\mu^-$ decay and observation of the $\Lc\to p\omega$ decay'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-039}{LHCb-PAPER-2017-039}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-038}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for dark photons produced in 13 TeV $pp$ collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1710.02867}{submitted to Phys. Rev. Lett, arXiv:1710.02867}, submitted to Phys. Rev. Lett]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-037}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $B^{\pm}$ production cross-section in $pp$ collisions at $\sqrt{s} = 7$ and $13$ TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1710.04921}{submitted to JHEP, arXiv:1710.04921}, submitted to JHEP]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-036}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precise measurement of the $\chi_{c1}$ and $\chi_{c2}$ resonance parameters with the decays $\chi_{c1,c2}\to J/\psi\mu^+\mu^-$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1709.04247}{submitted to Phys. Rev. Lett, arXiv:1709.04247}, submitted to Phys. Rev. Lett]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-035}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of the semitauonic decay $B^+_c\to J/\psi\tau^+\nu_{\tau}$'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-035}{LHCb-PAPER-2017-035}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-034}}{\ifthenelse{\boolean{articletitles}}{``\textsl First measurements of relative branching fractions of charmless four-body $\Lb$ and $\Xi_b^0$ decays'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-034}{LHCb-PAPER-2017-034}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-033}}{\ifthenelse{\boolean{articletitles}}{``\textsl Anatomy of the decay $\Bz\to\KS\pip\pim$ and first observation of $C\!P$ asymmetry in the transition $\Bzb \to\Kstarm (892)\pip$'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-033}{LHCb-PAPER-2017-033}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-032}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of $B^+ \to D_s^+ K^+ K^-$ decays and a search for $B^+ \to D_s^+\phi$ decays'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-032}{LHCb-PAPER-2017-032}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-031}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the lepton-flavour violating decays $B_{(s)}^0\to e^\pm\mu^\mp$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1710.04111}{submitted to JHEP, arXiv:1710.04111}, submitted to JHEP]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-030}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $C\!P$ observables in $B^\pm \to DK^{\ast \pm}$ decays using two- and four-body $D$-meson final states'' }{}#1[LHCb, \href{http://arxiv.org/abs/1709.05855}{submitted to JHEP, arXiv:1709.05855}, submitted to JHEP]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-029}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $C\!P$ violation in $B^0 \to \jpsi(e^+e^-)K_S^0$ and $B^0 \to \psi(2S)(\mu^+\mu^-)K_S^0$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1709.03944}{submitted to JHEP, arXiv:1709.03944}, submitted to JHEP]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-028}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Upsilon$ polarization in $pp$ collisions at $\sqrt{s} = 7$ and $8$ TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1709.01301}{submitted to JHEP, arXiv:1709.01301}, submitted to JHEP]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-027}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\mathcal{B}(B^0 \to D^{\ast-} \tau^+ \nu_{\tau})$ branching fraction using three-prong $\tau$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1711.02505}{submitted to Phys. Rev. D, arXiv:1711.02505}, submitted to Phys. Rev. D]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-026}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of $\Lc \to p K^-K^+$, $\Lc \to p \pi^-\pi^+$ and $\Lc\to p \pi^-K^+$ branching ratios'' }{}#1[LHCb, \href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-026}{LHCb-PAPER-2017-026}, in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-025}}{\ifthenelse{\boolean{articletitles}}{``\textsl Bose-Einstein correlations of same-sign charged pions in the forward region in $pp$ collisions at $\sqrt{s}=7$ TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1709.01769}{submitted to JHEP, arXiv:1709.01769}, submitted to JHEP]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-024}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of forward $Z\to b\bar{b}$ production in $pp$ collisions at $\sqrt{s}=8$ TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1709.03458}{submitted to Phys. Lett. B, arXiv:1709.03458}, submitted to Phys. Lett. B]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-023}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for baryon-number-violating $\Xi_b^0$ oscillations'' }{}#1[LHCb, \href{http://arxiv.org/abs/1708.05808}{Phys. Rev. Lett. 119 (2017) 181807, arXiv:1708.05808}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-022}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the rare purely baryonic decay $B^0\to\proton\antiproton$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1709.01156}{submitted to Phys. Rev. Lett, arXiv:1709.01156}, submitted to Phys. Rev. Lett]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-021}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $C\!P$ observables in $B^\pm \to D^{(\ast)}K^\pm$ and $B^\pm \to D^{(\ast)}\pi^\pm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1708.06370}{submitted to Phys. Lett. B, arXiv:1708.06370}, submitted to Phys. Lett. B]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-020}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $b\bar{b}$ correlations in high energy proton-proton collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1708.05994}{submitted to JHEP, arXiv:1708.05994}, submitted to JHEP]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-019}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $D^0$ meson decays to $\pi^+\pi^-\mu^+\mu^-$ and $K^+K^-\mu^+\mu^-$ final states'' }{}#1[LHCb, \href{http://arxiv.org/abs/1707.08377}{Phys. Rev. Lett. 119 (2017) 181805, arXiv:1707.08377}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the doubly charmed baryon $\Xi_{cc}^{++}$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1707.01621}{Phys. Rev. Lett. 119 (2017) 112001, arXiv:1707.01621}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the ratio of the $\mathcal{B}(B^0 \to D^{\ast-} \tau^+ \nu_{\tau})$ and \hbox{$\mathcal{B}(B^0\to D^{\ast-}\mu^+\nu_{\mu})$} branching fractions using three-prong $\tau$-lepton decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1708.08856}{submitted to Phys. Rev. Lett, arXiv:1708.08856}, submitted to Phys. Rev. Lett]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the shape of the $\Lb\to\Lc\mu^{-}\overline{\nu}_{\mu}$ differential decay rate'' }{}#1[LHCb, \href{http://arxiv.org/abs/1709.01920}{submitted to Phys. Rev. D, arXiv:1709.01920}, submitted to Phys. Rev. D]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of prompt $D^0$ meson production in $p$Pb collisions at $\sqrt{s_{NN}} = 5$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1707.02750}{submitted to JHEP, arXiv:1707.02750}, submitted to JHEP]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl Prompt and nonprompt \jpsi\ production and nuclear modification in $p$Pb collisions at $\sqrt{s_{NN}} = 8.16$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1706.07122}{submitted to Phys. Lett. B, arXiv:1706.07122}, submitted to Phys. Lett. B]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl Test of lepton universality with $B^0\to K^{*0} \ell^+ \ell^-$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1705.05802}{JHEP 08 (2017) 055, arXiv:1705.05802}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of a baryonic $B^0_s$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1704.07908}{Phys. Rev. Lett. 119 (2017) 041802, arXiv:1704.07908}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decays $\Lb\to\chicone\proton\Km$ and $\Lb\to\chictwo\proton\Km$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1704.07900}{Phys. Rev. Lett. 119 (2017) 062001, arXiv:1704.07900}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl Updated branching fraction measurements of $B^0_{(s)} \to K^0_S h^+ h^{\prime-}$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1707.01665}{submitted to JHEP, arXiv:1707.01665}, submitted to JHEP]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl Improved limit on the branching fraction of the rare decay $\KS\to\muon\muon$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1706.00758}{Eur. Phys. J. C77 (2017) 678, arXiv:1706.00758}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl Resonances and $C\!P$-violation in $\Bsb$ and $\Bs\to\jpsi\Kp\Km$ decays in the mass region above the $\phiz(1020)$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1704.08217}{JHEP 08 (2017) 037, arXiv:1704.08217}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of charmonium production in $b$-hadron decays and first evidence for the decay $B^0_s \to \phi\phi\phi$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1706.07013}{submitted to Eur. Phys. J., arXiv:1706.07013}, submitted to Eur. Phys. J.]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the $\Bp\to\Dstarm\Kp\pip$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1704.07581}{Phys. Rev. D96 (2017) 011101, arXiv:1704.07581}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of charmless baryonic decays $B^0_{(s)}\to\proton\antiproton\hadron^+\hadron^{\prime -}$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1704.08497}{Phys. Rev. D96 (2017) 051103, arXiv:1704.08497}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\Bs$ and $\Dsm$ meson lifetimes'' }{}#1[LHCb, \href{http://arxiv.org/abs/1705.03475}{Phys. Rev. Lett. 119 (2017) 101801, arXiv:1705.03475}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the decays $\Bs\to\taup\taum$ and $\Bz\to\taup\taum$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1703.02508}{Phys. Rev. Lett. 118 (2017) 251802, arXiv:1703.02508}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of five new narrow $\Omegac$ states decaying to $\Xicp\Km$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1703.04639}{Phys. Rev. Lett. 118 (2017) 182001, arXiv:1703.04639}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bs\to \mup\mun$ branching fraction and effective lifetime and search for $\Bd\to\mup\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1703.05747}{Phys. Rev. Lett. 118 (2017) 191801, arXiv:1703.05747}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-065}}{\ifthenelse{\boolean{articletitles}}{``\textsl Updated search for long-lived particles decaying to jet pairs'' }{}#1[LHCb, \href{http://arxiv.org/abs/1705.07332}{submitted to EPJC, arXiv:1705.07332}, submitted to EPJC]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-064}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of \jpsi\ production in jets'' }{}#1[LHCb, \href{http://arxiv.org/abs/1701.05116}{Phys. Rev. Lett. 118 (2017) 192001, arXiv:1701.05116}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-063}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the \CP\ violation parameter $A_\Gamma$ in $\Dz\to\Kp\Km$ and $\Dz\to\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1702.06490}{Phys. Rev. Lett. 118 (2017) 261803, arXiv:1702.06490}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-062}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of \Bd, \Bs, \Bp and \Lb\ production asymmetries in $7$ and $8$\tev\ \proton\proton\ collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1703.08464}{submitted to Phys. Lett. B, arXiv:1703.08464}, submitted to Phys. Lett. B]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-061}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of the $\Dz\proton$ amplitude in $\Lb\to\Dz\proton\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1701.07873}{JHEP 05 (2017) 030, arXiv:1701.07873}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-060}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the $\Bs\to\etapr\phiz$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.08110}{JHEP 05 (2017) 158, arXiv:1612.08110}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-059}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decay $\Lb\to\proton\Km\mup\mun$ a search for \CP\ violation'' }{}#1[LHCb, \href{http://arxiv.org/abs/1703.00256}{JHEP 06 (2017) 108, arXiv:1703.00256}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-058}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bc\to\Dz\Kp$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1701.01856}{Phys. Rev. Lett. 118 (2017) 111803, arXiv:1701.01856}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-057}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the \jpsi\ pair production cross-section in $\proton\proton$ collisions at $\sqrt{s}=13$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.07451}{JHEP 06 (2017) 047, arXiv:1612.07451}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-056}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decay $\Bs\to\etac\phiz$ and evidence for $\Bs\to\etac\pip\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1702.08048}{JHEP 07 (2017) 21, arXiv:1702.08048}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-055}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bc\to\jpsi D^{(\ast)} K^{(\ast)}$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.07421}{Phys. Rev. D95 (2017) 032005, arXiv:1612.07421}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-054}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $B^\pm$ production asymmetry and the $C\!P$ asymmetry in $B^\pm\to \jpsi K^\pm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1701.05501}{Phys. Rev. D95 (2017) 052005, arXiv:1701.05501}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-053}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the $\Xibm\to\jpsi\Lz\Km$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1701.05274}{Phys. Lett. B772 (2017) 265, arXiv:1701.05274}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-052}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for long-lived scalar particles in $\Bp\to\Kp\chi(\mumu)$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.07818}{Phys. Rev. D95 (2017) 071101, arXiv:1612.07818}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-051}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the branching fraction ratio and \CP\ asymmetry difference of the decays $\Bp\to\jpsi\pip$ and $\Bp\to\jpsi\Kp$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.06116}{JHEP 03 (2017) 036, arXiv:1612.06116}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-050}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decay $\Xibm\to\proton\Km\Km$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.02244}{Phys. Rev. Lett. 118 (2017) 071801, arXiv:1612.02244}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-049}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the suppressed decay $\Lb\to\proton\pim\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1701.08705}{JHEP 04 (2017) 029, arXiv:1701.08705}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-048}}{\ifthenelse{\boolean{articletitles}}{``\textsl Evidence for the two-body charmless baryonic decay $\Bp\to p\Lbar$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1611.07805}{JHEP 04 (2017) 162, arXiv:1611.07805}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-047}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for massive long-lived particles decaying semileptonically in the LHCb detector'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.00945}{Eur. Phys. J. C77 (2017) 224, arXiv:1612.00945}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-046}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the $\CP$-violating strong decays $\eta\to\pip\pim$ and $\etapr(958)\to \pip\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1610.03666}{Phys. Lett. B764 (2016) 233, arXiv:1610.03666}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-045}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the phase difference between the short- and long-distance amplitudes in the $\Bp\to\Kp\mup\mun$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.06764}{Eur. Phys. J. C77 (2017) 161, arXiv:1612.06764}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-044}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for \CP violation in the phase space of $\Dz\to \pip\pim\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.03207}{Phys. Lett. B769 (2017) 345, arXiv:1612.03207}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-043}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for decays of neutral beauty mesons into four muons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1611.07704}{JHEP 03 (2017) 001, arXiv:1611.07704}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-042}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of prompt charm production cross-sections in $\proton\proton$ collisions at $\sqrt{s} = 5$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1610.02230}{JHEP 06 (2017) 147, arXiv:1610.02230}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-041}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of \CP\ asymmetries in $\Dpm \to \etapr\pipm$ and $\Dspm \to\etapr\pipm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1701.01871}{Phys. Lett. B771 (2017) 21, arXiv:1701.01871}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-040}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bp \to\jpsi 3\pip 2\pim$ and $\Bp \to \psitwos \pip\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1610.01383}{Eur. Phys. J. C77 (2016) 72, arXiv:1610.01383}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-039}}{\ifthenelse{\boolean{articletitles}}{``\textsl New algorithms for identifying the flavour of $\Bz$ mesons using pions and protons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1610.06019}{Eur. Phys. J. C77 (2017) 238, arXiv:1610.06019}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-038}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\ttbar$, $W + \bbbar$ and $W + \ccbar$ production cross sections in $\proton\proton$ collisions at $\sqrt{s}=8$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1610.08142}{Phys. Lett. B767 (2017) 110, arXiv:1610.08142}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-037}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of \CP\ violation in $\B \to \Dp\Dm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1608.06620}{Phys. Rev. Lett. 117 (2016) 261801, arXiv:1608.06620}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-036}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the annihilation decay mode $\Bz \to \Kp\Km$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1610.08288}{Phys. Rev. Lett. 118 (2017) 081801, arXiv:1610.08288}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-035}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of \CP\ asymmetry in $\Dz\to\Kp\Km$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1610.09476}{Phys. Lett. B767 (2017) 177, arXiv:1610.09476}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-034}}{\ifthenelse{\boolean{articletitles}}{``\textsl First experimental study of photon polarization in radiative $\Bs$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1609.02032}{Phys. Rev. Lett. 118 (2017) 021801, arXiv:1609.02032}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-033}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of charm mixing and \CP\ violation using $\Dz\to\Kpm\pimp$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1611.06143}{Phys. Rev. D95 (2017) 052004, arXiv:1611.06143}, Erratum in preparation]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-032}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the CKM angle $\gamma$ from a combination of LHCb results'' }{}#1[LHCb, \href{http://arxiv.org/abs/1611.03076}{JHEP 12 (2016) 087, arXiv:1611.03076}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-031}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\bquark$-quark production cross-section in 7 and 13\,TeV $\proton\proton$ collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1612.05140}{Phys. Rev. Lett. 118 (2017) 052002, arXiv:1612.05140}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-030}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of matter-antimatter differences in beauty baryon decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1609.05216}{Nature Physics 13 (2017) 391, arXiv:1609.05216}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-029}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for structure in the $\Bs\pipm$ invariant mass spectrum'' }{}#1[LHCb, \href{http://arxiv.org/abs/1608.00435}{Phys. Rev. Lett. 117 (2016) 152003, arXiv:1608.00435}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-028}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decays $\Bs\to\phiz\pip\pim$ and $\Bd\to\phiz\pip\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1610.05187}{Phys. Rev. D95 (2017) 012006, arXiv:1610.05187}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-027}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$ violating phase and decay-width difference in $\Bs \to \psitwos\phi$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1608.04855}{Phys. Lett. B762 (2016) 253, arXiv:1608.04855}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-026}}{\ifthenelse{\boolean{articletitles}}{``\textsl Amplitude analysis of $\Bm \to \Dp \pim \pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1608.01289}{Phys. Rev. D94 (2016) 072001, arXiv:1608.01289}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-025}}{\ifthenelse{\boolean{articletitles}}{``\textsl Differential branching fraction and angular analysis of the decay $Bz\to \Kp\pim\mup\mun$ in the $K^{*}_{0,2}(1430)^0$ region'' }{}#1[LHCb, \href{http://arxiv.org/abs/1609.04736}{JHEP 12 (2016) 065, arXiv:1609.04736}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-024}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of forward $\W\to\electron\neu$ production in $\proton\proton$ collisions at $\sqrt{s}=8$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1608.01484}{JHEP 10 (2016) 030, arXiv:1608.01484}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-023}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the suppressed decays $\Bp \to \Kp\Kp\pim$ and $Bp\to \pip\pip\Km$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1608.01478}{Phys. Lett. B765 (2017) 307, arXiv:1608.01478}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-022}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $\Bcp$ decays to the $\Kp\Km\pip$ final state and evidence for the decay $\Bcp\to\chiczero\pip$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1607.06134}{Phys. Rev. D94 (2016) 091102(R), arXiv:1607.06134}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-021}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the forward $\Z$ boson production cross-section in $\proton\proton$ collisions at $\sqrt{s}=13$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1607.06495}{JHEP 09 (2016) 136, arXiv:1607.06495}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-020}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the ratio of branching fractions $\BF(\Bcp\to\jpsi\Kp)/\BF(\Bcp\to \jpsi\pip)$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1607.06823}{JHEP 09 (2016) 153, arXiv:1607.06823}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-019}}{\ifthenelse{\boolean{articletitles}}{``\textsl Amplitude analysis of $\Bp\to \jpsi\phi\Kp$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1606.07898}{Phys. Rev. D95 (2016) 012002, arXiv:1606.07898}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of exotic $\jpsi\phi$ structures from amplitude analysis of $\Bp \to \jpsi\phi\Kp$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1606.07895}{Phys. Rev. Lett. 118 (2016) 022003, arXiv:1606.07895}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bs \to \jpsi\eta$ lifetime'' }{}#1[LHCb, \href{http://arxiv.org/abs/1607.06314}{Phys. Lett. B762 (2016) 484, arXiv:1607.06314}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\etac(2S)\to \proton\antiproton$ and search for $X(3872) \to\proton\antiproton$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1607.06446}{Phys. Lett. B769 (2017) 305, arXiv:1607.06446}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl Evidence for exotic hadron contributions to $\Lb \to \jpsi\proton\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1606.06999}{Phys. Rev. Lett. 117 (2016) 082003, arXiv:1606.06999}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for Higgs-like boson decaying into pair of long-lived particles'' }{}#1[LHCb, \href{http://arxiv.org/abs/1609.03124}{Eur. Phys. J. C76 (2016) 664, arXiv:1609.03124}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$ asymmetry in $\Bs$--$\Bsb$ mixing'' }{}#1[LHCb, \href{http://arxiv.org/abs/1605.09768}{Phys. Rev. Lett. 117 (2016) 061803, arXiv:1605.09768}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the S-wave fraction in $\Bz\to\Kp\pim\mup\mun$ decays and the $\Bz\to \Kstar(892)^0\mup\mun$ differential branching fraction'' }{}#1[LHCb, \href{http://arxiv.org/abs/1606.04731}{JHEP 11 (2016) 047, arXiv:1606.04731}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of forward $\W\!$ and $\Z$ boson production in association with jets in proton-proton collisions at $\sqrt{s}=8$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1605.00951}{JHEP 05 (2016) 131, arXiv:1605.00951}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the properties of the $\Xi_b^{\ast 0}$ baryon'' }{}#1[LHCb, \href{http://arxiv.org/abs/1604.03896}{JHEP 05 (2016) 161, arXiv:1604.03896}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl Model-independent evidence for $\jpsi\proton$ contributions to $\Lb\to \jpsi\proton\Km$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1604.05708}{Phys. Rev. Lett. 117 (2016) 082002, arXiv:1604.05708}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of the mass and lifetime of the $\Omegab$ baryon'' }{}#1[LHCb, \href{http://arxiv.org/abs/1604.01412}{Phys. Rev. D93 (2016) 092007, arXiv:1604.01412}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the CKM angle $\gamma$ using $\Bz \to \D\Kstarz$ with $\D\to\KS\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1605.01082}{JHEP 08 (2016) 137, arXiv:1605.01082}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl Model-independent measurement of the CKM angle $\gamma$ using $\Bz \to \D\Kstarz$ decays with $\D\to\KS\pip\pim$ and $\KS\Kp\Km$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1604.01525}{JHEP 06 (2016) 131, arXiv:1604.01525}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for violations of Lorentz invariance and $CPT$ symmetry in $B^0_{(s)}$ mixing'' }{}#1[LHCb, \href{http://arxiv.org/abs/1603.04804}{Phys. Rev. Lett. 116 (2016) 241601, arXiv:1603.04804}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observations of $\Lb\to\Lz\Kp\pim$ and $\Lb\to\Lz\Kp\Km$ decays and searches for other $\Lb$ and $\Xibz$ decays to $\Lz h^+h^-$ final states'' }{}#1[LHCb, \href{http://arxiv.org/abs/1603.00413}{JHEP 05 (2016) 081, arXiv:1603.00413}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ observables in $\Bpm\to\D \Kpm$ and $\Bpm\to\D\pipm$ with two- and four-body $\D$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1603.08993}{Phys. Lett. B760 (2016) 117, arXiv:1603.08993}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the $\Lb\to\Lz\phi$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1603.02870}{Phys. Lett. B759 (2016) 282, arXiv:1603.02870}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for $\Bcp$ decays to the $\proton\antiproton\pip$ final state'' }{}#1[LHCb, \href{http://arxiv.org/abs/1603.07037}{Phys. Lett. B759 (2016) 313, arXiv:1603.07037}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-060}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Lb\to\psitwos\proton\Km$ and $\Lb\to\jpsi\pip\pim\proton\Km$ decays and a measurement of the $\Lb$ baryon mass'' }{}#1[LHCb, \href{http://arxiv.org/abs/1603.06961}{JHEP 05 (2016) 132, arXiv:1603.06961}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-059}}{\ifthenelse{\boolean{articletitles}}{``\textsl Constraints on the unitarity triangle angle $\gamma$ from Dalitz plot analysis of $\Bz\to\D\Kp\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1602.03455}{Phys. Rev. D93 (2016) 112018, arXiv:1602.03455}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-058}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $\psitwos$ production cross-sections and cold nuclear matter effects in $p$Pb collisions at $\sqrt{s_{NN}} = 5$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1601.07878}{JHEP 03 (2016) 133, arXiv:1601.07878}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-057}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of $\Dz-\Dzb$ oscillations in $\Dz\to\Kp\pip\pim\pim$ decays and a measurement of the associated coherence parameters'' }{}#1[LHCb, \href{http://arxiv.org/abs/1602.07224}{Phys. Rev. Lett. 116 (2016) 241801, arXiv:1602.07224}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-056}}{\ifthenelse{\boolean{articletitles}}{``\textsl A new algorithm for identifying the flavour of $\Bs$ mesons at LHCb'' }{}#1[LHCb, \href{http://arxiv.org/abs/1602.07252}{JINST 11 (2016) P05010, arXiv:1602.07252}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-055}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the difference of time-integrated $\CP$ asymmetries in $\Dz\to\Km\Kp$ and $\Dz\to\pim\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1602.03160}{Phys. Rev. Lett. 116 (2016) 191601, arXiv:1602.03160}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-054}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the rare $\Bp\to\Dp\Kp\pim$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1512.02494}{Phys. Rev. D93 (2016) 051101(R), arXiv:1512.02494}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-053}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bs\to D_s^{(*)+}D_s^{(*)-}$ branching fractions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1602.07543}{Phys. Rev. D93 (2016) 092008, arXiv:1602.07543}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-052}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $D_{sJ}^+$ mesons decaying to $\Dstarp\KS$ and $\Dstarz\Kp$ final states'' }{}#1[LHCb, \href{http://arxiv.org/abs/1601.01495}{JHEP 02 (2016) 133, arXiv:1601.01495}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-051}}{\ifthenelse{\boolean{articletitles}}{``\textsl Angular analysis of the $\Bz\to\Kstarz\mup\mun$ decay using $3\invfb$ of integrated luminosity'' }{}#1[LHCb, \href{http://arxiv.org/abs/1512.04442}{JHEP 02 (2016) 104, arXiv:1512.04442}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-050}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bs\to\Dzb\KS$ and evidence for $\Bs \to\Dstarzb\KS$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1603.02408}{Phys. Rev. Lett. 116 (2016) 161802, arXiv:1603.02408}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-049}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of forward $\W\!$ and $\Z$ boson production in $\proton\proton$ collisions at $\sqrt{s}=8$\,TeV '' }{}#1[LHCb, \href{http://arxiv.org/abs/1511.08039}{JHEP 01 (2016) 155, arXiv:1511.08039}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-048}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the lepton-flavour violating decay $\Dz\to\epm\mu^\mp$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1512.00322}{Phys. Lett. B754 (2016) 167, arXiv:1512.00322}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-047}}{\ifthenelse{\boolean{articletitles}}{``\textsl Evidence for the strangeness-changing weak decay $\Xibm\to\Lb\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1510.03829}{Phys. Rev. Lett. 115 (2015) 241801, arXiv:1510.03829}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-046}}{\ifthenelse{\boolean{articletitles}}{``\textsl Production of associated $\Upsilon$ and open charm hadrons in $\proton\proton$ collisions at $\sqrt{s} = 7$ and $8$\,TeV via double parton scattering'' }{}#1[LHCb, \href{http://arxiv.org/abs/1510.05949}{JHEP 07 (2016) 052, arXiv:1510.05949}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-045}}{\ifthenelse{\boolean{articletitles}}{``\textsl Forward production of $\Upsilon$ mesons in $\proton\proton$ collisions at $\sqrt{s}=7$ and $8$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1509.02372}{JHEP 11 (2015) 103, arXiv:1509.02372}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-044}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the decays $\Bz\to\jpsi\gamma$ and $\Bs\to\jpsi\gamma$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1510.04866}{Phys. Rev. D92 (2015) 112002, arXiv:1510.04866}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-043}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decay $\Dz\to\Km\pip\mup\mun$ in the $\rhoz-\omegaz$ region of the dimuon mass spectrum'' }{}#1[LHCb, \href{http://arxiv.org/abs/1510.08367}{Phys. Lett. B757 (2016) 558, arXiv:1510.08367}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-042}}{\ifthenelse{\boolean{articletitles}}{``\textsl Model-independent measurement of mixing parameters in $\Dz\to\KS\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1510.01664}{JHEP 04 (2016) 033, arXiv:1510.01664}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-041}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of prompt charm production cross-sections in $\proton\proton$ collisions at $\sqrt{s} = 13$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1510.01707}{JHEP 03 (2016) 159, arXiv:1510.01707}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-040}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of two-particle correlations in proton-ion collisions at $\sqrt{s_{NN}} = 5$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1512.00439}{Phys. Lett. B762 (2016) 473, arXiv:1512.00439}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-039}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the forward-backward asymmetry in $Z/\gamma^\ast\to\mup\mun$ decays and determination of the effective weak mixing angle'' }{}#1[LHCb, \href{http://arxiv.org/abs/1509.07645}{JHEP 11 (2015) 190, arXiv:1509.07645}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-038}}{\ifthenelse{\boolean{articletitles}}{``\textsl Model-independent confirmation of the $Z(4430)^-$ state'' }{}#1[LHCb, \href{http://arxiv.org/abs/1510.01951}{Phys. Rev. D92 (2015) 112009, arXiv:1510.01951}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-037}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of forward $\jpsi$ production cross-sections in $\proton\proton$ collisions at $\sqrt{s}=13$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1509.00771}{JHEP 10 (2015) 172, arXiv:1509.00771}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-036}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for hidden-sector bosons in $\Bz\to\Kstarz\mup\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1508.04094}{Phys. Rev. Lett. 115 (2015) 161802, arXiv:1508.04094}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-035}}{\ifthenelse{\boolean{articletitles}}{``\textsl First measurement of the differential branching fraction and $\CP$ asymmetry of the $\Bp\to\pip\mup\mun$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1509.00414}{JHEP 10 (2015) 034, arXiv:1509.00414}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-034}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ violation parameters and polarisation fractions in $\Bs\to\jpsi\Kstarzb$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1509.00400}{JHEP 11 (2015) 082, arXiv:1509.00400}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-033}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the $\Bs\to\jpsi\phi\phi$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1601.05284}{JHEP 03 (2016) 040, arXiv:1601.05284}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-032}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of the productions of $\Lb$ and $\Bzb$ hadrons in $\proton\proton$ collisions and first measurement of the $\Lb\to\jpsi\proton\Km$ branching fraction'' }{}#1[LHCb, \href{http://arxiv.org/abs/1509.00292}{Chin. Phys. C 40 (2016) 011001, arXiv:1509.00292}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-031}}{\ifthenelse{\boolean{articletitles}}{``\textsl A precise measurement of the $\Bz$ meson oscillation frequency'' }{}#1[LHCb, \href{http://arxiv.org/abs/1604.03475}{Eur. Phys. J. C76 (2016) 412, arXiv:1604.03475}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-030}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the time-integrated $\CP$ asymmetry in $\Dz\to\KS\KS$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1508.06087}{JHEP 10 (2015) 055, arXiv:1508.06087}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-029}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\jpsi\proton$ resonances consistent with pentaquark states in $\Lb\to\jpsi\proton\Km$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1507.03414}{Phys. Rev. Lett. 115 (2015) 072001, arXiv:1507.03414}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-028}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bs\to\phi\phi$ branching fraction and search for the decay $\Bz\to\phi\phi$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1508.00788}{JHEP 10 (2015) 053, arXiv:1508.00788}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-027}}{\ifthenelse{\boolean{articletitles}}{``\textsl $\B$ flavour tagging using charm decays at the LHCb experiment'' }{}#1[LHCb, \href{http://arxiv.org/abs/1507.07892}{JINST 10 (2015) P10005, arXiv:1507.07892}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-026}}{\ifthenelse{\boolean{articletitles}}{``\textsl Studies of the resonance structure in $\Dz\to\KS\Kpm\pimp$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1509.06628}{Phys. Rev. D93 (2016) 052018, arXiv:1509.06628}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-025}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the ratio of branching fractions $\BF(\Bzb\to\Dstarp\taum\neutb)/\BF(\Bzb\to\Dstarp\mun\neumb)$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1506.08614}{Phys. Rev. Lett. 115 (2015) 111803, arXiv:1506.08614}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-024}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the branching fraction ratio $\BF(\Bcp\to\psitwos\pip)/\BF(\Bcp\to\jpsi\pip)$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1507.03516}{Phys. Rev. D92 (2015) 057007, arXiv:1507.03516}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-023}}{\ifthenelse{\boolean{articletitles}}{``\textsl Angular analysis and differential branching fraction of the decay $\Bs\to\phi\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1506.08777}{JHEP 09 (2015) 179, arXiv:1506.08777}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-022}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of top quark production in the forward region'' }{}#1[LHCb, \href{http://arxiv.org/abs/1506.00903}{Phys. Rev. Lett. 115 (2015) 112001, arXiv:1506.00903}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-021}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $\W\!$ boson production in association with beauty and charm'' }{}#1[LHCb, \href{http://arxiv.org/abs/1505.04051}{Phys. Rev. D92 (2015) 052012, arXiv:1505.04051}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-020}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $\Bm\to\D\Km\pip\pim$ and $\Bm\to\D\pim\pip\pim$ decays and determination of the CKM angle $\gamma$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1505.07044}{Phys. Rev. D92 (2015) 112005, arXiv:1505.07044}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-019}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the $\Lb\to\Lz\etaz$ and $\Lb\to\Lz\etapr$ decays with the LHCb detector'' }{}#1[LHCb, \href{http://arxiv.org/abs/1505.03295}{JHEP 09 (2015) 006, arXiv:1505.03295}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decay $\Bs\to\KS\Kstar(892)^0$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1506.08634}{JHEP 01 (2016) 012, arXiv:1506.08634}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl Amplitude analysis of $\Bz\to\Dzb\Kp\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1505.01505}{Phys. Rev. D92 (2015) 012012, arXiv:1505.01505}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl Identification of beauty and charm quark jets at LHCb'' }{}#1[LHCb, \href{http://arxiv.org/abs/1504.07670}{JINST 10 (2015) P06013, arXiv:1504.07670}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl Quantum numbers of the $X(3872)$ state and orbital angular momentum in its $\rhoz\jpsi$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1504.06339}{Phys. Rev. D92 (2015) 011102(R), arXiv:1504.06339}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl A study of $\CP$ violation in $\Bmp\to\D h^\mp$ $(h=K,\pi)$ with the modes $\D\to\Kmp\pipm\piz$, $\D\to\pip\pim\piz$ and $\D\to\Kp\Km\piz$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1504.05442}{Phys. Rev. D91 (2015) 112014, arXiv:1504.05442}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl Determination of the quark coupling strength $|\Vub|$ using baryonic decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1504.01568}{Nature Physics 11 (2015) 743, arXiv:1504.01568}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the decay $\Bs\to\Dzb f_0(980)$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1505.01654}{JHEP 08 (2015) 005, arXiv:1505.01654}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the exclusive $\Upsilon(nS)$ production cross-section in $\proton\proton$ collisions at $\sqrt{s}=7$\tev and $8$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1505.08139}{JHEP 09 (2015) 084, arXiv:1505.08139}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decay $\Bsb\to\psitwos\Kp\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.07112}{Phys. Lett. B747 (2015) 484, arXiv:1503.07112}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl Differential branching fraction and angular anaysis of $\Lb\to\Lz\mup\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.07138}{JHEP 06 (2015) 115, arXiv:1503.07138}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation and measurement of the branching fraction for the decay $\Bs\to\Dssmp\Kpm$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.09086}{JHEP 06 (2015) 130, arXiv:1503.09086}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation and amplitude analysis of the $\Bm\to\Dp\Km\pim$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.02995}{Phys. Rev. D91 (2015) 092002, arXiv:1503.02995}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the $\Bz\to\rhoz\rhoz$ decay from an amplitude analysis of $\Bz\to(\pip\pim)(\pip\pim)$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.07770}{Phys. Lett. B747 (2015) 468, arXiv:1503.07770}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the time-dependent $\CP$ asymmetries in $\Bs\to\jpsi\KS$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.07055}{JHEP 06 (2015) 131, arXiv:1503.07055}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ violation in $\Bz\to\jpsi\KS$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.07089}{Phys. Rev. Lett. 115 (2015) 031601, arXiv:1503.07089}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\Z\to\epem$ production at $\sqrt{s}=8$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.00963}{JHEP 05 (2015) 109, arXiv:1503.00963}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for long-lived heavy charged particles using a ring-imaging Cherenkov technique at LHCb'' }{}#1[LHCb, \href{http://arxiv.org/abs/1506.09173}{Eur. Phys. J. C75 (2015) 595, arXiv:1506.09173}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the forward $\Z$ boson cross-section in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1505.07024}{JHEP 08 (2015) 039, arXiv:1505.07024}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-070}}{\ifthenelse{\boolean{articletitles}}{``\textsl Dalitz plot analysis of $\Bz\to\Dzb\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1505.01710}{Phys. Rev. D92 (2015) 032002, arXiv:1505.01710}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-069}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of indirect $\CP$ asymmetries in $\Dz\to\Km\Kp$ and $\Dz\to\pim\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1501.06777}{JHEP 04 (2015) 043, arXiv:1501.06777}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-068}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ asymmetries and polarisation fractions in $\Bs\to\Kstarz\Kstarzb$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.05362}{JHEP 07 (2015) 166, arXiv:1503.05362}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-067}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precise measurements of the properties of the $B_1(5721)^{0,+}$ and $B^*_2(5747)^{0,+}$ states and observation of structure at higher invariant mass in the $\Bp\pim$ and $\Bz\pip$ spectra'' }{}#1[LHCb, \href{http://arxiv.org/abs/1502.02638}{JHEP 04 (2015) 024, arXiv:1502.02638}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-066}}{\ifthenelse{\boolean{articletitles}}{``\textsl Angular analysis of the $\Bz\to\Kstar\epem$ decay in the low-$q^2$ region'' }{}#1[LHCb, \href{http://arxiv.org/abs/1501.03038}{JHEP 04 (2015) 064, arXiv:1501.03038}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-065}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the $\Bs\to\etapr\etapr$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1503.07483}{Phys. Rev. Lett. 115 (2015) 051801, arXiv:1503.07483}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-064}}{\ifthenelse{\boolean{articletitles}}{``\textsl Determination of the branching fractions of $\Bs\to\Dsmp\Kpm$ and $\Bz\to\Dsm\Kp$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1412.7654}{JHEP 02 (2015) 029, arXiv:1412.7654}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-063}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of the rare $\Bs$ and $\Bz$ decays into the $\pip\pim\mup\mun$ final state'' }{}#1[LHCb, \href{http://arxiv.org/abs/1412.6433}{Phys. Lett. B743 (2015) 46, arXiv:1412.6433}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-062}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for long-lived particles decaying to jet pairs'' }{}#1[LHCb, \href{http://arxiv.org/abs/1412.3021}{Eur. Phys. J. C75 (2015) 152, arXiv:1412.3021}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-061}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of two new $\Xibm$ baryon resonances'' }{}#1[LHCb, \href{http://arxiv.org/abs/1411.4849}{Phys. Rev. Lett. 114 (2015) 062004, arXiv:1411.4849}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-060}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the lifetime of the $\Bcp$ meson using the $\Bcp\to\jpsi\pip$ decay mode'' }{}#1[LHCb, \href{http://arxiv.org/abs/1411.6899}{Phys. Lett. B742 (2015) 29, arXiv:1411.6899}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-059}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precision measurement of $\CP$ violation in $\Bs\to\jpsi\Kp\Km$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1411.3104}{Phys. Rev. Lett. 114 (2015) 041801, arXiv:1411.3104}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-058}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$-violating phase $\beta$ in $\Bzb\to\jpsi\pip\pim$ decays and limits on penguin effects'' }{}#1[LHCb, \href{http://arxiv.org/abs/1411.1634}{Phys. Lett. B742 (2015) 38, arXiv:1411.1634}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-057}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the inelastic $\proton\proton$ cross-section at a centre-of-mass energy of $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1412.2500}{JHEP 02 (2015) 029, arXiv:1412.2500}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-056}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $\etaz$--$\etapr$ mixing from measurement of $B^0_{(s)} \to\jpsi\eta^{(\prime)}$ decay rates'' }{}#1[LHCb, \href{http://arxiv.org/abs/1411.0943}{JHEP 01 (2015) 024, arXiv:1411.0943}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-055}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Z+\bquark$-jet cross-section in $\proton\proton$ collisions at $\sqrt{s}=7$\tev in the forward region'' }{}#1[LHCb, \href{http://arxiv.org/abs/1411.1264}{JHEP 01 (2015) 064, arXiv:1411.1264}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-054}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for $\CP$ violation in $\Dz\to\pim\pip\piz$ decays with the energy test'' }{}#1[LHCb, \href{http://arxiv.org/abs/1410.4170}{Phys. Lett. B740 (2015) 158, arXiv:1410.4170}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-053}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the semileptonic $\CP$ asymmetry in $\Bz$--$\Bzb$ mixing'' }{}#1[LHCb, \href{http://arxiv.org/abs/1409.8586}{Phys. Rev. Lett. 114 (2015) 041601, arXiv:1409.8586}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-052}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the lepton flavour violating decay $\taum\to\mun\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1409.8548}{JHEP 02 (2015) 121, arXiv:1409.8548}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-051}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$-violating phase $\phis$ in $\Bsb\to \Dsp\Dsm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1409.4619}{Phys. Rev. Lett. 113 (2014) 211801, arXiv:1409.4619}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-050}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\Bcp$ production in proton-proton collisions at $\sqrt{s}=8$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1411.2943}{Phys. Rev. Lett. 114 (2015) 132001, arXiv:1411.2943}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-049}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the rare $\Bs\to\mup\mun$ decay from the combined analysis of CMS and LHCb data'' }{}#1[CMS and LHCb, \href{http://arxiv.org/abs/1411.4413}{Nature 522 (2015) 68, arXiv:1411.4413}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-048}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precision measurement of the mass and lifetime of the $\Xibm$ baryon'' }{}#1[LHCb, \href{http://arxiv.org/abs/1409.8568}{Phys. Rev. Lett. 113 (2014) 242002, arXiv:1409.8568}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-047}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precision luminosity measurements at LHCb'' }{}#1[LHCb, \href{http://arxiv.org/abs/1410.0149}{JINST 9 (2014) P12005, arXiv:1410.0149}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-046}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for $\CP$ violation using $T$-odd correlations in $\Dz\to\Kp\Km\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1408.1299}{JHEP 10 (2014) 005, arXiv:1408.1299}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-045}}{\ifthenelse{\boolean{articletitles}}{``\textsl Determination of $\gamma$ and $-2\beta_s$ from charmless two-body decays of beauty mesons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1408.4368}{Phys. Lett. B739 (2015) 1, arXiv:1408.4368}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-044}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ violation in the three-body phase space of charmless $\Bpm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1408.5373}{Phys. Rev. D90 (2014) 112004, arXiv:1408.5373}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-043}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bs\to\Kstarpm\Kmp$ and evidence of $\Bs\to\Kstarm\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.7704}{New J. Phys. 16 (2014) 123001, arXiv:1407.7704}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-042}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bzb$--$\Bz$ and $\Bsb$--$\Bs$ production asymmetries in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1408.0275}{Phys. Lett. B739 (2014) 218, arXiv:1408.0275}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-041}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the CKM angle $\gamma$ using $\Bpm\to\D\Kpm$ with $\D\to\KS\pip\pim$, $\KS\Kp\Km$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1408.2748}{JHEP 10 (2014) 097, arXiv:1408.2748}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-040}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\chi_b(3P)$ mass and of the relative rate of $\chi_{b1}(1P)$ and $\chi_{b2}(1P)$ production'' }{}#1[LHCb, \href{http://arxiv.org/abs/1409.1408}{JHEP 10 (2014) 088, arXiv:1409.1408}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-039}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of a baryonic $\Bcp$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1408.0971}{Phys. Rev. Lett. 113 (2014) 152003, arXiv:1408.0971}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-038}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ asymmetry in $\Bs\to\Dsmp\Kpm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.6127}{JHEP 11 (2014) 060, arXiv:1407.6127}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-037}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bsb$ meson lifetime in $\Dsp\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.5873}{Phys. Rev. Lett. 113 (2014) 172001, arXiv:1407.5873}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-036}}{\ifthenelse{\boolean{articletitles}}{``\textsl Dalitz plot analysis of $\Bs\to\Dzb\Km\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.7712}{Phys. Rev. D90 (2014) 072003, arXiv:1407.7712}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-035}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of overlapping spin-$1$ and spin-$3$ $\Dzb\Km$ resonances at mass $2.86$\gevcc'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.7574}{Phys. Rev. Lett. 113 (2014) 162001, arXiv:1407.7574}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-034}}{\ifthenelse{\boolean{articletitles}}{``\textsl Evidence for $\CP$ violation in $\Bp\to\proton\antiproton\Kp$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.5907}{Phys. Rev. Lett. 113 (2014) 141801, arXiv:1407.5907}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-033}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the forward $\W$ boson production cross-section in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1408.4354}{JHEP 12 (2014) 079, arXiv:1408.4354}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-032}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ asymmetries in the decays $\Bz\to\Kstarz\mup\mun$ and $\Bp\to\Kp\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1408.0978}{JHEP 09 (2014) 177, arXiv:1408.0978}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-031}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $\chi_b$ meson production in $\proton\proton$ collisions at $\sqrt{s}=7$ and $8$\tev and observation of the decay $\chi_b \to \ThreeS\gamma$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.7734}{Eur. Phys. J. C74 (2014) 3092, arXiv:1407.7734}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-030}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observations of the rare decays $\Bp\to\Kp\pip\pim\mup\mun$ and $\Bp\to\phiz\Kp\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1408.1137}{JHEP 10 (2014) 064, arXiv:1408.1137}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-029}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\etac(1S)$ production cross-section in proton-proton collisions via the decay $\etac(1S) \to\proton\antiproton$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1409.3612}{Eur. Phys. J. C75 (2015) 311, arXiv:1409.3612}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-028}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ violation parameters in $\Bz\to\D\Kstarz$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.8136}{Phys. Rev. D90 (2014) 112002, arXiv:1407.8136}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-027}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of charmonium pairs produced exclusively in $\proton\proton$ collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.5973}{J. Phys. G41 (2014) 115002, arXiv:1407.5973}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-026}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ violation in $\Bs\to\phiz\phiz$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.2222}{Phys. Rev. D90 (2014) 052011, arXiv:1407.2222}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-025}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the ratio of $\Bcp$ branching fractions to $\jpsi\pip$ and $\jpsi\mup\neum$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.2126}{Phys. Rev. D90 (2014) 032009, arXiv:1407.2126}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-024}}{\ifthenelse{\boolean{articletitles}}{``\textsl Test of lepton universality using $\Bp\to\Kp\ell^+\ell^-$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1406.6482}{Phys. Rev. Lett. 113 (2014) 151601, arXiv:1406.6482}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-023}}{\ifthenelse{\boolean{articletitles}}{``\textsl First measurement of the charge asymmetry in beauty-quark pair production'' }{}#1[LHCb, \href{http://arxiv.org/abs/1406.4789}{Phys. Rev. Lett. 113 (2014) 082003, arXiv:1406.4789}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-022}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Z$ production in proton-lead collisions at LHCb'' }{}#1[LHCb, \href{http://arxiv.org/abs/1406.2885}{JHEP 09 (2014) 030, arXiv:1406.2885}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-021}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precision measurement of the mass and lifetime of the $\Xibz$ baryon'' }{}#1[LHCb, \href{http://arxiv.org/abs/1405.7223}{Phys. Rev. Lett. 113 (2014) 032001, arXiv:1405.7223}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-020}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the $\Lb\to\jpsi\proton\pim$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1406.0755}{JHEP 07 (2014) 103, arXiv:1406.0755}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-019}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$-violating phase $\phis$ in $\Bsb\to\jpsi\pim\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1405.4140}{Phys. Lett. B736 (2014) 186, arXiv:1405.4140}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for $\CP$ violation in $\Dpm\to\KS\Kpm$ and $\Dspm\to\KS\pipm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1406.2624}{JHEP 10 (2014) 025, arXiv:1406.2624}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ violation and constraints on the CKM angle $\gamma$ in $\Bpm\to\D\Kpm$ with $\D\to\KS\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1407.6211}{Nucl. Phys. B888 (2014) 169, arXiv:1407.6211}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the $\Bs\to\jpsi\KS\Kpm\pimp$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1405.3219}{JHEP 07 (2014) 140, arXiv:1405.3219}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $\Upsilon$ production and cold nuclear matter effects in $\proton$Pb collisions at $\sqrt{s_{NN}} = 5$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1405.5152}{JHEP 07 (2014) 094, arXiv:1405.5152}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the resonant character of the $Z(4430)^-$ state'' }{}#1[LHCb, \href{http://arxiv.org/abs/1404.1903}{Phys. Rev. Lett. 112 (2014) 222002, arXiv:1404.1903}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ asymmetry in $\Dz\to\Km\Kp$ and $\Dz\to\pim\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1405.2797}{JHEP 07 (2014) 041, arXiv:1405.2797}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the resonant and $\CP$ components in $\Bzb\to\jpsi\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1404.5673}{Phys. Rev. D90 (2014) 012003, arXiv:1404.5673}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl Effective lifetime measurements in the $\Bs\to\Kp\Km$, $\Bz\to\Kp\pim$ and $\Bs\to\pip\Km$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1406.7204}{Phys. Lett. B736 (2014) 446, arXiv:1406.7204}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Xibm$ and $\Omegab$ baryon lifetimes'' }{}#1[LHCb, \href{http://arxiv.org/abs/1405.1543}{Phys. Lett. B736 (2014) 154, arXiv:1405.1543}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl Evidence for the decay $\Bcp\to\jpsi 3\pip 2\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1404.0287}{JHEP 05 (2014) 148, arXiv:1404.0287}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl Evidence for the decay $X(3872)\to\psitwos\gamma$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1404.0275}{Nucl. Phys. B886 (2014) 665, arXiv:1404.0275}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl Angular analysis of charged and neutral $\B\to K\mup\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1403.8045}{JHEP 05 (2014) 082, arXiv:1403.8045}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl Differential branching fractions and isospin asymmetries of $\B\to\Kstar\mup\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1403.8044}{JHEP 06 (2014) 133, arXiv:1403.8044}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of polarization amplitudes and $\CP$ asymmetries in $\Bz\to\phiz\Kstar(892)^0$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1403.2888}{JHEP 05 (2014) 069, arXiv:1403.2888}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of the kinematic dependences of $\Lb$ production in $\proton\proton$ collisions and a measurement of the $\Lb\to\Lc\pim$ branching fraction'' }{}#1[LHCb, \href{http://arxiv.org/abs/1405.6842}{JHEP 08 (2014) 143, arXiv:1405.6842}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precision measurement of the ratio of the $\Lb$ to $\Bzb$ lifetimes'' }{}#1[LHCb, \href{http://arxiv.org/abs/1402.6242}{Phys. Lett. B734 (2014) 122, arXiv:1402.6242}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of beauty hadron decays into pairs of charm hadrons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1403.3606}{Phys. Rev. Lett. 112 (2014) 202001, arXiv:1403.3606}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of photon polarization in the $\bquark\to\squark\g$ transition'' }{}#1[LHCb, \href{http://arxiv.org/abs/1402.6852}{Phys. Rev. Lett. 112 (2014) 161801, arXiv:1402.6852}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-070}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of charged particle multiplicities and densities in $\proton\proton$ collisions at $\sqrt{s}=7$\tev in the forward region'' }{}#1[LHCb, \href{http://arxiv.org/abs/1402.4430}{Eur. Phys. J. C74 (2014) 2888, arXiv:1402.4430}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-069}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of resonant and $\CP$ components in $\Bsb\to\jpsi\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1402.6248}{Phys. Rev. D89 (2014) 092006, arXiv:1402.6248}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-068}}{\ifthenelse{\boolean{articletitles}}{``\textsl A study of $\CP$ violation in $\Bpm\to\D\Kpm$ and $\Bpm\to\D\pipm$ decays with $\D\to\KS\Kpm\pimp$ final states'' }{}#1[LHCb, \href{http://arxiv.org/abs/1402.2982}{Phys. Lett. B733 (2014) 36, arXiv:1402.2982}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-067}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\psitwos$ polarisation in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1403.1339}{Eur. Phys. J. C74 (2014) 2872, arXiv:1403.1339}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-066}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\Upsilon$ production in $\proton\proton$ collisions at $\sqrt{s} = 2.76$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1402.2539}{Eur. Phys. J. C74 (2014) 2835, arXiv:1402.2539}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-065}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of the $\Bp$, $\Bz$, $\Bs$ meson and $\Lb$ baryon lifetimes'' }{}#1[LHCb, \href{http://arxiv.org/abs/1402.2554}{JHEP 04 (2014) 114, arXiv:1402.2554}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-064}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for Majorana neutrinos in $\Bm\to\pip\mun\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1401.5361}{Phys. Rev. Lett. 112 (2014) 131802, arXiv:1401.5361}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-063}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bcp$ meson lifetime using $\Bcp\to\jpsi\mup\neum X$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1401.6932}{Eur. Phys. J. C74 (2014) 2839, arXiv:1401.6932}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-062}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of associated production of a $\Z$ boson with a $\D$ meson in the forward region'' }{}#1[LHCb, \href{http://arxiv.org/abs/1401.3245}{JHEP 04 (2014) 091, arXiv:1401.3245}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-061}}{\ifthenelse{\boolean{articletitles}}{``\textsl Searches for $\Lb$ and $\Xibz$ decays to $\KS\proton\pim$ and $\KS\proton\Km$ final states with first observation of the $\Lb \to\KS\proton\pim$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1402.0770}{JHEP 04 (2014) 087, arXiv:1402.0770}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-060}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bsb\to\Dsm\Dsp$ and $\Bsb\to\Dm\Dsp$ effective lifetimes'' }{}#1[LHCb, \href{http://arxiv.org/abs/1312.1217}{Phys. Rev. Lett. 112 (2014) 111802, arXiv:1312.1217}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-059}}{\ifthenelse{\boolean{articletitles}}{``\textsl Updated measurements of exclusive $\jpsi$ and $\psitwos$ production cross-sections in $\proton\proton$ collisions at $\sqrt{s} = 7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1401.3288}{J. Phys. G41 (2014) 055002, arXiv:1401.3288}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-058}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of forward $\Z$+jet production in $\proton\proton$ collisions at $\sqrt{s} = 7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1310.8197}{JHEP 01 (2014) 033, arXiv:1310.8197}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-057}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for $\CP$ violation in the decay $\Dp\to\pim\pip\pip$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1310.7953}{Phys. Lett. B728 (2014) 585, arXiv:1310.7953}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-056}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of beauty baryon decays to $\Dz\proton h^-$ and $\Lc h^-$ final states'' }{}#1[LHCb, \href{http://arxiv.org/abs/1311.4823}{Phys. Rev. D89 (2014) 032001, arXiv:1311.4823}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-055}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bzb_{\!\!\!\!\!(s)}\to\jpsi f_1(1285)$ decays and measurement of the $f_1(1285)$ mixing angle'' }{}#1[LHCb, \href{http://arxiv.org/abs/1310.2145}{Phys. Rev. Lett. 112 (2014) 091802, arXiv:1310.2145}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-054}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of indirect $\CP$ asymmetries in $\Dz\to\Km\Kp$ and $\Dz\to\pim\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1310.7201}{Phys. Rev. Lett. 112 (2014) 041801, arXiv:1310.7201}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-053}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\Dz$--$\Dzb$ mixing parameters and search for $\CP$ violation using $\Dz\to\Kp\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1309.6534}{Phys. Rev. Lett. 111 (2013) 251801, arXiv:1309.6534}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-052}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $\jpsi$ production and cold nuclear matter effects in $\proton$Pb collisions at $\sqrt{s_{NN}} = 5$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.6729}{JHEP 02 (2014) 072, arXiv:1308.6729}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-051}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ violation in the phase space of $\Bpm\to\Kp\Km\pipm$ and $\Bpm\to\pip\pim\pipm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1310.4740}{Phys. Rev. Lett. 112 (2014) 011801, arXiv:1310.4740}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-050}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the decay $\Dz\to\pip\pim\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1310.2535}{Phys. Lett. B728 (2014) 234, arXiv:1310.2535}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-049}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the doubly charmed baryon $\Xi_{cc}^+$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1310.2538}{JHEP 12 (2013) 090, arXiv:1310.2538}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-048}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the charge asymmetry in $\Bpm\to\phiz\Kpm$ and search for $\Bpm \to\phiz\pipm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1309.3742}{Phys. Lett. B728 (2014) 85, arXiv:1309.3742}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-047}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decay $\Bcp\to\jpsi\Kp\Km\pip$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1309.0587}{JHEP 11 (2013) 094, arXiv:1309.0587}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-046}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bs\to\mup\mun$ branching fraction and search for $\Bz\to\mup\mun$ decays at the LHCb experiment'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.5024}{Phys. Rev. Lett. 111 (2013) 101805, arXiv:1307.5024}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-045}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of $\Bzb\to\jpsi\Kp\Km$ and search for $\Bzb\to\jpsi\phiz$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.5916}{Phys. Rev. D88 (2013) 072005, arXiv:1308.5916}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-044}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decay $\Bcp\to \Bs\pip$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.4544}{Phys. Rev. Lett. 111 (2013) 181801, arXiv:1308.4544}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-043}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$ asymmetry in $\Bp\to\Kp\mup\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.1340}{Phys. Rev. Lett. 111 (2013) 151801, arXiv:1308.1340}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-042}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $B_{(s)}^0 \to\KS h^+ h^{\prime -}$ decays with first observation of $\Bs\to\KS\Kpm\pimp$ and $\Bs\to\KS\pip\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.7648}{JHEP 10 (2013) 143, arXiv:1307.7648}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-041}}{\ifthenelse{\boolean{articletitles}}{``\textsl Model-independent search for $\CP$ violation in $\Dz\to\Km\Kp\pip\pim$ and $\Dz\to\pim\pip\pim\pip$ decays '' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.3189}{Phys. Lett. B726 (2013) 623, arXiv:1308.3189}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-040}}{\ifthenelse{\boolean{articletitles}}{``\textsl First measurement of time-dependent $\CP$ violation in $\Bs\to\Kp\Km$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.1428}{JHEP 10 (2013) 183, arXiv:1308.1428}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-039}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of a resonance in $\Bp\to\Kp\mup\mun$ decays at low recoil'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.7595}{Phys. Rev. Lett. 111 (2013) 112003, arXiv:1307.7595}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-038}}{\ifthenelse{\boolean{articletitles}}{``\textsl First evidence for the two-body charmless baryonic decay $\Bz\to\proton\antiproton$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.0961}{JHEP 10 (2013) 005, arXiv:1308.0961}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-037}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of form-factor-independent observables in the decay $\Bz\to\Kstarz\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.1707}{Phys. Rev. Lett. 111 (2013) 191801, arXiv:1308.1707}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-036}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bs$--$\Bsb$ mixing and measurement of mixing frequencies using semileptonic $\B$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.1302}{Eur. Phys. J. C73 (2013) 2655, arXiv:1308.1302}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-035}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decay $\Bs\to\Dzb\phis$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.4583}{Phys. Lett. B727 (2013) 403, arXiv:1308.4583}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-034}}{\ifthenelse{\boolean{articletitles}}{``\textsl Branching fraction and $\CP$ asymmetry of the decays $\Bp\to\KS\pip$ and $\Bp\to\KS\Kp$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.1277}{Phys. Lett. B726 (2013) 646, arXiv:1308.1277}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-033}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the flavour-specific $\CP$-violating asymmetry $a_{\mathrm{sl}}^s$ in $\Bs$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1308.1048}{Phys. Lett. B728 (2014) 607, arXiv:1308.1048}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-032}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precision measurement of the $\Lb$ baryon lifetime'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.2476}{Phys. Rev. Lett. 111 (2013) 102003, arXiv:1307.2476}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-031}}{\ifthenelse{\boolean{articletitles}}{``\textsl Studies of the decays $\Bp\to\proton\antiproton h^+$ and observation of $\Bp\to \Lbar(1520)\proton$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.6165}{Phys. Rev. D88 (2013) 052015, arXiv:1307.6165}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-030}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the lepton-flavour-violating decays $\Bs \to \epm\muon^\mp$ and $\Bz\to\epm \muon^\mp$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.4889}{Phys. Rev. Lett. 111 (2013) 141801, arXiv:1307.4889}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-029}}{\ifthenelse{\boolean{articletitles}}{``\textsl Searches for $B^0_{(s)}\to\jpsi \proton\antiproton$ and $\Bp\to\jpsi\proton\antiproton\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1306.4489}{JHEP 09 (2013) 006, arXiv:1306.4489}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-028}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the relative rate of prompt $\chiczero$, $\chicone$ and $\chictwo$ production at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.4285}{JHEP 10 (2013) 115, arXiv:1307.4285}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-027}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ violation in the phase space of $\Bpm\to\Kpm\pip\pim$ and $\Bpm\to\Kpm\Kp\Km$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1306.1246}{Phys. Rev. Lett. 111 (2013) 101801, arXiv:1306.1246}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-026}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $D_J$ meson decays to $\Dp\pim$, $\Dz\pip$ and $\Dstarp\pim$ final states in $\proton\proton$ collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.4556}{JHEP 09 (2013) 145, arXiv:1307.4556}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-025}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the differential branching fraction of the decay $\Lb\to\Lz\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1306.2577}{Phys. Lett. B725 (2013) 25, arXiv:1306.2577}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-024}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bs\to\chicone\phiz$ decay and study of $\Bz\to\chi_{c1,2}\Kstarz$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1305.6511}{Nucl. Phys. B874 (2013) 663, arXiv:1305.6511}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-023}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the polarization amplitudes in $\Bz\to\jpsi\Kstar(892)^0$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.2782}{Phys. Rev. D88 (2013) 052002, arXiv:1307.2782}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-022}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of the branching fractions of the decays $\Bs\to\Dzb\Km\pip$ and $\Bz\to\Dzb\Kp\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.6317}{Phys. Rev. D87 (2013) 112009, arXiv:1304.6317}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-021}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decay $\Bcp\to\jpsi\Kp$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1306.6723}{JHEP 09 (2013) 075, arXiv:1306.6723}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-020}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the CKM angle $\gamma$ from a combination of $\Bpm\to\D h^\pm$ analyses'' }{}#1[LHCb, \href{http://arxiv.org/abs/1305.2050}{Phys. Lett. B726 (2013) 151, arXiv:1305.2050}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-019}}{\ifthenelse{\boolean{articletitles}}{``\textsl Differential branching fraction and angular analysis of the decay $\Bz\to\Kstarz\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.6325}{JHEP 08 (2013) 131, arXiv:1304.6325}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of $\CP$ violation in the decays of $\Bs$ mesons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.6173}{Phys. Rev. Lett. 110 (2013) 221601, arXiv:1304.6173}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl Differential branching fraction and angular analysis of the decay $\Bs\to\phiz\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1305.2168}{JHEP 07 (2013) 084, arXiv:1305.2168}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl Production of $\jpsi$ and $\Upsilon$ mesons in $\proton\proton$ collisions at $\sqrt{s}=8$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.6977}{JHEP 06 (2013) 064, arXiv:1304.6977}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the effective $\Bs\to\jpsi\KS$ lifetime'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.4500}{Nucl. Phys. B873 (2013) 275-292, arXiv:1304.4500}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl Searches for violation of lepton flavour and baryon number in tau lepton decays at LHCb'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.4518}{Phys. Lett. B724 (2013) 36, arXiv:1304.4518}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the rare decay $\Dz\to\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1305.5059}{Phys. Lett. B725 (2013) 15, arXiv:1305.5059}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decay $\Bs\to\phiz\Kstarzb$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1306.2239}{JHEP 11 (2013) 092, arXiv:1306.2239}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precision measurement of $\D$ meson mass differences'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.6865}{JHEP 06 (2013) 065, arXiv:1304.6865}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bcp\to\jpsi\Dsp$ and $\Bcp\to\jpsi\Dssp$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.4530}{Phys. Rev. D87 (2013) 112012, arXiv:1304.4530}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl Limits on neutral Higgs boson production in the forward region in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.2591}{JHEP 05 (2013) 132, arXiv:1304.2591}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\jpsi$ polarization in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1307.6379}{Eur. Phys. J. C73 (2013) 2631, arXiv:1307.6379}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl First measurement of the $\CP$-violating phase in $\Bs\to\phiz\phiz$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1303.7125}{Phys. Rev. Lett. 110 (2013) 241802, arXiv:1303.7125}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl Precision measurement of the $\Bs$--$\Bsb$ oscillation frequency in the decay $\Bs\to\Dsm\pip$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.4741}{New J. Phys. 15 (2013) 053021, arXiv:1304.4741}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bz\to\Kstarz\epem$ branching fraction at low dilepton mass'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.3035}{JHEP 05 (2013) 159, arXiv:1304.3035}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\B$ meson production cross-sections in proton-proton collisions at $\sqrt{s} = 7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1306.3663}{JHEP 08 (2013) 117, arXiv:1306.3663}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for direct $\CP$ violation in $\Dz\to h^- h^+$ modes using semileptonic $\B$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1303.2614}{Phys. Lett. B723 (2013) 33, arXiv:1303.2614}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ violation and the $\Bs$ meson decay width difference with $\Bs\to\jpsi\Kp\Km$ and $\Bs\to\jpsi\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.2600}{Phys. Rev. D87 (2013) 112010, arXiv:1304.2600}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl Determination of the $X(3872)$ meson quantum numbers'' }{}#1[LHCb, \href{http://arxiv.org/abs/1302.6269}{Phys. Rev. Lett. 110 (2013) 222001, arXiv:1302.6269}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-057}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of the $\Lb\to\jpsi\Lz$ decay amplitudes and the $\Lb$ polarisation in $\proton\proton$ collisions at $\sqrt{s} = 7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1302.5578}{Phys. Lett. B724 (2013) 27, arXiv:1302.5578}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-056}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the decay $\Bs\to\Dssmp\pipm$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1302.6446}{Phys. Rev. D87 (2013) 071101(R), arXiv:1302.6446}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-055}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the suppressed ADS modes $\Bpm \to [\pipm\Kmp\pip\pim]_D \Kpm$ and $\Bpm \to [\pipm\Kmp\pip\pim]_D \pipm$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1303.4646}{Phys. Lett. B723 (2013) 44, arXiv:1303.4646}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-054}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of the decay $\Bcp\to\psitwos\pip$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1303.1737}{Phys. Rev. D87 (2013) 071103(R), arXiv:1303.1737}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-053}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observations of $\Bs\to\psitwos\eta$ and $B^0_{(s)}\to\psitwos\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1302.6354}{Nucl. Phys. B871 (2013) 403 - 419, arXiv:1302.6354}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-052}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for $\CP$ violation in $\Dp\to\phiz\pip$ and $\Dsp\to\KS\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1303.4906}{JHEP 06 (2013) 112, arXiv:1303.4906}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-051}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for $D^+_{(s)}\to\pip\mup\mun$ and $D^+_{(s)}\to\pim\mup\mup$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1304.6365}{Phys. Lett. B724 (2013) 203, arXiv:1304.6365}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-050}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observations of $\Bsb\to\Dp\Dm$, $\Dsp\Dm$ and $\Dz\Dzb$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1302.5854}{Phys. Rev. D87 (2013) 092007, arXiv:1302.5854}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-049}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for rare $B_{(s)}^0\to\mup\mun\mup\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1303.1092}{Phys. Rev. Lett. 110 (2013) 211801, arXiv:1303.1092}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-048}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of the $\Lb$, $\Xibm$, and $\Omegab$ baryon masses'' }{}#1[LHCb, \href{http://arxiv.org/abs/1302.1072}{Phys. Rev. Lett. 110 (2013) 182001, arXiv:1302.1072}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-047}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of the branching fractions of $Bp\to\proton\antiproton\Kp$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1303.7133}{Eur. Phys. J. C73 (2013) 2462, arXiv:1303.7133}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-046}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $\Bz\to\Dstarm\pip\pim\pip$ and $\Bz\to\Dstarm\Kp\pim\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1303.6861}{Phys. Rev. D87 (2013) 092001, arXiv:1303.6861}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-045}}{\ifthenelse{\boolean{articletitles}}{``\textsl Analysis of the resonant components in $\Bzb\to\jpsi\pip\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1301.5347}{Phys. Rev. D87 (2013) 052001, arXiv:1301.5347}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-044}}{\ifthenelse{\boolean{articletitles}}{``\textsl Exclusive $\jpsi$ and $\psitwos$ production in $\proton\proton$ collisions at $\sqrt{s} = 7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1301.7084}{J. Phys. G40 (2013) 045001, arXiv:1301.7084}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-043}}{\ifthenelse{\boolean{articletitles}}{``\textsl First evidence for the decay $\Bs\to\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1211.2674}{Phys. Rev. Lett. 110 (2013) 021801, arXiv:1211.2674}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-042}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\CP$ observables in $\Bz\to\D\Kstarz$ with $\D\to\Kp\Km$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1212.5205}{JHEP 03 (2013) 067, arXiv:1212.5205}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-041}}{\ifthenelse{\boolean{articletitles}}{``\textsl Prompt charm production in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1302.2864}{Nucl. Phys. B871 (2013) 1, arXiv:1302.2864}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-040}}{\ifthenelse{\boolean{articletitles}}{``\textsl Amplitude analysis and branching fraction measurement of $\Bsb \to\jpsi\Kp\Km$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1302.1213}{Phys. Rev. D87 (2013) 072004, arXiv:1302.1213}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-039}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\jpsi$ production in $\proton\proton$ collisions at $\sqrt{s}=2.76$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1212.1045}{JHEP 02 (2013) 041, arXiv:1212.1045}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-038}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Dz$--$\Dzb$ oscillations'' }{}#1[LHCb, \href{http://arxiv.org/abs/1211.1230}{Phys. Rev. Lett. 110 (2013) 101802, arXiv:1211.1230}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-037}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the fragmentation fraction ratio $f_s/f_d$ and its dependence on $\B$ meson kinematics'' }{}#1[LHCb, \href{http://arxiv.org/abs/1301.5286}{JHEP 04 (2013) 001, arXiv:1301.5286}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-036}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the cross-section for $\Z\to\epem$ production in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1212.4620}{JHEP 02 (2013) 106, arXiv:1212.4620}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-035}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the time-dependent $\CP$ asymmetry in $\Bz\to\jpsi\KS$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1211.6093}{Phys. Lett. B721 (2013) 24, arXiv:1211.6093}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-034}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the forward energy flow in $\proton\proton$ collisions at $\sqrt{s}= 7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1212.4755}{Eur. Phys. J. C73 (2013) 2421, arXiv:1212.4755}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-033}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decays $\Bzb_{\!\!\!\!(s)} \to\Dsp\Km\pip\pim$ and $\Bsb\to D_{s1}(2536)^+\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1211.1541}{Phys. Rev. D86 (2012) 112005, arXiv:1211.1541}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-032}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bz$--$\Bzb$ oscillation frequency $\dmd$ with the decays $\Bz\to\Dm\pip$ and $\Bz\to\jpsi\Kstarz$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1210.6750}{Phys. Lett. B719 (2013) 318, arXiv:1210.6750}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-031}}{\ifthenelse{\boolean{articletitles}}{``\textsl Implications of LHCb measurements and future prospects'' }{}#1[LHCb, \href{http://arxiv.org/abs/1208.3355}{Eur. Phys. J. C73 (2013) 2373, arXiv:1208.3355}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-030}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decay $B_{s2}^*(5840)^0 \to B^{*+}\Km$ and studies of excited $\Bs$ mesons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1211.5994}{Phys. Rev. Lett. 110 (2013) 151803, arXiv:1211.5994}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-029}}{\ifthenelse{\boolean{articletitles}}{``\textsl A study of the $\Z$ production cross-section in $\proton\proton$ collisions at $\sqrt{s}=7$\tev using tau final states'' }{}#1[LHCb, \href{http://arxiv.org/abs/1210.6289}{JHEP 01 (2013) 111, arXiv:1210.6289}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-028}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of $\Bcp$ production and mass with the $\Bcp\to\jpsi\pip$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1209.5634}{Phys. Rev. Lett. 109 (2012) 232001, arXiv:1209.5634}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-027}}{\ifthenelse{\boolean{articletitles}}{``\textsl A model-independent Dalitz plot analysis of $\Bpm\to\D\Kpm$ with $\D\to\KS h^+h^-$ ($h=\pi, K$) decays and constraints on the CKM angle $\gamma$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1209.5869}{Phys. Lett. B718 (2012) 43-55, arXiv:1209.5869}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-026}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Dpm$ production asymmetry in $7$\tev $\proton\proton$ collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1210.4112}{Phys. Lett. B718 (2013) 902-909, arXiv:1210.4112}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-025}}{\ifthenelse{\boolean{articletitles}}{``\textsl First evidence for the annihilation decay mode $\Bp\to\Dsp\phiz$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1210.1089}{JHEP 02 (2013) 043, arXiv:1210.1089}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-024}}{\ifthenelse{\boolean{articletitles}}{``\textsl Differential branching fraction and angular analysis of the $\Bp\to\Kp\mup\mun$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1209.4284}{JHEP 02 (2013) 105, arXiv:1209.4284}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-023}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the rare decay $\KS\to\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1209.4029}{JHEP 01 (2013) 090, arXiv:1209.4029}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-022}}{\ifthenelse{\boolean{articletitles}}{``\textsl Evidence for the decay $\Bz\to\jpsi\omegaz$ and measurement of the relative branching fractions of $\Bs$ meson decays to $\jpsi\etaz$ and $\jpsi\etapr$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1210.2631}{Nucl. Phys. B867 (2013) 547-566, arXiv:1210.2631}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-021}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$ asymmetry in $\Bz\to\Kstarz\mup\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1210.4492}{Phys. Rev. Lett. 110 (2013) 031801, arXiv:1210.4492}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-020}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decay $\Bp\to\pip\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1210.2645}{JHEP 12 (2012) 125, arXiv:1210.2645}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-019}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the ratio of branching fractions $\BF(\Bz\to\Kstarz\g) / \BF(\Bs\to\phiz\g)$ and the direct $\CP$ asymmetry in $\Bz\to\Kstarz\g$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1209.0313}{Nucl. Phys. B867 (2013) 1-18, arXiv:1209.0313}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bz\to\Dzb\Kp\Km$ and evidence for $\Bs\to\Dzb\Kp\Km$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1207.5991}{Phys. Rev. Lett. 109 (2012) 131801, arXiv:1207.5991}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bsb$ effective lifetime in the $\jpsi f_0(980)$ final state'' }{}#1[LHCb, \href{http://arxiv.org/abs/1207.0878}{Phys. Rev. Lett. 109 (2012) 152002, arXiv:1207.0878}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl Study of $D_{sJ}$ decays to $\Dp\KS$ and $\Dz\Kp$ final states in $\proton\proton$ collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1207.6016}{JHEP 10 (2012) 151, arXiv:1207.6016}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the fraction of $\OneS$ originating from $\chi_b(1P)$ decays in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1209.0282}{JHEP 11 (2012) 031, arXiv:1209.0282}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bs\to\jpsi\Kstarzb$ branching fraction and angular amplitudes'' }{}#1[LHCb, \href{http://arxiv.org/abs/1208.0738}{Phys. Rev. D86 (2012) 071102(R), arXiv:1208.0738}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the effective $\Bs\to\Kp\Km$ lifetime'' }{}#1[LHCb, \href{http://arxiv.org/abs/1207.5993}{Phys. Lett. B716 (2012) 393-400, arXiv:1207.5993}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of excited $\Lb$ baryons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1205.3452}{Phys. Rev. Lett. 109 (2012) 172003, arXiv:1205.3452}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the isospin asymmetry in $\B\to\Kstar\mup\mun$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1205.3422}{JHEP 07 (2012) 133, arXiv:1205.3422}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of relative branching fractions of $\B$ decays to $\psitwos$ and $\jpsi$ mesons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1205.0918}{Eur. Phys. J. C72 (2012) 2118, arXiv:1205.0918}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Dsp$--$\Dsm$ production asymmetry in $7$\tev $\proton\proton$ collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1205.0897}{Phys. Lett. B713 (2012) 186-195, arXiv:1205.0897}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl Inclusive $\W$ and $\Z$ production in the forward region at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1204.1620}{JHEP 06 (2012) 058, arXiv:1204.1620}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl Strong constraints on the rare decays $\Bs\to\mup\mun$ and $\Bz\to\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1203.4493}{Phys. Rev. Lett. 108 (2012) 231801, arXiv:1203.4493}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$-violating phase $\phis$ in $\Bsb\to\jpsi\pip\pim$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1204.5675}{Phys. Lett. B713 (2012) 378-386, arXiv:1204.5675}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl Analysis of the resonant components in $\Bsb\to\jpsi\pip\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1204.5643}{Phys. Rev. D86 (2012) 052006, arXiv:1204.5643}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the polarization amplitudes and triple product asymmetries in the $\Bs\to\phiz\phiz$ decay'' }{}#1[LHCb, \href{http://arxiv.org/abs/1204.2813}{Phys. Lett. B713 (2012) 369-377, arXiv:1204.2813}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of double charm production involving open charm in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1205.0975}{JHEP 06 (2012) 141, arXiv:1205.0975}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\bquark$-hadron branching fractions for two-body decays into charmless charged hadrons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1206.2794}{JHEP 10 (2012) 037, arXiv:1206.2794}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\CP$ violation in $\Bpm\to\D\Kpm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1203.3662}{Phys. Lett. B712 (2012) 203, arXiv:1203.3662}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-045}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\psitwos$ meson production in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1204.1258}{Eur. Phys. J. C72 (2012) 2100, arXiv:1204.1258}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-044}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decay $\Bcp\to\jpsi\pip\pim\pip$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1204.0079}{Phys. Rev. Lett. 108 (2012) 251802, arXiv:1204.0079}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-043}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bpm$ production cross-section in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1202.4812}{JHEP 04 (2012) 093, arXiv:1202.4812}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-042}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the ratio of branching fractions $\BF(\Bz\to\Kstarz\g)/\BF(\Bs\to\phiz\g)$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1202.6267}{Phys. Rev. D85 (2012) 112013, arXiv:1202.6267}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-041}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $B^0_s \to J/\psi K^0_S$ branching fraction'' }{}#1[LHCb, \href{http://arxiv.org/abs/1205.0934}{Phys. Lett. B713 (2012) 172-179, arXiv:1205.0934}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-040}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decays $\Bzb\to\Dp\Km\pip\pim$ and $\Bm \to\Dz\Km\pip\pim$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1201.4402}{Phys. Rev. Lett. 108 (2012) 161801, arXiv:1201.4402}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-038}}{\ifthenelse{\boolean{articletitles}}{``\textsl Searches for Majorana neutrinos in $\Bm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1201.5600}{Phys. Rev. D85 (2012) 112004, arXiv:1201.5600}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-037}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of prompt hadron production ratios in $\proton\proton$ collisions at $\sqrt{s}=0.9$ and $7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1206.5160}{Eur. Phys. J. C72 (2012) 2168, arXiv:1206.5160}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-036}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\Upsilon$ production in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1202.6579}{Eur. Phys. J. C72 (2012) 2025, arXiv:1202.6579}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-035}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\bquark$-hadron masses'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.4896}{Phys. Lett. B708 (2012) 241, arXiv:1112.4896}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-034}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $X(3872)$ production in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.5310}{Eur. Phys. J. C72 (2012) 1972, arXiv:1112.5310}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-033}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the $X(4140)$ state in $\Bp\to\jpsi\phiz\Kp$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1202.5087}{Phys. Rev. D85 (2012) 091103(R), arXiv:1202.5087}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-032}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of mixing and $\CP$ violation parameters in two-body charm decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.4698}{JHEP 04 (2012) 129, arXiv:1112.4698}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-031}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$ violating phase $\phis$ in $\Bsb\to\jpsi f_0(980)$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.3056}{Phys. Lett. B707 (2012) 497, arXiv:1112.3056}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-030}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the ratio of prompt $\chi_{c}$ to $\jpsi$ production in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1204.1462}{Phys. Lett. B718 (2012) 431, arXiv:1204.1462}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-029}}{\ifthenelse{\boolean{articletitles}}{``\textsl First evidence of direct $\CP$ violation in charmless two-body decays of $\Bs$ mesons'' }{}#1[LHCb, \href{http://arxiv.org/abs/1202.6251}{Phys. Rev. Lett. 108 (2012) 201601, arXiv:1202.6251}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-028}}{\ifthenelse{\boolean{articletitles}}{``\textsl Determination of the sign of the decay width difference in the $\Bs$ system'' }{}#1[LHCb, \href{http://arxiv.org/abs/1202.4717}{Phys. Rev. Lett. 108 (2012) 241801, arXiv:1202.4717}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-027}}{\ifthenelse{\boolean{articletitles}}{``\textsl Opposite-side flavour tagging of $\B$ mesons at the LHCb experiment'' }{}#1[LHCb, \href{http://arxiv.org/abs/1202.4979}{Eur. Phys. J. C72 (2012) 2022, arXiv:1202.4979}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-026}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\Bsb\to\jpsi f'_2(1525)$ in $\jpsi\Kp\Km$ final states'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.4695}{Phys. Rev. Lett. 108 (2012) 151801, arXiv:1112.4695}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-025}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the rare decays $\Bs\to\mup\mun$ and $\Bz\to\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.1600}{Phys. Lett. B708 (2012) 55, arXiv:1112.1600}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-024}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of the branching fractions and $\CP$ asymmetries of $\Bpm\to\jpsi\pipm$ and $\Bpm\to\psitwos\pipm$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1203.3592}{Phys. Rev. D85 (2012) 091105(R), arXiv:1203.3592}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-023}}{\ifthenelse{\boolean{articletitles}}{``\textsl Evidence for $\CP$ violation in time-integrated $\Dz\to h^-h^+$ decay rates'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.0938}{Phys. Rev. Lett. 108 (2012) 111602, arXiv:1112.0938}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-022}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of the branching fractions of the decays $\Bs\to\Dsmp\Kpm$ and $\Bs\to\Dsm\pip$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1204.1237}{JHEP 06 (2012) 115, arXiv:1204.1237}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-021}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\CP$-violating phase $\phis$ in the decay $\Bs\to\jpsi\phiz$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.3183}{Phys. Rev. Lett. 108 (2012) 101803, arXiv:1112.3183}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-020}}{\ifthenelse{\boolean{articletitles}}{``\textsl Differential branching fraction and angular analysis of the decay $\Bz\to\Kstarz\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.3515}{Phys. Rev. Lett. 108 (2012) 181806, arXiv:1112.3515}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-019}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the cross-section ratio $\sigma(\chictwo)/\sigma(\chicone)$ for prompt $\chi_c$ production at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1202.1080}{Phys. Lett. B714 (2012) 215-223, arXiv:1202.1080}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\bquark$ hadron production fractions in 7\,TeV $\proton\proton$ collisions'' }{}#1[LHCb, \href{http://arxiv.org/abs/1111.2357}{Phys. Rev. D85 (2012) 032008, arXiv:1111.2357}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for $\CP$ violation in $\Dp\to\Km\Kp\pip$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1110.3970}{Phys. Rev. D84 (2011) 112008, arXiv:1110.3970}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurements of the branching fractions for $B_{(s)}\to D_{(s)}\pi\pi\pi$ and $\Lb\to\Lc\pi\pi\pi$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1109.6831}{Phys. Rev. D84 (2011) 092001, arXiv:1109.6831}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl Absolute luminosity measurements with the LHCb detector at the LHC'' }{}#1[LHCb, \href{http://arxiv.org/abs/1110.2866}{JINST 7 (2012) P01010, arXiv:1110.2866}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the effective $\Bs\to\Kp\Km$ lifetime'' }{}#1[LHCb, \href{http://arxiv.org/abs/1111.0521}{Phys. Lett. B707 (2012) 349, arXiv:1111.0521}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl Observation of $\jpsi$-pair production in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1109.0963}{Phys. Lett. B707 (2012) 52, arXiv:1109.0963}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decay $\Bs\to\Kstarz\Kstarzb$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1111.4183}{Phys. Lett. B709 (2012) 50, arXiv:1111.4183}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of charged particle multiplicities in $\proton\proton$ collisions at $\sqrt{s}=7$\tev in the forward region'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.4592}{Eur. Phys. J. C72 (2012) 1947, arXiv:1112.4592}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the $\Bs$--$\Bsb$ oscillation frequency $\dms$ in $\Bs\to\Dsm (3)\pi$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1112.4311}{Phys. Lett. B709 (2012) 177, arXiv:1112.4311}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for lepton number violating decays $\Bp\to\pim\mup\mup$ and $\Bp\to\Km\mup\mup$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1110.0730}{Phys. Rev. Lett. 108 (2012) 101601, arXiv:1110.0730}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of the decay $\Bsb\to\Dz\Kstarz$ and a measurement of the ratio of branching fractions $\frac{\BF(\Bsb\to\Dz\Kstarz)}{\BF(\Bz\to\Dz\rhoz)}$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1110.3676}{Phys. Lett. B706 (2011) 32, arXiv:1110.3676}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of the inclusive $\phiz$ cross-section in $\proton\proton$ collisions at $\sqrt{s}=7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1107.3935}{Phys. Lett. B703 (2011) 267, arXiv:1107.3935}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl Determination of $f_s/f_d$ for 7 TeV $\proton\proton$ collisions and measurement of the $\Bz\to\Dm\Kp$ branching fraction'' }{}#1[LHCb, \href{http://arxiv.org/abs/1106.4435}{Phys. Rev. Lett. 107 (2011) 211801, arXiv:1106.4435}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $V^0$ production ratios in $\proton\proton$ collisions at $\sqrt{s} = 0.9$ and $7$\tev'' }{}#1[LHCb, \href{http://arxiv.org/abs/1107.0882}{JHEP 08 (2011) 034, arXiv:1107.0882}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl Search for the rare decays $\Bs\to\mup\mun$ and $\Bz\to\mup\mun$'' }{}#1[LHCb, \href{http://arxiv.org/abs/1103.2465}{Phys. Lett. B699 (2011) 330, arXiv:1103.2465}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\jpsi$ production in $\proton\proton$ collisions at $\sqrt{s}=7$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1103.0423}{Eur. Phys. J. C71 (2011) 1645, arXiv:1103.0423}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of $\Bs\to\jpsi f_0(980)$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1102.0206}{Phys. Lett. B698 (2011) 115, arXiv:1102.0206}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl First observation of $\Bsb\to D_{s2}^{*+} X \mun\neub$ decays'' }{}#1[LHCb, \href{http://arxiv.org/abs/1102.0348}{Phys. Lett. B698 (2011) 14, arXiv:1102.0348}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2010-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl Measurement of $\sigma(pp\to\bbbar X)$ at $\sqrt{s}=7$ TeV in the forward region'' }{}#1[LHCb, \href{http://arxiv.org/abs/1009.2731}{Phys. Lett. B694 (2010) 209, arXiv:1009.2731}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2010-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl Prompt $\KS$ production in $\proton\proton$ collisions at $\sqrt{s}=0.9$\,TeV'' }{}#1[LHCb, \href{http://arxiv.org/abs/1008.3105}{Phys. Lett. B693 (2010) 69, arXiv:1008.3105}, ]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl {TBC}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-008}{LHCb-CONF-2017-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl {TBC}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-007}{LHCb-CONF-2017-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl {TBC}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-006}{LHCb-CONF-2017-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Prompt $\Lambda^+_c$ production in $p$Pb collisions at $\sqrt{s_{NN}} = 5.02$ TeV}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-005}{LHCb-CONF-2017-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the CKM angle $\gamma$ from a combination of $B\to DK$ analyses}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-004}{LHCb-CONF-2017-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Abandoned - not to be used}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-003}{LHCb-CONF-2017-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of antiproton production in $p$He collisions at $\sqrt{s_{NN}} = 110$ GeV}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-002}{LHCb-CONF-2017-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of $\jpsi$ and $\Dz$ production in $p$Ar collisions at $\sqrt{s_{NN}} = 110$ GeV}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-001}{LHCb-CONF-2017-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of time-dependent $C\!P$ violating                          asymmetries in $B^0 \to \pi^+\pi^-$ and                          $B^0_s \to K^+ K^-$ decays at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-018}{LHCb-CONF-2016-018}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl {*** UNASSIGNED ***}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-017}{LHCb-CONF-2016-017}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First observation of a baryonic $B^0_s$ decay}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-016}{LHCb-CONF-2016-016}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of $C\!P$ asymmetry in $B^0_s \to D_s^\mp K^\pm$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-015}{LHCb-CONF-2016-015}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Study of the decay $B^\pm \to DK^{\ast \pm}$ with two-body $D$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-014}{LHCb-CONF-2016-014}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Evidence for the rare decay $\Sigma^+ \to p\mumu$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-013}{LHCb-CONF-2016-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the decay $\KS\to\mumu$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-012}{LHCb-CONF-2016-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the rare decays $B_{(s)}^0 \to \taup\taum$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-011}{LHCb-CONF-2016-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl {$\CP$-violating asymmetries from the decay time distribution of                         promt $\Dz\to\Kp\Km$ and $\Dz\to\pip\pim$ decays in the full                         LHCb Run 1 data sample. Measurement using unbinned, acceptance                         corrected decay-time}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-010}{LHCb-CONF-2016-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl {$\CP$-violating asymmetries from the decay time distribution of                         promt $\Dz\to\Kp\Km$ and $\Dz\to\pip\pim$ decays in the full                         LHCb Run 1 data sample. Measurement using yield asymmetries in bins of decay time}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-009}{LHCb-CONF-2016-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Dalitz plot analysis of the $\Dp \to \Km\Kp\Kp$                          decay with the isobar model}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-008}{LHCb-CONF-2016-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Central exclusive production of $\jpsi$ and                          $\psitwos$ mesons in $pp$ collisions                          at $\sqrt{s}=13\,$TeV}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-007}{LHCb-CONF-2016-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for $\H\to \bbbar$ or $\ccbar$ in                         association with a $\W$ or $\Z$ boson in                          the forward region of $pp$ collisions}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-006}{LHCb-CONF-2016-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl {LHCb dimuon and charm mass distributions}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-005}{LHCb-CONF-2016-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for structure in the $B^0_s \pi^\pm$                          invariant mass spectrum}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-004}{LHCb-CONF-2016-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Study of cold nuclear matter effect using prompt                         $D^0$ meson production in $p$Pb collisions at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-003}{LHCb-CONF-2016-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $Z \to \mu\mu$ production cross-section                         at forward rapidities in $pp$ collisions at ${\sqrt s} = 13$~TeV}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-002}{LHCb-CONF-2016-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl {LHCb $\gamma$ combination update from $B \to DKX$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-001}{LHCb-CONF-2016-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Study of $\psi(2S)$ production and cold nuclear matter                          effects in $p$Pb collisions at $\sqrt {s_{NN}} = 5$ TeV}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-005}{LHCb-CONF-2015-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First measurements of long-range near-side angular                          correlations in $\sqrt{s_\text{NN} }= 5$ TeV                          proton-lead collisions in the forward region}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-004}{LHCb-CONF-2015-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $B^0$ oscillation frequency                          $\Delta m_d$ with $B^0\to D^{(*)-}\mu^+\nu_\mu$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-003}{LHCb-CONF-2015-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Angular analysis of the $B_d^0\to K^{*0}\mu^+\mu^-$ decay}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-002}{LHCb-CONF-2015-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Study of the decay $B^+\to K^+\pi^0$ at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-001}{LHCb-CONF-2015-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2014-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Improved constraints on $\gamma$: CKM2014 update}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2014-004}{LHCb-CONF-2014-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2014-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Reference pp cross-sections for $\Upsilon(1S)$                         studies in proton-lead collisions at                         $\sqrt{s_{NN}} = 5.02$~TeV and comparisons                         between ALICE and LHCb results}'' }{}#1[{ALICE and LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2014-003}{LHCb-CONF-2014-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2014-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the forward $W$ boson cross-section                         in $pp$ collisions at $\sqrt{s}=7$ TeV}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2014-002}{LHCb-CONF-2014-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2014-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl {A search for heavy long-lived stau pair production                         in the LHCb detector}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2014-001}{LHCb-CONF-2014-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Reference $pp$ cross-sections for $J/\psi$ studies in                         proton-lead collisions at $\sqrt{s_{NN}} = 5.02$~TeV                         and comparisons between ALICE and LHCb results}'' }{}#1[{ALICE and LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-013}{LHCb-CONF-2013-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Combination of results on the rare decays                         $\B^0_{(s)} \to \mumu$ from the CMS and LHCb experiments}'' }{}#1[{CMS and LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-012}{LHCb-CONF-2013-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Updated average $f_{s}/f_{d}$ $b$-hadron production fraction ratio for $7 \tev$ $pp$ collisions}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-011}{LHCb-CONF-2013-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the $\Lb \rightarrow \Lz\eta^{\prime}$ decay at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-010}{LHCb-CONF-2013-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl {\CP and up-down asymmetries in                         $B^{\pm}\to K^{\pm}\pi^{\mp}\pi^{\pm}\gamma$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-009}{LHCb-CONF-2013-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Study of the $J/\psi$ production cross-section                         in proton-lead collisions at $\sqrt{s_{NN}}=5 \tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-008}{LHCb-CONF-2013-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the cross section for                         $Z\rightarrow\mu^{+}\mu^{-}$ production with                         $1.0 \invfb$ of $pp$ collisions at $\sqrt{s}=7 \tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-007}{LHCb-CONF-2013-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl {A measurement of $\gamma$ from a combination of                         $B^\pm \to DK^\pm$ analyses including first                         results using $2 \invfb$ of 2012 data}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-006}{LHCb-CONF-2013-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Graphical comparison of the LHCb measurements of $W$ and $Z$ boson production with ATLAS and CMS}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-005}{LHCb-CONF-2013-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Model-independent measurement of CP violation parameters in $B^\pm \to (K_S^0h^+h^-)_D K^\pm$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-004}{LHCb-CONF-2013-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl {A search for time-integrated \CP violation in $D^0 \to K^-K^+$ and $D^0 \to \pi^-\pi^+$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-003}{LHCb-CONF-2013-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of $\sigma(b\bar{b})$ with inclusive final states}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-002}{LHCb-CONF-2013-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the forward-central $b\bar{b}$ production asymmetry at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-001}{LHCb-CONF-2013-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-034}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First look at the $p$Pb pilot run}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-034}{LHCb-CONF-2012-034}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-033}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Optimization and calibration of the same-side kaon tagging algorithm using hadronic $\Bs$ decays in 2011 data}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-033}{LHCb-CONF-2012-033}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-032}}{\ifthenelse{\boolean{articletitles}}{``\textsl {A measurement of $\gamma$ from a combination of $B^+\to Dh^+$ analyses}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-032}{LHCb-CONF-2012-032}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-031}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Studies of $\Lambda_b^0 \to J/\psi \Lambda$ production in $pp$ collisions at $\sqrt{s}=7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-031}{LHCb-CONF-2012-031}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-030}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the suppressed ADS modes $B^\pm \to [\pi^\pm K^\mp \pi^+\pi^-]_D K^\pm$ and $B^\pm \to [\pi^\pm K^\mp \pi^+\pi^-]_D \pi^\pm$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-030}{LHCb-CONF-2012-030}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-029}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the time-dependent \CP-violation parameters in $B^0_s \to D_s^\mp K^\pm$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-029}{LHCb-CONF-2012-029}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-028}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Evidence for \CP violation in $B \to KK\pi$ and $B \to \pi\pi\pi$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-028}{LHCb-CONF-2012-028}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-027}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the lepton flavour violating and baryon number violating decays $\tau^- \to \antiproton \mu^+ \mu^-$ and $\tau^- \to \proton \mu^- \mu^-$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-027}{LHCb-CONF-2012-027}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-026}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Performance of flavor tagging algorithms optimised for the analysis of $B_s^0 \to J/\psi \phi$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-026}{LHCb-CONF-2012-026}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-025}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Production of $J/\psi$ and $\Upsilon(1S)$, $\Upsilon(2S)$ and $\Upsilon(3S)$~mesons at $\sqrt{s}=8\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-025}{LHCb-CONF-2012-025}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-024}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of $CP$ observables in $B^0\to D K^{*0}$ with $D\to K^+K^-$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-024}{LHCb-CONF-2012-024}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-023}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Branching fraction measurements of $B^0_{d,s}$ decays to $K^0_S h h^{'}$ final states, including first observation of $B^0_s \to K_S K \pi$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-023}{LHCb-CONF-2012-023}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-022}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the flavour-specific \CP violating asymmetry $a_{\mathrm{sl}}^s$ in \Bs decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-022}{LHCb-CONF-2012-022}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-021}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First observation of $B^-\to D^0 K^-\pi^+\pi^-$ decays to \CP even final states}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-021}{LHCb-CONF-2012-021}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-020}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Observation of $\chi_b(3P)$ state at LHCb in pp collisions at $\sqrt{s}=7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-020}{LHCb-CONF-2012-020}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-019}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for $CP$ violation in $D^{0} \to \pi^{-} \pi^{+} \pi^{+} \pi^{-}$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-019}{LHCb-CONF-2012-019}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Evidence for CP violation in $B \to K\pi\pi$ and $B \to KKK$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-018}{LHCb-CONF-2012-018}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the rare decays $B^0_{(s)}\rightarrow\mu\mu$ at the LHC with the ATLAS, CMS and LHCb experiments}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-017}{LHCb-CONF-2012-017}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of jet production in $Z^0/\gamma^*\rightarrow\mu^+\mu^-$ events at LHCb in $\sqrt s = 7\tev$ $pp$ collisions}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-016}{LHCb-CONF-2012-016}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the lepton flavour violating decay $\tau^- \rightarrow \mu^+ \mu^- \mu^-$ }'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-015}{LHCb-CONF-2012-015}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for (Higgs-like) bosons decaying into long-lived exotic particles}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-014}{LHCb-CONF-2012-014}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Inclusive low mass Drell-Yan production in the forward                       region at $\sqrt{s} = 7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-013}{LHCb-CONF-2012-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the forward energy flow in $pp$ collisions                       at $\sqrt{s} = 7\tev$ with the LHCb experiment}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-012}{LHCb-CONF-2012-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the cross-section for $Z^0\rightarrow e^+e^-$ production in $pp$ collisions at $\sqrt{s} = 7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-011}{LHCb-CONF-2012-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the rare decays $B_s^0 \rightarrow \mu^+ \mu^-                        \mu^+ \mu^-$ and $B_d^0 \rightarrow \mu^+ \mu^- \mu^+                       \mu^-$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-010}{LHCb-CONF-2012-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First observations and branching fraction measurements of                       $\overline{B}_s^0$ to double-charm final states}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-009}{LHCb-CONF-2012-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Differential branching fraction and angular analysis of the                       $B^{0} \to K^{*0} \mu^{+}\mu^{-}$ decay}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-008}{LHCb-CONF-2012-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of time-dependent $CP$ violation in charmless                       two-body $B$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-007}{LHCb-CONF-2012-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First observation of $B^+ \rightarrow \pi^+\mu^+\mu^-$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-006}{LHCb-CONF-2012-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the $D^0 \to \mu^+ \mu^-$ decay with $0.9 \invfb$ at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-005}{LHCb-CONF-2012-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the direct $CP$ asymmetry in the $B_d^0\to                       K^{*0}\gamma$ decay}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-004}{LHCb-CONF-2012-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the ratio of branching fractions for $B ^0_s \rightarrow \phi\mu\mu$ and $B ^0_s \rightarrow  J/\psi \phi$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-003}{LHCb-CONF-2012-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Tagged time-dependent angular analysis of $B_s^0 \to                       J/\psi\phi$ decays at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-002}{LHCb-CONF-2012-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the effective $B^0_s \rightarrow K^+ K^-$                       lifetime}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-001}{LHCb-CONF-2012-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-062}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the relative cross-section                       $\sigma(\chi_{c_2})/\sigma(\chi_{c_1})$ of prompt $\chi_c$                       mesons using at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-062}{LHCb-CONF-2011-062}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-061}}{\ifthenelse{\boolean{articletitles}}{``\textsl {A search for time-integrated CP violation in $D^0 \to                       h^-h^+$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-061}{LHCb-CONF-2011-061}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-060}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the masses of the  $\Xi_b^{-}$ and                       $\Omega_b^{-}$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-060}{LHCb-CONF-2011-060}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-059}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Relative branching ratio measurements of charmless                       $B^{\pm}$ decays to three hadrons}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-059}{LHCb-CONF-2011-059}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-058}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurements of the relative branching fractions of the                       $B^{\pm} \to p \bar p K^{\pm}$ decay channel including                       charmonium contributions}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-058}{LHCb-CONF-2011-058}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-057}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurements of the relative and absolute branching                       fractions of the decays $B^0_s\rightarrow D^\mp_s K^\pm$ and                       $B^0_s\rightarrow D^-_s \pi^+$ }'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-057}{LHCb-CONF-2011-057}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-056}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Combination of $\phi_s$ measurements from $B_{s}^{0}\to                       J/\psi\phi$ and $B_{s}^{0}\to J/\psi f_{0}(980)$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-056}{LHCb-CONF-2011-056}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-047}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the rare decay $B^{0}_{s}\to \mu^{+}\mu^{-}$ at                       the LHC with the CMS and LHCb experiments}'' }{}#1[{CMS and LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-047}{LHCb-CONF-2011-047}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-055}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the ratio of branching fractions                       $\mathcal{B}(B_d\to K^{*0}\gamma)/\mathcal{B}(B_s\to                       \phi\gamma)$ with the LHCb experiment at $\sqrt{s}=7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-055}{LHCb-CONF-2011-055}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-054}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the Charm Mixing Parameter $y_{CP}$ in                       Two-Body Charm Decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-054}{LHCb-CONF-2011-054}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-053}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Observations of Orbitally Excited $B_{(s)}^{**}$ Mesons}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-053}{LHCb-CONF-2011-053}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-052}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Study of Triple Product Asymmetries in $B_s \rightarrow                       \phi\phi$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-052}{LHCb-CONF-2011-052}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-051}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of $\phi_s$ in $B_s \to J/\psi f_0(980)$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-051}{LHCb-CONF-2011-051}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-050}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of $\Delta m_s$ in the decay $B^0_s \rightarrow                       D^-_s(K^+K^-\pi^-)\pi^+$ using opposite-side and same-side                       flavour tagging algorithms}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-050}{LHCb-CONF-2011-050}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-049}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Tagged time-dependent angular analysis of $B_s\to                       J/\psi\phi$ decays with 337~pb$^{-1}$ at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-049}{LHCb-CONF-2011-049}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-048}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $B^0_s \to J/\psi K^0_s$ branching                       fraction}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-048}{LHCb-CONF-2011-048}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-046}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $CP$ Violation Parameter                       $\mathcal{A}_{\Gamma}$ in Two-Body Charm Decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-046}{LHCb-CONF-2011-046}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-045}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for $X(4140)$ in $B^+\to J/\psi\phi K^+$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-045}{LHCb-CONF-2011-045}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-044}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Evidence for the suppressed decay                       $B^{\pm}\to(K^{\mp}\pi^{\pm})_{D}K^{\pm}$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-044}{LHCb-CONF-2011-044}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-043}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Inclusive $X(3872)$ production in $pp$ collisions at                       $\sqrt{s}=7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-043}{LHCb-CONF-2011-043}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-042}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Charmless charged two-body $B$ decays at LHCb with 2011                       data}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-042}{LHCb-CONF-2011-042}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-041}}{\ifthenelse{\boolean{articletitles}}{``\textsl {$Z$ cross-section measurement at $\sqrt{s}=7\tev$ using the                       channel $Z \rightarrow\tau\tau$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-041}{LHCb-CONF-2011-041}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-040}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First observation of $B_c^+\to J/\psi \pi^+\pi^-\pi^+$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-040}{LHCb-CONF-2011-040}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-039}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Updated measurements of $W$ and $Z$ production at                       $\sqrt{s} = 7\tev$ with the LHCb experiment}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-039}{LHCb-CONF-2011-039}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-038}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Angular analysis of $B^0\rightarrow K^{*0}\mu^+\mu^-$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-038}{LHCb-CONF-2011-038}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-037}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for the rare decays $B^0_{(s)} \to \mu^{+} \mu^{-}$                       with 300 pb$^{-1}$ at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-037}{LHCb-CONF-2011-037}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-036}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Studies of beauty baryons decaying to $D^{0}p\pi^{-}$ and                       $D^{0}pK^{-}$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-036}{LHCb-CONF-2011-036}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-035}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Analysis of $\overline{B}^0_s\to J/\psi \left(\pi^+\pi^-~{                       \mathrm{ and~}}K^+K^-\right)$ and the first observation of $J/\psi                       f'_2(1525)$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-035}{LHCb-CONF-2011-035}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-034}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Average $f_s/f_d$ b-hadron production fraction for $7\tev$ pp                       collisions}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-034}{LHCb-CONF-2011-034}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-033}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the B$^{\pm}$ production cross-section at                       LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-033}{LHCb-CONF-2011-033}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-031}}{\ifthenelse{\boolean{articletitles}}{``\textsl {A measurement of the ratio of branching fractions:                       $\frac{\mathcal{B}(B^{\pm}\rightarrow D                       K^{\pm})}{\mathcal{B}(B^{\pm}\rightarrow D\pi^{\pm})}$ for                       $D\rightarrow K\pi$, $KK$, $K\pi\pi\pi$ and $K^0_S\pi\pi$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-031}{LHCb-CONF-2011-031}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-030}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the Ratio of Branching Fractions                       $\mathcal{B}\mathrm{(B^{\pm} \rightarrow J/\psi                       \pi^{\pm})/\mathcal{B}\mathrm{(B^{\pm} \rightarrow J/\psi                       K^{\pm})}}$ at $\sqrt{\mathrm{s}}=7\tev$ with the                       LHCb Detector}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-030}{LHCb-CONF-2011-030}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-029}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Time integrated ratio of wrong-sign to right-sign $D^0                       \rightarrow K\pi$ decays in 2010 data at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-029}{LHCb-CONF-2011-029}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-028}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of b-hadron production fractions in $7\tev$                       centre-of-mass energy pp collisions}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-028}{LHCb-CONF-2011-028}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-027}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of $b$-hadron masses with exclusive $J/\psi X$                       decays in 2010 data}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-027}{LHCb-CONF-2011-027}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-026}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $\psi(2S)$ production cross-section at                       $\sqrt{s}=7\tev$ in LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-026}{LHCb-CONF-2011-026}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-025}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Evidence for the decay $B_s^0 \rightarrow J/\psi                       \overline{K}^{*0}$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-025}{LHCb-CONF-2011-025}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-024}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First observations of the Cabibbo-suppressed decays                       $\overline{B}^0\to D^{+}K^{-}\pi^{+}\pi^{-}$ and $B^{-}\to D^{0}                       K^{-}\pi^{+}\pi^{-}$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-024}{LHCb-CONF-2011-024}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-023}}{\ifthenelse{\boolean{articletitles}}{``\textsl {A search for time-integrated $CP$ violation in $D^0                       \rightarrow h^{+}h^{-}$ decays and a measurement of the                       $D^0$ production asymmetry}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-023}{LHCb-CONF-2011-023}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-022}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Central exclusive dimuon production at $\sqrt{s}=7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-022}{LHCb-CONF-2011-022}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-021}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $X$(3872) mass with first LHCb data}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-021}{LHCb-CONF-2011-021}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-019}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First observation of the decay $B^0_s \to K^{*0}                       \overline{K}^{*0}$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-019}{LHCb-CONF-2011-019}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-020}}{\ifthenelse{\boolean{articletitles}}{``\textsl {A measurement of the cross-section ratio                       $\sigma(\chi_{c2})/\sigma(\chi_{c1})$ for prompt $\chi_{c}$                       production at $\sqrt{s} = 7\tev$ in LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-020}{LHCb-CONF-2011-020}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-018}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the effective $B_s^0 \rightarrow K^{+}K^{-}$                       Lifetime}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-018}{LHCb-CONF-2011-018}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-017}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $B_c^+$ to $B^+$ production                       cross-section ratios at $\sqrt{s} = 7\tev$ in LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-017}{LHCb-CONF-2011-017}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-016}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $\Upsilon (1S)$ production                       cross-section at $\sqrt{s} = 7\tev$ in LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-016}{LHCb-CONF-2011-016}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-015}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Inclusive jets and dijets in LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-015}{LHCb-CONF-2011-015}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl {$\mathcal{B}(B^0_s\rightarrow\psi(2S)\phi)/                       \mathcal{B}(B^0_s\rightarrow J/\psi\phi)$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-014}{LHCb-CONF-2011-014}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the relative yields of the decay modes                       $B^0\to D^- \pi^+$, $B^0\to D^- K^+$, $B^0_s \to D^-_s                       \pi^+$, and determination of $f_s/f_d$ for $7\tev$ $pp$                       collisions}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-013}{LHCb-CONF-2011-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl {W and Z production at $\sqrt{s} = 7\tev$ with the LHCb                       experiment}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-012}{LHCb-CONF-2011-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of direct $\mathcal{CP}$ violation in charmless                       charged two-body $B$ decays at LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-011}{LHCb-CONF-2011-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of $\Delta m_d$ in $B^0 \rightarrow                       D^-(K^+\pi^-\pi^-)\pi^+$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-010}{LHCb-CONF-2011-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Observation of double $J/\psi$ production in proton-proton                       collisions at a centre-of-mass energy of $\sqrt{s} = 7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-009}{LHCb-CONF-2011-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl {First observation of the decay $\overline{B}^0_s \to D^0                       K^{*0}$ and measurement of the ratio of branching fractions                       $\frac{\mathcal{B}\left(\overline{B}^0_s \to D^0                       K^{*0}\right)}{\mathcal{B}\left(\overline{B}^0_d \to D^0                       \rho^{0}\right)}$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-008}{LHCb-CONF-2011-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-007}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Improved Measurements of the Cabibbo Favored Decays                       $B_{(s)} \to D_{(s)} \pi\pi\pi$ and $\Lambda_b \to                       \Lambda_{c\pi\pi\pi}$ Branching Fractions}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-007}{LHCb-CONF-2011-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-006}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Tagged time-dependent angular analysis of $B^0_s \to                       J/\psi\phi$ decays with the 2010 LHCb data}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-006}{LHCb-CONF-2011-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-005}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of $\Delta m_s$ in the decay $B^0_s \rightarrow                       D^-_s(K^+K^-\pi^-)(3)\pi$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-005}{LHCb-CONF-2011-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-004}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Search for $CP$ violation in $B^0 \to J/\psi K^0_S$ decays                       with first LHCb data}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-004}{LHCb-CONF-2011-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-003}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Optimization and calibration of the LHCb flavour tagging                       performance using 2010 data}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-003}{LHCb-CONF-2011-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-002}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Flavor-untagged angular analysis of                       $\textrm{B}_\textrm{d}^0\rightarrow J/\psi \textrm{K}^*$                        and  $\textrm{B}_\textrm{s}^0\rightarrow J/\psi\phi$ decays                                }'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-002}{LHCb-CONF-2011-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-001}}{\ifthenelse{\boolean{articletitles}}{``\textsl {$b$-hadron lifetime measurements with exclusive $b\to                       J/\psi X$ decays reconstructed in the 2010 data}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-001}{LHCb-CONF-2011-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-014}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the inclusive $\phi$ cross-section in $pp$                       collisions at $\sqrt{s}=7\tev$ with the LHCb                       experiment}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-014}{LHCb-CONF-2010-014}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-013}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Prompt charm production in $pp$ collisions at $\sqrt{s} =7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-013}{LHCb-CONF-2010-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-012}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurements of $B^0$ mesons production cross-section in pp                       collisions at $\sqrt{s} = 7\tev$ using $B^0 \rightarrow                       D^{*-}\mu^+ \nu_\mu X$ decays}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-012}{LHCb-CONF-2010-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-011}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of prompt $\overline{\Lambda}/\Lambda$ and                       $\overline{\Lambda}/K^{0}_{\mathrm{S}}$ production                       ratios in inelastic non-diffractive pp collisions at                       $\sqrt{s}$ = 0.9 and $7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-011}{LHCb-CONF-2010-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-010}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $J/\psi$ production cross-section at                       $\sqrt{s} = 7\tev$ in LHCb}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-010}{LHCb-CONF-2010-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-009}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Measurement of the $\bar{p}/{p}$ ratio in LHCb at                       $\sqrt{s} = 900\gev$ and $7\tev$}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-009}{LHCb-CONF-2010-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-008}}{\ifthenelse{\boolean{articletitles}}{``\textsl {Prompt $K_S^0$ production in $pp$ collisions at $\sqrt{s}$                       = 900 GeV}'' }{}#1[{LHCb, }\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-008}{LHCb-CONF-2010-008}]}{}%
}}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\LHCbShortCitation}[2][\DefaultLHCbCitationStyle]{{%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-050}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-050}{LHCb-PAPER-2017-050}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-049}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-049}{LHCb-PAPER-2017-049}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-048}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-048}{LHCb-PAPER-2017-048}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-047}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-047}{LHCb-PAPER-2017-047}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-046}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-046}{LHCb-PAPER-2017-046}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-045}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-045}{LHCb-PAPER-2017-045}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-044}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-044}{LHCb-PAPER-2017-044}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-043}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-043}{LHCb-PAPER-2017-043}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-042}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-042}{LHCb-PAPER-2017-042}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-041}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-041}{LHCb-PAPER-2017-041}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-040}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-040}{LHCb-PAPER-2017-040}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-039}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-039}{LHCb-PAPER-2017-039}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-038}}{#1[\href{http://arxiv.org/abs/1710.02867}{arXiv:1710.02867}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-037}}{#1[\href{http://arxiv.org/abs/1710.04921}{arXiv:1710.04921}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-036}}{#1[\href{http://arxiv.org/abs/1709.04247}{arXiv:1709.04247}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-035}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-035}{LHCb-PAPER-2017-035}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-034}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-034}{LHCb-PAPER-2017-034}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-033}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-033}{LHCb-PAPER-2017-033}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-032}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-032}{LHCb-PAPER-2017-032}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-031}}{#1[\href{http://arxiv.org/abs/1710.04111}{arXiv:1710.04111}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-030}}{#1[\href{http://arxiv.org/abs/1709.05855}{arXiv:1709.05855}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-029}}{#1[\href{http://arxiv.org/abs/1709.03944}{arXiv:1709.03944}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-028}}{#1[\href{http://arxiv.org/abs/1709.01301}{arXiv:1709.01301}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-027}}{#1[\href{http://arxiv.org/abs/1711.02505}{arXiv:1711.02505}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-026}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-PAPER-2017-026}{LHCb-PAPER-2017-026}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-025}}{#1[\href{http://arxiv.org/abs/1709.01769}{arXiv:1709.01769}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-024}}{#1[\href{http://arxiv.org/abs/1709.03458}{arXiv:1709.03458}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-023}}{#1[\href{http://arxiv.org/abs/1708.05808}{PRL 119 (2017) 181807}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-022}}{#1[\href{http://arxiv.org/abs/1709.01156}{arXiv:1709.01156}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-021}}{#1[\href{http://arxiv.org/abs/1708.06370}{arXiv:1708.06370}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-020}}{#1[\href{http://arxiv.org/abs/1708.05994}{arXiv:1708.05994}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-019}}{#1[\href{http://arxiv.org/abs/1707.08377}{PRL 119 (2017) 181805}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-018}}{#1[\href{http://arxiv.org/abs/1707.01621}{PRL 119 (2017) 112001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-017}}{#1[\href{http://arxiv.org/abs/1708.08856}{arXiv:1708.08856}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-016}}{#1[\href{http://arxiv.org/abs/1709.01920}{arXiv:1709.01920}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-015}}{#1[\href{http://arxiv.org/abs/1707.02750}{arXiv:1707.02750}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-014}}{#1[\href{http://arxiv.org/abs/1706.07122}{arXiv:1706.07122}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-013}}{#1[\href{http://arxiv.org/abs/1705.05802}{JHEP 08 (2017) 055}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-012}}{#1[\href{http://arxiv.org/abs/1704.07908}{PRL 119 (2017) 041802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-011}}{#1[\href{http://arxiv.org/abs/1704.07900}{PRL 119 (2017) 062001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-010}}{#1[\href{http://arxiv.org/abs/1707.01665}{arXiv:1707.01665}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-009}}{#1[\href{http://arxiv.org/abs/1706.00758}{Eur. Phys. J. C77 (2017) 678}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-008}}{#1[\href{http://arxiv.org/abs/1704.08217}{JHEP 08 (2017) 037}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-007}}{#1[\href{http://arxiv.org/abs/1706.07013}{arXiv:1706.07013}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-006}}{#1[\href{http://arxiv.org/abs/1704.07581}{PRD 96 (2017) 011101}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-005}}{#1[\href{http://arxiv.org/abs/1704.08497}{PRD 96 (2017) 051103}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-004}}{#1[\href{http://arxiv.org/abs/1705.03475}{PRL 119 (2017) 101801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-003}}{#1[\href{http://arxiv.org/abs/1703.02508}{PRL 118 (2017) 251802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-002}}{#1[\href{http://arxiv.org/abs/1703.04639}{PRL 118 (2017) 182001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2017-001}}{#1[\href{http://arxiv.org/abs/1703.05747}{PRL 118 (2017) 191801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-065}}{#1[\href{http://arxiv.org/abs/1705.07332}{arXiv:1705.07332}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-064}}{#1[\href{http://arxiv.org/abs/1701.05116}{PRL 118 (2017) 192001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-063}}{#1[\href{http://arxiv.org/abs/1702.06490}{PRL 118 (2017) 261803}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-062}}{#1[\href{http://arxiv.org/abs/1703.08464}{arXiv:1703.08464}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-061}}{#1[\href{http://arxiv.org/abs/1701.07873}{JHEP 05 (2017) 030}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-060}}{#1[\href{http://arxiv.org/abs/1612.08110}{JHEP 05 (2017) 158}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-059}}{#1[\href{http://arxiv.org/abs/1703.00256}{JHEP 06 (2017) 108}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-058}}{#1[\href{http://arxiv.org/abs/1701.01856}{PRL 118 (2017) 111803}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-057}}{#1[\href{http://arxiv.org/abs/1612.07451}{JHEP 06 (2017) 047}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-056}}{#1[\href{http://arxiv.org/abs/1702.08048}{JHEP 07 (2017) 21}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-055}}{#1[\href{http://arxiv.org/abs/1612.07421}{PRD 95 (2017) 032005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-054}}{#1[\href{http://arxiv.org/abs/1701.05501}{PRD 95 (2017) 052005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-053}}{#1[\href{http://arxiv.org/abs/1701.05274}{PLB 772 (2017) 265}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-052}}{#1[\href{http://arxiv.org/abs/1612.07818}{PRD 95 (2017) 071101}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-051}}{#1[\href{http://arxiv.org/abs/1612.06116}{JHEP 03 (2017) 036}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-050}}{#1[\href{http://arxiv.org/abs/1612.02244}{PRL 118 (2017) 071801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-049}}{#1[\href{http://arxiv.org/abs/1701.08705}{JHEP 04 (2017) 029}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-048}}{#1[\href{http://arxiv.org/abs/1611.07805}{JHEP 04 (2017) 162}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-047}}{#1[\href{http://arxiv.org/abs/1612.00945}{Eur. Phys. J. C77 (2017) 224}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-046}}{#1[\href{http://arxiv.org/abs/1610.03666}{PLB 764 (2016) 233}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-045}}{#1[\href{http://arxiv.org/abs/1612.06764}{Eur. Phys. J. C77 (2017) 161}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-044}}{#1[\href{http://arxiv.org/abs/1612.03207}{PLB 769 (2017) 345}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-043}}{#1[\href{http://arxiv.org/abs/1611.07704}{JHEP 03 (2017) 001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-042}}{#1[\href{http://arxiv.org/abs/1610.02230}{JHEP 06 (2017) 147}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-041}}{#1[\href{http://arxiv.org/abs/1701.01871}{PLB 771 (2017) 21}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-040}}{#1[\href{http://arxiv.org/abs/1610.01383}{Eur. Phys. J. C77 (2016) 72}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-039}}{#1[\href{http://arxiv.org/abs/1610.06019}{Eur. Phys. J. C77 (2017) 238}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-038}}{#1[\href{http://arxiv.org/abs/1610.08142}{PLB 767 (2017) 110}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-037}}{#1[\href{http://arxiv.org/abs/1608.06620}{PRL 117 (2016) 261801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-036}}{#1[\href{http://arxiv.org/abs/1610.08288}{PRL 118 (2017) 081801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-035}}{#1[\href{http://arxiv.org/abs/1610.09476}{PLB 767 (2017) 177}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-034}}{#1[\href{http://arxiv.org/abs/1609.02032}{PRL 118 (2017) 021801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-033}}{#1[\href{http://arxiv.org/abs/1611.06143}{PRD 95 (2017) 052004}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-032}}{#1[\href{http://arxiv.org/abs/1611.03076}{JHEP 12 (2016) 087}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-031}}{#1[\href{http://arxiv.org/abs/1612.05140}{PRL 118 (2017) 052002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-030}}{#1[\href{http://arxiv.org/abs/1609.05216}{Nature Physics 13 (2017) 391}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-029}}{#1[\href{http://arxiv.org/abs/1608.00435}{PRL 117 (2016) 152003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-028}}{#1[\href{http://arxiv.org/abs/1610.05187}{PRD 95 (2017) 012006}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-027}}{#1[\href{http://arxiv.org/abs/1608.04855}{PLB 762 (2016) 253}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-026}}{#1[\href{http://arxiv.org/abs/1608.01289}{PRD 94 (2016) 072001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-025}}{#1[\href{http://arxiv.org/abs/1609.04736}{JHEP 12 (2016) 065}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-024}}{#1[\href{http://arxiv.org/abs/1608.01484}{JHEP 10 (2016) 030}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-023}}{#1[\href{http://arxiv.org/abs/1608.01478}{PLB 765 (2017) 307}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-022}}{#1[\href{http://arxiv.org/abs/1607.06134}{PRD 94 (2016) 091102(R)}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-021}}{#1[\href{http://arxiv.org/abs/1607.06495}{JHEP 09 (2016) 136}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-020}}{#1[\href{http://arxiv.org/abs/1607.06823}{JHEP 09 (2016) 153}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-019}}{#1[\href{http://arxiv.org/abs/1606.07898}{PRD 95 (2016) 012002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-018}}{#1[\href{http://arxiv.org/abs/1606.07895}{PRL 118 (2016) 022003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-017}}{#1[\href{http://arxiv.org/abs/1607.06314}{PLB 762 (2016) 484}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-016}}{#1[\href{http://arxiv.org/abs/1607.06446}{PLB 769 (2017) 305}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-015}}{#1[\href{http://arxiv.org/abs/1606.06999}{PRL 117 (2016) 082003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-014}}{#1[\href{http://arxiv.org/abs/1609.03124}{Eur. Phys. J. C76 (2016) 664}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-013}}{#1[\href{http://arxiv.org/abs/1605.09768}{PRL 117 (2016) 061803}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-012}}{#1[\href{http://arxiv.org/abs/1606.04731}{JHEP 11 (2016) 047}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-011}}{#1[\href{http://arxiv.org/abs/1605.00951}{JHEP 05 (2016) 131}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-010}}{#1[\href{http://arxiv.org/abs/1604.03896}{JHEP 05 (2016) 161}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-009}}{#1[\href{http://arxiv.org/abs/1604.05708}{PRL 117 (2016) 082002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-008}}{#1[\href{http://arxiv.org/abs/1604.01412}{PRD 93 (2016) 092007}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-007}}{#1[\href{http://arxiv.org/abs/1605.01082}{JHEP 08 (2016) 137}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-006}}{#1[\href{http://arxiv.org/abs/1604.01525}{JHEP 06 (2016) 131}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-005}}{#1[\href{http://arxiv.org/abs/1603.04804}{PRL 116 (2016) 241601}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-004}}{#1[\href{http://arxiv.org/abs/1603.00413}{JHEP 05 (2016) 081}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-003}}{#1[\href{http://arxiv.org/abs/1603.08993}{PLB 760 (2016) 117}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-002}}{#1[\href{http://arxiv.org/abs/1603.02870}{PLB 759 (2016) 282}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2016-001}}{#1[\href{http://arxiv.org/abs/1603.07037}{PLB 759 (2016) 313}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-060}}{#1[\href{http://arxiv.org/abs/1603.06961}{JHEP 05 (2016) 132}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-059}}{#1[\href{http://arxiv.org/abs/1602.03455}{PRD 93 (2016) 112018}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-058}}{#1[\href{http://arxiv.org/abs/1601.07878}{JHEP 03 (2016) 133}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-057}}{#1[\href{http://arxiv.org/abs/1602.07224}{PRL 116 (2016) 241801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-056}}{#1[\href{http://arxiv.org/abs/1602.07252}{JINST 11 (2016) P05010}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-055}}{#1[\href{http://arxiv.org/abs/1602.03160}{PRL 116 (2016) 191601}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-054}}{#1[\href{http://arxiv.org/abs/1512.02494}{PRD 93 (2016) 051101(R)}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-053}}{#1[\href{http://arxiv.org/abs/1602.07543}{PRD 93 (2016) 092008}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-052}}{#1[\href{http://arxiv.org/abs/1601.01495}{JHEP 02 (2016) 133}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-051}}{#1[\href{http://arxiv.org/abs/1512.04442}{JHEP 02 (2016) 104}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-050}}{#1[\href{http://arxiv.org/abs/1603.02408}{PRL 116 (2016) 161802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-049}}{#1[\href{http://arxiv.org/abs/1511.08039}{JHEP 01 (2016) 155}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-048}}{#1[\href{http://arxiv.org/abs/1512.00322}{PLB 754 (2016) 167}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-047}}{#1[\href{http://arxiv.org/abs/1510.03829}{PRL 115 (2015) 241801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-046}}{#1[\href{http://arxiv.org/abs/1510.05949}{JHEP 07 (2016) 052}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-045}}{#1[\href{http://arxiv.org/abs/1509.02372}{JHEP 11 (2015) 103}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-044}}{#1[\href{http://arxiv.org/abs/1510.04866}{PRD 92 (2015) 112002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-043}}{#1[\href{http://arxiv.org/abs/1510.08367}{PLB 757 (2016) 558}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-042}}{#1[\href{http://arxiv.org/abs/1510.01664}{JHEP 04 (2016) 033}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-041}}{#1[\href{http://arxiv.org/abs/1510.01707}{JHEP 03 (2016) 159}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-040}}{#1[\href{http://arxiv.org/abs/1512.00439}{PLB 762 (2016) 473}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-039}}{#1[\href{http://arxiv.org/abs/1509.07645}{JHEP 11 (2015) 190}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-038}}{#1[\href{http://arxiv.org/abs/1510.01951}{PRD 92 (2015) 112009}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-037}}{#1[\href{http://arxiv.org/abs/1509.00771}{JHEP 10 (2015) 172}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-036}}{#1[\href{http://arxiv.org/abs/1508.04094}{PRL 115 (2015) 161802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-035}}{#1[\href{http://arxiv.org/abs/1509.00414}{JHEP 10 (2015) 034}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-034}}{#1[\href{http://arxiv.org/abs/1509.00400}{JHEP 11 (2015) 082}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-033}}{#1[\href{http://arxiv.org/abs/1601.05284}{JHEP 03 (2016) 040}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-032}}{#1[\href{http://arxiv.org/abs/1509.00292}{Chin. Phys. C 40 (2016) 011001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-031}}{#1[\href{http://arxiv.org/abs/1604.03475}{Eur. Phys. J. C76 (2016) 412}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-030}}{#1[\href{http://arxiv.org/abs/1508.06087}{JHEP 10 (2015) 055}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-029}}{#1[\href{http://arxiv.org/abs/1507.03414}{PRL 115 (2015) 072001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-028}}{#1[\href{http://arxiv.org/abs/1508.00788}{JHEP 10 (2015) 053}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-027}}{#1[\href{http://arxiv.org/abs/1507.07892}{JINST 10 (2015) P10005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-026}}{#1[\href{http://arxiv.org/abs/1509.06628}{PRD 93 (2016) 052018}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-025}}{#1[\href{http://arxiv.org/abs/1506.08614}{PRL 115 (2015) 111803}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-024}}{#1[\href{http://arxiv.org/abs/1507.03516}{PRD 92 (2015) 057007}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-023}}{#1[\href{http://arxiv.org/abs/1506.08777}{JHEP 09 (2015) 179}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-022}}{#1[\href{http://arxiv.org/abs/1506.00903}{PRL 115 (2015) 112001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-021}}{#1[\href{http://arxiv.org/abs/1505.04051}{PRD 92 (2015) 052012}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-020}}{#1[\href{http://arxiv.org/abs/1505.07044}{PRD 92 (2015) 112005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-019}}{#1[\href{http://arxiv.org/abs/1505.03295}{JHEP 09 (2015) 006}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-018}}{#1[\href{http://arxiv.org/abs/1506.08634}{JHEP 01 (2016) 012}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-017}}{#1[\href{http://arxiv.org/abs/1505.01505}{PRD 92 (2015) 012012}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-016}}{#1[\href{http://arxiv.org/abs/1504.07670}{JINST 10 (2015) P06013}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-015}}{#1[\href{http://arxiv.org/abs/1504.06339}{PRD 92 (2015) 011102(R)}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-014}}{#1[\href{http://arxiv.org/abs/1504.05442}{PRD 91 (2015) 112014}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-013}}{#1[\href{http://arxiv.org/abs/1504.01568}{Nature Physics 11 (2015) 743}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-012}}{#1[\href{http://arxiv.org/abs/1505.01654}{JHEP 08 (2015) 005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-011}}{#1[\href{http://arxiv.org/abs/1505.08139}{JHEP 09 (2015) 084}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-010}}{#1[\href{http://arxiv.org/abs/1503.07112}{PLB 747 (2015) 484}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-009}}{#1[\href{http://arxiv.org/abs/1503.07138}{JHEP 06 (2015) 115}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-008}}{#1[\href{http://arxiv.org/abs/1503.09086}{JHEP 06 (2015) 130}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-007}}{#1[\href{http://arxiv.org/abs/1503.02995}{PRD 91 (2015) 092002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-006}}{#1[\href{http://arxiv.org/abs/1503.07770}{PLB 747 (2015) 468}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-005}}{#1[\href{http://arxiv.org/abs/1503.07055}{JHEP 06 (2015) 131}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-004}}{#1[\href{http://arxiv.org/abs/1503.07089}{PRL 115 (2015) 031601}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-003}}{#1[\href{http://arxiv.org/abs/1503.00963}{JHEP 05 (2015) 109}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-002}}{#1[\href{http://arxiv.org/abs/1506.09173}{Eur. Phys. J. C75 (2015) 595}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2015-001}}{#1[\href{http://arxiv.org/abs/1505.07024}{JHEP 08 (2015) 039}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-070}}{#1[\href{http://arxiv.org/abs/1505.01710}{PRD 92 (2015) 032002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-069}}{#1[\href{http://arxiv.org/abs/1501.06777}{JHEP 04 (2015) 043}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-068}}{#1[\href{http://arxiv.org/abs/1503.05362}{JHEP 07 (2015) 166}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-067}}{#1[\href{http://arxiv.org/abs/1502.02638}{JHEP 04 (2015) 024}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-066}}{#1[\href{http://arxiv.org/abs/1501.03038}{JHEP 04 (2015) 064}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-065}}{#1[\href{http://arxiv.org/abs/1503.07483}{PRL 115 (2015) 051801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-064}}{#1[\href{http://arxiv.org/abs/1412.7654}{JHEP 02 (2015) 029}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-063}}{#1[\href{http://arxiv.org/abs/1412.6433}{PLB 743 (2015) 46}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-062}}{#1[\href{http://arxiv.org/abs/1412.3021}{Eur. Phys. J. C75 (2015) 152}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-061}}{#1[\href{http://arxiv.org/abs/1411.4849}{PRL 114 (2015) 062004}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-060}}{#1[\href{http://arxiv.org/abs/1411.6899}{PLB 742 (2015) 29}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-059}}{#1[\href{http://arxiv.org/abs/1411.3104}{PRL 114 (2015) 041801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-058}}{#1[\href{http://arxiv.org/abs/1411.1634}{PLB 742 (2015) 38}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-057}}{#1[\href{http://arxiv.org/abs/1412.2500}{JHEP 02 (2015) 029}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-056}}{#1[\href{http://arxiv.org/abs/1411.0943}{JHEP 01 (2015) 024}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-055}}{#1[\href{http://arxiv.org/abs/1411.1264}{JHEP 01 (2015) 064}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-054}}{#1[\href{http://arxiv.org/abs/1410.4170}{PLB 740 (2015) 158}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-053}}{#1[\href{http://arxiv.org/abs/1409.8586}{PRL 114 (2015) 041601}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-052}}{#1[\href{http://arxiv.org/abs/1409.8548}{JHEP 02 (2015) 121}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-051}}{#1[\href{http://arxiv.org/abs/1409.4619}{PRL 113 (2014) 211801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-050}}{#1[\href{http://arxiv.org/abs/1411.2943}{PRL 114 (2015) 132001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-049}}{#1[\href{http://arxiv.org/abs/1411.4413}{Nature 522 (2015) 68}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-048}}{#1[\href{http://arxiv.org/abs/1409.8568}{PRL 113 (2014) 242002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-047}}{#1[\href{http://arxiv.org/abs/1410.0149}{JINST 9 (2014) P12005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-046}}{#1[\href{http://arxiv.org/abs/1408.1299}{JHEP 10 (2014) 005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-045}}{#1[\href{http://arxiv.org/abs/1408.4368}{PLB 739 (2015) 1}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-044}}{#1[\href{http://arxiv.org/abs/1408.5373}{PRD 90 (2014) 112004}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-043}}{#1[\href{http://arxiv.org/abs/1407.7704}{New J. Phys. 16 (2014) 123001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-042}}{#1[\href{http://arxiv.org/abs/1408.0275}{PLB 739 (2014) 218}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-041}}{#1[\href{http://arxiv.org/abs/1408.2748}{JHEP 10 (2014) 097}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-040}}{#1[\href{http://arxiv.org/abs/1409.1408}{JHEP 10 (2014) 088}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-039}}{#1[\href{http://arxiv.org/abs/1408.0971}{PRL 113 (2014) 152003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-038}}{#1[\href{http://arxiv.org/abs/1407.6127}{JHEP 11 (2014) 060}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-037}}{#1[\href{http://arxiv.org/abs/1407.5873}{PRL 113 (2014) 172001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-036}}{#1[\href{http://arxiv.org/abs/1407.7712}{PRD 90 (2014) 072003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-035}}{#1[\href{http://arxiv.org/abs/1407.7574}{PRL 113 (2014) 162001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-034}}{#1[\href{http://arxiv.org/abs/1407.5907}{PRL 113 (2014) 141801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-033}}{#1[\href{http://arxiv.org/abs/1408.4354}{JHEP 12 (2014) 079}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-032}}{#1[\href{http://arxiv.org/abs/1408.0978}{JHEP 09 (2014) 177}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-031}}{#1[\href{http://arxiv.org/abs/1407.7734}{Eur. Phys. J. C74 (2014) 3092}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-030}}{#1[\href{http://arxiv.org/abs/1408.1137}{JHEP 10 (2014) 064}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-029}}{#1[\href{http://arxiv.org/abs/1409.3612}{Eur. Phys. J. C75 (2015) 311}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-028}}{#1[\href{http://arxiv.org/abs/1407.8136}{PRD 90 (2014) 112002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-027}}{#1[\href{http://arxiv.org/abs/1407.5973}{J. Phys. G41 (2014) 115002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-026}}{#1[\href{http://arxiv.org/abs/1407.2222}{PRD 90 (2014) 052011}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-025}}{#1[\href{http://arxiv.org/abs/1407.2126}{PRD 90 (2014) 032009}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-024}}{#1[\href{http://arxiv.org/abs/1406.6482}{PRL 113 (2014) 151601}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-023}}{#1[\href{http://arxiv.org/abs/1406.4789}{PRL 113 (2014) 082003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-022}}{#1[\href{http://arxiv.org/abs/1406.2885}{JHEP 09 (2014) 030}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-021}}{#1[\href{http://arxiv.org/abs/1405.7223}{PRL 113 (2014) 032001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-020}}{#1[\href{http://arxiv.org/abs/1406.0755}{JHEP 07 (2014) 103}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-019}}{#1[\href{http://arxiv.org/abs/1405.4140}{PLB 736 (2014) 186}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-018}}{#1[\href{http://arxiv.org/abs/1406.2624}{JHEP 10 (2014) 025}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-017}}{#1[\href{http://arxiv.org/abs/1407.6211}{Nucl. Phys. B888 (2014) 169}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-016}}{#1[\href{http://arxiv.org/abs/1405.3219}{JHEP 07 (2014) 140}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-015}}{#1[\href{http://arxiv.org/abs/1405.5152}{JHEP 07 (2014) 094}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-014}}{#1[\href{http://arxiv.org/abs/1404.1903}{PRL 112 (2014) 222002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-013}}{#1[\href{http://arxiv.org/abs/1405.2797}{JHEP 07 (2014) 041}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-012}}{#1[\href{http://arxiv.org/abs/1404.5673}{PRD 90 (2014) 012003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-011}}{#1[\href{http://arxiv.org/abs/1406.7204}{PLB 736 (2014) 446}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-010}}{#1[\href{http://arxiv.org/abs/1405.1543}{PLB 736 (2014) 154}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-009}}{#1[\href{http://arxiv.org/abs/1404.0287}{JHEP 05 (2014) 148}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-008}}{#1[\href{http://arxiv.org/abs/1404.0275}{Nucl. Phys. B886 (2014) 665}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-007}}{#1[\href{http://arxiv.org/abs/1403.8045}{JHEP 05 (2014) 082}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-006}}{#1[\href{http://arxiv.org/abs/1403.8044}{JHEP 06 (2014) 133}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-005}}{#1[\href{http://arxiv.org/abs/1403.2888}{JHEP 05 (2014) 069}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-004}}{#1[\href{http://arxiv.org/abs/1405.6842}{JHEP 08 (2014) 143}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-003}}{#1[\href{http://arxiv.org/abs/1402.6242}{PLB 734 (2014) 122}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-002}}{#1[\href{http://arxiv.org/abs/1403.3606}{PRL 112 (2014) 202001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2014-001}}{#1[\href{http://arxiv.org/abs/1402.6852}{PRL 112 (2014) 161801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-070}}{#1[\href{http://arxiv.org/abs/1402.4430}{Eur. Phys. J. C74 (2014) 2888}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-069}}{#1[\href{http://arxiv.org/abs/1402.6248}{PRD 89 (2014) 092006}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-068}}{#1[\href{http://arxiv.org/abs/1402.2982}{PLB 733 (2014) 36}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-067}}{#1[\href{http://arxiv.org/abs/1403.1339}{Eur. Phys. J. C74 (2014) 2872}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-066}}{#1[\href{http://arxiv.org/abs/1402.2539}{Eur. Phys. J. C74 (2014) 2835}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-065}}{#1[\href{http://arxiv.org/abs/1402.2554}{JHEP 04 (2014) 114}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-064}}{#1[\href{http://arxiv.org/abs/1401.5361}{PRL 112 (2014) 131802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-063}}{#1[\href{http://arxiv.org/abs/1401.6932}{Eur. Phys. J. C74 (2014) 2839}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-062}}{#1[\href{http://arxiv.org/abs/1401.3245}{JHEP 04 (2014) 091}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-061}}{#1[\href{http://arxiv.org/abs/1402.0770}{JHEP 04 (2014) 087}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-060}}{#1[\href{http://arxiv.org/abs/1312.1217}{PRL 112 (2014) 111802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-059}}{#1[\href{http://arxiv.org/abs/1401.3288}{J. Phys. G41 (2014) 055002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-058}}{#1[\href{http://arxiv.org/abs/1310.8197}{JHEP 01 (2014) 033}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-057}}{#1[\href{http://arxiv.org/abs/1310.7953}{PLB 728 (2014) 585}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-056}}{#1[\href{http://arxiv.org/abs/1311.4823}{PRD 89 (2014) 032001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-055}}{#1[\href{http://arxiv.org/abs/1310.2145}{PRL 112 (2014) 091802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-054}}{#1[\href{http://arxiv.org/abs/1310.7201}{PRL 112 (2014) 041801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-053}}{#1[\href{http://arxiv.org/abs/1309.6534}{PRL 111 (2013) 251801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-052}}{#1[\href{http://arxiv.org/abs/1308.6729}{JHEP 02 (2014) 072}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-051}}{#1[\href{http://arxiv.org/abs/1310.4740}{PRL 112 (2014) 011801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-050}}{#1[\href{http://arxiv.org/abs/1310.2535}{PLB 728 (2014) 234}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-049}}{#1[\href{http://arxiv.org/abs/1310.2538}{JHEP 12 (2013) 090}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-048}}{#1[\href{http://arxiv.org/abs/1309.3742}{PLB 728 (2014) 85}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-047}}{#1[\href{http://arxiv.org/abs/1309.0587}{JHEP 11 (2013) 094}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-046}}{#1[\href{http://arxiv.org/abs/1307.5024}{PRL 111 (2013) 101805}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-045}}{#1[\href{http://arxiv.org/abs/1308.5916}{PRD 88 (2013) 072005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-044}}{#1[\href{http://arxiv.org/abs/1308.4544}{PRL 111 (2013) 181801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-043}}{#1[\href{http://arxiv.org/abs/1308.1340}{PRL 111 (2013) 151801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-042}}{#1[\href{http://arxiv.org/abs/1307.7648}{JHEP 10 (2013) 143}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-041}}{#1[\href{http://arxiv.org/abs/1308.3189}{PLB 726 (2013) 623}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-040}}{#1[\href{http://arxiv.org/abs/1308.1428}{JHEP 10 (2013) 183}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-039}}{#1[\href{http://arxiv.org/abs/1307.7595}{PRL 111 (2013) 112003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-038}}{#1[\href{http://arxiv.org/abs/1308.0961}{JHEP 10 (2013) 005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-037}}{#1[\href{http://arxiv.org/abs/1308.1707}{PRL 111 (2013) 191801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-036}}{#1[\href{http://arxiv.org/abs/1308.1302}{Eur. Phys. J. C73 (2013) 2655}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-035}}{#1[\href{http://arxiv.org/abs/1308.4583}{PLB 727 (2013) 403}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-034}}{#1[\href{http://arxiv.org/abs/1308.1277}{PLB 726 (2013) 646}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-033}}{#1[\href{http://arxiv.org/abs/1308.1048}{PLB 728 (2014) 607}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-032}}{#1[\href{http://arxiv.org/abs/1307.2476}{PRL 111 (2013) 102003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-031}}{#1[\href{http://arxiv.org/abs/1307.6165}{PRD 88 (2013) 052015}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-030}}{#1[\href{http://arxiv.org/abs/1307.4889}{PRL 111 (2013) 141801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-029}}{#1[\href{http://arxiv.org/abs/1306.4489}{JHEP 09 (2013) 006}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-028}}{#1[\href{http://arxiv.org/abs/1307.4285}{JHEP 10 (2013) 115}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-027}}{#1[\href{http://arxiv.org/abs/1306.1246}{PRL 111 (2013) 101801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-026}}{#1[\href{http://arxiv.org/abs/1307.4556}{JHEP 09 (2013) 145}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-025}}{#1[\href{http://arxiv.org/abs/1306.2577}{PLB 725 (2013) 25}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-024}}{#1[\href{http://arxiv.org/abs/1305.6511}{Nucl. Phys. B874 (2013) 663}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-023}}{#1[\href{http://arxiv.org/abs/1307.2782}{PRD 88 (2013) 052002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-022}}{#1[\href{http://arxiv.org/abs/1304.6317}{PRD 87 (2013) 112009}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-021}}{#1[\href{http://arxiv.org/abs/1306.6723}{JHEP 09 (2013) 075}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-020}}{#1[\href{http://arxiv.org/abs/1305.2050}{PLB 726 (2013) 151}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-019}}{#1[\href{http://arxiv.org/abs/1304.6325}{JHEP 08 (2013) 131}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-018}}{#1[\href{http://arxiv.org/abs/1304.6173}{PRL 110 (2013) 221601}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-017}}{#1[\href{http://arxiv.org/abs/1305.2168}{JHEP 07 (2013) 084}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-016}}{#1[\href{http://arxiv.org/abs/1304.6977}{JHEP 06 (2013) 064}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-015}}{#1[\href{http://arxiv.org/abs/1304.4500}{Nucl. Phys. B873 (2013) 275-292}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-014}}{#1[\href{http://arxiv.org/abs/1304.4518}{PLB 724 (2013) 36}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-013}}{#1[\href{http://arxiv.org/abs/1305.5059}{PLB 725 (2013) 15}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-012}}{#1[\href{http://arxiv.org/abs/1306.2239}{JHEP 11 (2013) 092}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-011}}{#1[\href{http://arxiv.org/abs/1304.6865}{JHEP 06 (2013) 065}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-010}}{#1[\href{http://arxiv.org/abs/1304.4530}{PRD 87 (2013) 112012}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-009}}{#1[\href{http://arxiv.org/abs/1304.2591}{JHEP 05 (2013) 132}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-008}}{#1[\href{http://arxiv.org/abs/1307.6379}{Eur. Phys. J. C73 (2013) 2631}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-007}}{#1[\href{http://arxiv.org/abs/1303.7125}{PRL 110 (2013) 241802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-006}}{#1[\href{http://arxiv.org/abs/1304.4741}{New J. Phys. 15 (2013) 053021}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-005}}{#1[\href{http://arxiv.org/abs/1304.3035}{JHEP 05 (2013) 159}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-004}}{#1[\href{http://arxiv.org/abs/1306.3663}{JHEP 08 (2013) 117}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-003}}{#1[\href{http://arxiv.org/abs/1303.2614}{PLB 723 (2013) 33}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-002}}{#1[\href{http://arxiv.org/abs/1304.2600}{PRD 87 (2013) 112010}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2013-001}}{#1[\href{http://arxiv.org/abs/1302.6269}{PRL 110 (2013) 222001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-057}}{#1[\href{http://arxiv.org/abs/1302.5578}{PLB 724 (2013) 27}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-056}}{#1[\href{http://arxiv.org/abs/1302.6446}{PRD 87 (2013) 071101(R)}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-055}}{#1[\href{http://arxiv.org/abs/1303.4646}{PLB 723 (2013) 44}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-054}}{#1[\href{http://arxiv.org/abs/1303.1737}{PRD 87 (2013) 071103(R)}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-053}}{#1[\href{http://arxiv.org/abs/1302.6354}{Nucl. Phys. B871 (2013) 403 - 419}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-052}}{#1[\href{http://arxiv.org/abs/1303.4906}{JHEP 06 (2013) 112}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-051}}{#1[\href{http://arxiv.org/abs/1304.6365}{PLB 724 (2013) 203}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-050}}{#1[\href{http://arxiv.org/abs/1302.5854}{PRD 87 (2013) 092007}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-049}}{#1[\href{http://arxiv.org/abs/1303.1092}{PRL 110 (2013) 211801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-048}}{#1[\href{http://arxiv.org/abs/1302.1072}{PRL 110 (2013) 182001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-047}}{#1[\href{http://arxiv.org/abs/1303.7133}{Eur. Phys. J. C73 (2013) 2462}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-046}}{#1[\href{http://arxiv.org/abs/1303.6861}{PRD 87 (2013) 092001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-045}}{#1[\href{http://arxiv.org/abs/1301.5347}{PRD 87 (2013) 052001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-044}}{#1[\href{http://arxiv.org/abs/1301.7084}{J. Phys. G40 (2013) 045001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-043}}{#1[\href{http://arxiv.org/abs/1211.2674}{PRL 110 (2013) 021801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-042}}{#1[\href{http://arxiv.org/abs/1212.5205}{JHEP 03 (2013) 067}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-041}}{#1[\href{http://arxiv.org/abs/1302.2864}{Nucl. Phys. B871 (2013) 1}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-040}}{#1[\href{http://arxiv.org/abs/1302.1213}{PRD 87 (2013) 072004}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-039}}{#1[\href{http://arxiv.org/abs/1212.1045}{JHEP 02 (2013) 041}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-038}}{#1[\href{http://arxiv.org/abs/1211.1230}{PRL 110 (2013) 101802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-037}}{#1[\href{http://arxiv.org/abs/1301.5286}{JHEP 04 (2013) 001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-036}}{#1[\href{http://arxiv.org/abs/1212.4620}{JHEP 02 (2013) 106}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-035}}{#1[\href{http://arxiv.org/abs/1211.6093}{PLB 721 (2013) 24}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-034}}{#1[\href{http://arxiv.org/abs/1212.4755}{Eur. Phys. J. C73 (2013) 2421}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-033}}{#1[\href{http://arxiv.org/abs/1211.1541}{PRD 86 (2012) 112005}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-032}}{#1[\href{http://arxiv.org/abs/1210.6750}{PLB 719 (2013) 318}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-031}}{#1[\href{http://arxiv.org/abs/1208.3355}{Eur. Phys. J. C73 (2013) 2373}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-030}}{#1[\href{http://arxiv.org/abs/1211.5994}{PRL 110 (2013) 151803}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-029}}{#1[\href{http://arxiv.org/abs/1210.6289}{JHEP 01 (2013) 111}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-028}}{#1[\href{http://arxiv.org/abs/1209.5634}{PRL 109 (2012) 232001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-027}}{#1[\href{http://arxiv.org/abs/1209.5869}{PLB 718 (2012) 43-55}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-026}}{#1[\href{http://arxiv.org/abs/1210.4112}{PLB 718 (2013) 902-909}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-025}}{#1[\href{http://arxiv.org/abs/1210.1089}{JHEP 02 (2013) 043}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-024}}{#1[\href{http://arxiv.org/abs/1209.4284}{JHEP 02 (2013) 105}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-023}}{#1[\href{http://arxiv.org/abs/1209.4029}{JHEP 01 (2013) 090}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-022}}{#1[\href{http://arxiv.org/abs/1210.2631}{Nucl. Phys. B867 (2013) 547-566}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-021}}{#1[\href{http://arxiv.org/abs/1210.4492}{PRL 110 (2013) 031801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-020}}{#1[\href{http://arxiv.org/abs/1210.2645}{JHEP 12 (2012) 125}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-019}}{#1[\href{http://arxiv.org/abs/1209.0313}{Nucl. Phys. B867 (2013) 1-18}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-018}}{#1[\href{http://arxiv.org/abs/1207.5991}{PRL 109 (2012) 131801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-017}}{#1[\href{http://arxiv.org/abs/1207.0878}{PRL 109 (2012) 152002}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-016}}{#1[\href{http://arxiv.org/abs/1207.6016}{JHEP 10 (2012) 151}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-015}}{#1[\href{http://arxiv.org/abs/1209.0282}{JHEP 11 (2012) 031}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-014}}{#1[\href{http://arxiv.org/abs/1208.0738}{PRD 86 (2012) 071102(R)}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-013}}{#1[\href{http://arxiv.org/abs/1207.5993}{PLB 716 (2012) 393-400}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-012}}{#1[\href{http://arxiv.org/abs/1205.3452}{PRL 109 (2012) 172003}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-011}}{#1[\href{http://arxiv.org/abs/1205.3422}{JHEP 07 (2012) 133}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-010}}{#1[\href{http://arxiv.org/abs/1205.0918}{Eur. Phys. J. C72 (2012) 2118}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-009}}{#1[\href{http://arxiv.org/abs/1205.0897}{PLB 713 (2012) 186-195}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-008}}{#1[\href{http://arxiv.org/abs/1204.1620}{JHEP 06 (2012) 058}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-007}}{#1[\href{http://arxiv.org/abs/1203.4493}{PRL 108 (2012) 231801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-006}}{#1[\href{http://arxiv.org/abs/1204.5675}{PLB 713 (2012) 378-386}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-005}}{#1[\href{http://arxiv.org/abs/1204.5643}{PRD 86 (2012) 052006}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-004}}{#1[\href{http://arxiv.org/abs/1204.2813}{PLB 713 (2012) 369-377}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-003}}{#1[\href{http://arxiv.org/abs/1205.0975}{JHEP 06 (2012) 141}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-002}}{#1[\href{http://arxiv.org/abs/1206.2794}{JHEP 10 (2012) 037}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2012-001}}{#1[\href{http://arxiv.org/abs/1203.3662}{PLB 712 (2012) 203}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-045}}{#1[\href{http://arxiv.org/abs/1204.1258}{Eur. Phys. J. C72 (2012) 2100}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-044}}{#1[\href{http://arxiv.org/abs/1204.0079}{PRL 108 (2012) 251802}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-043}}{#1[\href{http://arxiv.org/abs/1202.4812}{JHEP 04 (2012) 093}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-042}}{#1[\href{http://arxiv.org/abs/1202.6267}{PRD 85 (2012) 112013}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-041}}{#1[\href{http://arxiv.org/abs/1205.0934}{PLB 713 (2012) 172-179}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-040}}{#1[\href{http://arxiv.org/abs/1201.4402}{PRL 108 (2012) 161801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-038}}{#1[\href{http://arxiv.org/abs/1201.5600}{PRD 85 (2012) 112004}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-037}}{#1[\href{http://arxiv.org/abs/1206.5160}{Eur. Phys. J. C72 (2012) 2168}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-036}}{#1[\href{http://arxiv.org/abs/1202.6579}{Eur. Phys. J. C72 (2012) 2025}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-035}}{#1[\href{http://arxiv.org/abs/1112.4896}{PLB 708 (2012) 241}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-034}}{#1[\href{http://arxiv.org/abs/1112.5310}{Eur. Phys. J. C72 (2012) 1972}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-033}}{#1[\href{http://arxiv.org/abs/1202.5087}{PRD 85 (2012) 091103(R)}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-032}}{#1[\href{http://arxiv.org/abs/1112.4698}{JHEP 04 (2012) 129}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-031}}{#1[\href{http://arxiv.org/abs/1112.3056}{PLB 707 (2012) 497}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-030}}{#1[\href{http://arxiv.org/abs/1204.1462}{PLB 718 (2012) 431}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-029}}{#1[\href{http://arxiv.org/abs/1202.6251}{PRL 108 (2012) 201601}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-028}}{#1[\href{http://arxiv.org/abs/1202.4717}{PRL 108 (2012) 241801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-027}}{#1[\href{http://arxiv.org/abs/1202.4979}{Eur. Phys. J. C72 (2012) 2022}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-026}}{#1[\href{http://arxiv.org/abs/1112.4695}{PRL 108 (2012) 151801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-025}}{#1[\href{http://arxiv.org/abs/1112.1600}{PLB 708 (2012) 55}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-024}}{#1[\href{http://arxiv.org/abs/1203.3592}{PRD 85 (2012) 091105(R)}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-023}}{#1[\href{http://arxiv.org/abs/1112.0938}{PRL 108 (2012) 111602}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-022}}{#1[\href{http://arxiv.org/abs/1204.1237}{JHEP 06 (2012) 115}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-021}}{#1[\href{http://arxiv.org/abs/1112.3183}{PRL 108 (2012) 101803}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-020}}{#1[\href{http://arxiv.org/abs/1112.3515}{PRL 108 (2012) 181806}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-019}}{#1[\href{http://arxiv.org/abs/1202.1080}{PLB 714 (2012) 215-223}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-018}}{#1[\href{http://arxiv.org/abs/1111.2357}{PRD 85 (2012) 032008}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-017}}{#1[\href{http://arxiv.org/abs/1110.3970}{PRD 84 (2011) 112008}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-016}}{#1[\href{http://arxiv.org/abs/1109.6831}{PRD 84 (2011) 092001}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-015}}{#1[\href{http://arxiv.org/abs/1110.2866}{JINST 7 (2012) P01010}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-014}}{#1[\href{http://arxiv.org/abs/1111.0521}{PLB 707 (2012) 349}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-013}}{#1[\href{http://arxiv.org/abs/1109.0963}{PLB 707 (2012) 52}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-012}}{#1[\href{http://arxiv.org/abs/1111.4183}{PLB 709 (2012) 50}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-011}}{#1[\href{http://arxiv.org/abs/1112.4592}{Eur. Phys. J. C72 (2012) 1947}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-010}}{#1[\href{http://arxiv.org/abs/1112.4311}{PLB 709 (2012) 177}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-009}}{#1[\href{http://arxiv.org/abs/1110.0730}{PRL 108 (2012) 101601}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-008}}{#1[\href{http://arxiv.org/abs/1110.3676}{PLB 706 (2011) 32}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-007}}{#1[\href{http://arxiv.org/abs/1107.3935}{PLB 703 (2011) 267}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-006}}{#1[\href{http://arxiv.org/abs/1106.4435}{PRL 107 (2011) 211801}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-005}}{#1[\href{http://arxiv.org/abs/1107.0882}{JHEP 08 (2011) 034}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-004}}{#1[\href{http://arxiv.org/abs/1103.2465}{PLB 699 (2011) 330}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-003}}{#1[\href{http://arxiv.org/abs/1103.0423}{Eur. Phys. J. C71 (2011) 1645}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-002}}{#1[\href{http://arxiv.org/abs/1102.0206}{PLB 698 (2011) 115}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2011-001}}{#1[\href{http://arxiv.org/abs/1102.0348}{PLB 698 (2011) 14}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2010-002}}{#1[\href{http://arxiv.org/abs/1009.2731}{PLB 694 (2010) 209}]}{}%
\ifthenelse{\equal{#2}{LHCb-PAPER-2010-001}}{#1[\href{http://arxiv.org/abs/1008.3105}{PLB 693 (2010) 69}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-008}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-008}{LHCb-CONF-2017-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-007}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-007}{LHCb-CONF-2017-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-006}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-006}{LHCb-CONF-2017-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-005}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-005}{LHCb-CONF-2017-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-004}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-004}{LHCb-CONF-2017-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-003}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-003}{LHCb-CONF-2017-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-002}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-002}{LHCb-CONF-2017-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2017-001}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2017-001}{LHCb-CONF-2017-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-018}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-018}{LHCb-CONF-2016-018}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-017}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-017}{LHCb-CONF-2016-017}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-016}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-016}{LHCb-CONF-2016-016}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-015}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-015}{LHCb-CONF-2016-015}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-014}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-014}{LHCb-CONF-2016-014}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-013}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-013}{LHCb-CONF-2016-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-012}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-012}{LHCb-CONF-2016-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-011}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-011}{LHCb-CONF-2016-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-010}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-010}{LHCb-CONF-2016-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-009}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-009}{LHCb-CONF-2016-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-008}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-008}{LHCb-CONF-2016-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-007}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-007}{LHCb-CONF-2016-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-006}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-006}{LHCb-CONF-2016-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-005}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-005}{LHCb-CONF-2016-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-004}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-004}{LHCb-CONF-2016-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-003}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-003}{LHCb-CONF-2016-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-002}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-002}{LHCb-CONF-2016-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2016-001}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2016-001}{LHCb-CONF-2016-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-005}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-005}{LHCb-CONF-2015-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-004}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-004}{LHCb-CONF-2015-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-003}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-003}{LHCb-CONF-2015-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-002}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-002}{LHCb-CONF-2015-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2015-001}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2015-001}{LHCb-CONF-2015-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2014-004}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2014-004}{LHCb-CONF-2014-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2014-003}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2014-003}{LHCb-CONF-2014-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2014-002}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2014-002}{LHCb-CONF-2014-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2014-001}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2014-001}{LHCb-CONF-2014-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-013}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-013}{LHCb-CONF-2013-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-012}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-012}{LHCb-CONF-2013-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-011}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-011}{LHCb-CONF-2013-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-010}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-010}{LHCb-CONF-2013-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-009}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-009}{LHCb-CONF-2013-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-008}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-008}{LHCb-CONF-2013-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-007}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-007}{LHCb-CONF-2013-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-006}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-006}{LHCb-CONF-2013-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-005}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-005}{LHCb-CONF-2013-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-004}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-004}{LHCb-CONF-2013-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-003}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-003}{LHCb-CONF-2013-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-002}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-002}{LHCb-CONF-2013-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2013-001}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2013-001}{LHCb-CONF-2013-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-034}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-034}{LHCb-CONF-2012-034}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-033}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-033}{LHCb-CONF-2012-033}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-032}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-032}{LHCb-CONF-2012-032}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-031}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-031}{LHCb-CONF-2012-031}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-030}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-030}{LHCb-CONF-2012-030}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-029}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-029}{LHCb-CONF-2012-029}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-028}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-028}{LHCb-CONF-2012-028}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-027}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-027}{LHCb-CONF-2012-027}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-026}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-026}{LHCb-CONF-2012-026}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-025}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-025}{LHCb-CONF-2012-025}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-024}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-024}{LHCb-CONF-2012-024}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-023}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-023}{LHCb-CONF-2012-023}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-022}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-022}{LHCb-CONF-2012-022}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-021}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-021}{LHCb-CONF-2012-021}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-020}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-020}{LHCb-CONF-2012-020}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-019}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-019}{LHCb-CONF-2012-019}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-018}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-018}{LHCb-CONF-2012-018}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-017}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-017}{LHCb-CONF-2012-017}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-016}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-016}{LHCb-CONF-2012-016}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-015}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-015}{LHCb-CONF-2012-015}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-014}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-014}{LHCb-CONF-2012-014}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-013}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-013}{LHCb-CONF-2012-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-012}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-012}{LHCb-CONF-2012-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-011}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-011}{LHCb-CONF-2012-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-010}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-010}{LHCb-CONF-2012-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-009}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-009}{LHCb-CONF-2012-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-008}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-008}{LHCb-CONF-2012-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-007}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-007}{LHCb-CONF-2012-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-006}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-006}{LHCb-CONF-2012-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-005}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-005}{LHCb-CONF-2012-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-004}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-004}{LHCb-CONF-2012-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-003}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-003}{LHCb-CONF-2012-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-002}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-002}{LHCb-CONF-2012-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2012-001}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2012-001}{LHCb-CONF-2012-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-062}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-062}{LHCb-CONF-2011-062}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-061}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-061}{LHCb-CONF-2011-061}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-060}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-060}{LHCb-CONF-2011-060}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-059}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-059}{LHCb-CONF-2011-059}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-058}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-058}{LHCb-CONF-2011-058}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-057}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-057}{LHCb-CONF-2011-057}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-056}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-056}{LHCb-CONF-2011-056}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-047}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-047}{LHCb-CONF-2011-047}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-055}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-055}{LHCb-CONF-2011-055}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-054}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-054}{LHCb-CONF-2011-054}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-053}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-053}{LHCb-CONF-2011-053}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-052}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-052}{LHCb-CONF-2011-052}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-051}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-051}{LHCb-CONF-2011-051}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-050}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-050}{LHCb-CONF-2011-050}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-049}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-049}{LHCb-CONF-2011-049}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-048}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-048}{LHCb-CONF-2011-048}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-046}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-046}{LHCb-CONF-2011-046}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-045}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-045}{LHCb-CONF-2011-045}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-044}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-044}{LHCb-CONF-2011-044}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-043}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-043}{LHCb-CONF-2011-043}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-042}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-042}{LHCb-CONF-2011-042}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-041}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-041}{LHCb-CONF-2011-041}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-040}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-040}{LHCb-CONF-2011-040}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-039}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-039}{LHCb-CONF-2011-039}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-038}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-038}{LHCb-CONF-2011-038}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-037}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-037}{LHCb-CONF-2011-037}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-036}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-036}{LHCb-CONF-2011-036}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-035}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-035}{LHCb-CONF-2011-035}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-034}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-034}{LHCb-CONF-2011-034}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-033}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-033}{LHCb-CONF-2011-033}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-031}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-031}{LHCb-CONF-2011-031}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-030}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-030}{LHCb-CONF-2011-030}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-029}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-029}{LHCb-CONF-2011-029}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-028}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-028}{LHCb-CONF-2011-028}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-027}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-027}{LHCb-CONF-2011-027}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-026}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-026}{LHCb-CONF-2011-026}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-025}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-025}{LHCb-CONF-2011-025}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-024}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-024}{LHCb-CONF-2011-024}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-023}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-023}{LHCb-CONF-2011-023}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-022}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-022}{LHCb-CONF-2011-022}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-021}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-021}{LHCb-CONF-2011-021}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-019}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-019}{LHCb-CONF-2011-019}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-020}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-020}{LHCb-CONF-2011-020}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-018}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-018}{LHCb-CONF-2011-018}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-017}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-017}{LHCb-CONF-2011-017}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-016}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-016}{LHCb-CONF-2011-016}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-015}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-015}{LHCb-CONF-2011-015}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-014}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-014}{LHCb-CONF-2011-014}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-013}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-013}{LHCb-CONF-2011-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-012}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-012}{LHCb-CONF-2011-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-011}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-011}{LHCb-CONF-2011-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-010}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-010}{LHCb-CONF-2011-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-009}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-009}{LHCb-CONF-2011-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-008}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-008}{LHCb-CONF-2011-008}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-007}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-007}{LHCb-CONF-2011-007}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-006}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-006}{LHCb-CONF-2011-006}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-005}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-005}{LHCb-CONF-2011-005}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-004}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-004}{LHCb-CONF-2011-004}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-003}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-003}{LHCb-CONF-2011-003}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-002}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-002}{LHCb-CONF-2011-002}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2011-001}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2011-001}{LHCb-CONF-2011-001}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-014}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-014}{LHCb-CONF-2010-014}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-013}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-013}{LHCb-CONF-2010-013}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-012}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-012}{LHCb-CONF-2010-012}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-011}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-011}{LHCb-CONF-2010-011}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-010}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-010}{LHCb-CONF-2010-010}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-009}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-009}{LHCb-CONF-2010-009}]}{}%
\ifthenelse{\equal{#2}{LHCb-CONF-2010-008}}{#1[\href{https://cds.cern.ch/search?ln=en&as=1&m1=p&f1=reportnumber&p1=LHCb-CONF-2010-008}{LHCb-CONF-2010-008}]}{}%
}}

==> LHCbInternal/Scripts/trunk/python/latexdiff <==
#!/usr/bin/env perl
##!/usr/bin/perl -w
# latexdiff - differences two latex files on the word level
#             and produces a latex file with the differences marked up.
#
#   Copyright (C) 2004-12  F J Tilmann (tilmann@gfz-potsdam.de, ftilmann@users.berlios.de)
#
# Project webpages:   http://latexdiff.berlios.de/
# CTAN page:          http://www.ctan.org/tex-archive/support/latexdiff
#
#    This program is free software: you can redistribute it and/or modify
#    it under the terms of the GNU General Public License as published by
#    the Free Software Foundation, either version 3 of the License, or
#    (at your option) any later version.
#
#    This program is distributed in the hope that it will be useful,
#    but WITHOUT ANY WARRANTY; without even the implied warranty of
#    MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
#    GNU General Public License for more details.
#    You should have received a copy of the GNU General Public License
#    along with this program.  If not, see <http://www.gnu.org/licenses/>.
#
# Detailed usage information at the end of the file
#
# Version 1.0.1 - treat \big,\bigg etc. equivalently to \left and
#              \right - include starred version in MATHENV - apply
#            - flatten recursively and --flatten expansion is now
#              aware of comments (thanks to Tim Connors for patch) 
#            - Change to post-processing for more reliability for
#              deleted math environments
#            - On linux systems, recognise  and remove DOS style newlines 
#            - Provide markup for some special preamble commands (\title,
#              \author,\date, 
#            - configurable by setting context2cmd 
#            - for styles using ulem package, remove \emph and \text.. from list of
#              safe commands in order to allow linebreaks within the
#              highlighted sections.  
#            - for ulem style, now show citations by enclosing them in \mbox commands. 
#              This unfortunately implies linebreaks within citations no longer function, 
#              so this functionality can be turned off (Option --disable-citation-markup). 
#              With --enable-citation-markup, the mbox markup is forced for other styles)
#            - new substyle COLOR.  This is particularly useful for marking up citations
#              and some special post-processing is implemented to retain cite
#              commands in deleted blocks.
#            - four different levels of math-markup
#            - Option --driver for choosing driver for modes employing changebar package
#            - accept \\* as valid command (and other commands of form \.*). Also accept
#              \<nl> (backslashed newline) 
#            - some typo fixes, include commands defined in preamble as safe commands
#              (Sebastian Gouezel) 
#            - include compared filenames as comments as line 2 and 3 of
#              the preamble (can be modified with option --label, and suppressed with 
#              --no-label), option --visible-label to show files in generated pdf or dvi
#              at the beginning of main document
#
# Version 0.5  A number of minor improvements based on feedback
#              Deleted blocks are now shown before added blocks
#              Package specific processing
#
# Version 0.43 unreleased typo in list of styles at the end
#              Add protect to all \cbstart, \cbend commands
#              More robust substitution of deleted math commands
#
# Version 0.42 November 06  Bug fixes only
#
# Version 0.4   March 06 option for fast differencing using UNIX diff command, several minor bug fixes (\par bug, improved highlighting of textcmds)
#
# Version 0.3   August 05 improved parsing of displayed math, --allow-spaces 
#               option, several minor bug fixes
#
# Version 0.25  October 04 Fix bug with deleted equations, add math mode commands to safecmd, add | to allowed interpunctuation signs
# Version 0.2   September 04 extension to utf-8 and variable encodings
# Version 0.1   August 04    First public release

# Inserted block for stand-alone version replaces
# use Algorithm::Diff qw(traverse_sequences);
# in standard version
# The following BEGIN block contains a verbatim copy of
# Ned Konz' Algorithm::Diff package version 1.15 except
# that all POD documentation has been stripped out.
# I encourage you to download and install the Algorithm::Diff
# package and use the standard latexdiff version instead
# (current distribution available from http://search.cpan.org/~nedkonz/Algorithm-Diff-1.15
#  the most recent version can be found via  http://search.cpan.org/search?module=Algorithm::Diff )
# Please note that the LICENCSE for Algorithm::Diff :
#   "Copyright (c) 2000-2002 Ned Konz.  All rights reserved.
#    This program is free software;
#    you can redistribute it and/or modify it under the same terms
#    as Perl itself."
# The stand-alone version of latexdiff is provided as a convenience
# for latex users with no knowledge of PERL who do not wish to install
# additional packages to be able to use latexdiff.  If you believe
# the inlining of Algorithm::Diff violates its license please contact
# me and I will modify the latexdiff distribution accordingly.
# Frederik Tilmann (tilmann@esc.cam.ac.uk)
BEGIN { 
package Algorithm::Diff;
use strict;
use vars qw($VERSION @EXPORT_OK @ISA @EXPORT);
use integer;    # see below in _replaceNextLargerWith() for mod to make
                # if you don't use this
require Exporter;
@ISA       = qw(Exporter);
@EXPORT    = qw();
@EXPORT_OK = qw(LCS diff traverse_sequences traverse_balanced sdiff);
$VERSION = sprintf('%d.%02d so', (q$Revision: 1.15 $ =~ /\d+/g));

# McIlroy-Hunt diff algorithm
# Adapted from the Smalltalk code of Mario I. Wolczko, <mario@wolczko.com>
# by Ned Konz, perl@bike-nomad.com


# Create a hash that maps each element of $aCollection to the set of positions
# it occupies in $aCollection, restricted to the elements within the range of
# indexes specified by $start and $end.
# The fourth parameter is a subroutine reference that will be called to
# generate a string to use as a key.
# Additional parameters, if any, will be passed to this subroutine.
#
# my $hashRef = _withPositionsOfInInterval( \@array, $start, $end, $keyGen );

sub _withPositionsOfInInterval
{
	my $aCollection = shift;    # array ref
	my $start       = shift;
	my $end         = shift;
	my $keyGen      = shift;
	my %d;
	my $index;
	for ( $index = $start ; $index <= $end ; $index++ )
	{
		my $element = $aCollection->[$index];
		my $key = &$keyGen( $element, @_ );
		if ( exists( $d{$key} ) )
		{
			unshift ( @{ $d{$key} }, $index );
		}
		else
		{
			$d{$key} = [$index];
		}
	}
	return wantarray ? %d : \%d;
}

# Find the place at which aValue would normally be inserted into the array. If
# that place is already occupied by aValue, do nothing, and return undef. If
# the place does not exist (i.e., it is off the end of the array), add it to
# the end, otherwise replace the element at that point with aValue.
# It is assumed that the array's values are numeric.
# This is where the bulk (75%) of the time is spent in this module, so try to
# make it fast!

sub _replaceNextLargerWith
{
	my ( $array, $aValue, $high ) = @_;
	$high ||= $#$array;

	# off the end?
	if ( $high == -1 || $aValue > $array->[-1] )
	{
		push ( @$array, $aValue );
		return $high + 1;
	}

	# binary search for insertion point...
	my $low = 0;
	my $index;
	my $found;
	while ( $low <= $high )
	{
		$index = ( $high + $low ) / 2;

		#		$index = int(( $high + $low ) / 2);		# without 'use integer'
		$found = $array->[$index];

		if ( $aValue == $found )
		{
			return undef;
		}
		elsif ( $aValue > $found )
		{
			$low = $index + 1;
		}
		else
		{
			$high = $index - 1;
		}
	}

	# now insertion point is in $low.
	$array->[$low] = $aValue;    # overwrite next larger
	return $low;
}

# This method computes the longest common subsequence in $a and $b.

# Result is array or ref, whose contents is such that
# 	$a->[ $i ] == $b->[ $result[ $i ] ]
# foreach $i in ( 0 .. $#result ) if $result[ $i ] is defined.

# An additional argument may be passed; this is a hash or key generating
# function that should return a string that uniquely identifies the given
# element.  It should be the case that if the key is the same, the elements
# will compare the same. If this parameter is undef or missing, the key
# will be the element as a string.

# By default, comparisons will use "eq" and elements will be turned into keys
# using the default stringizing operator '""'.

# Additional parameters, if any, will be passed to the key generation routine.

sub _longestCommonSubsequence
{
	my $a      = shift;    # array ref
	my $b      = shift;    # array ref
	my $keyGen = shift;    # code ref
	my $compare;           # code ref

	# set up code refs
	# Note that these are optimized.
	if ( !defined($keyGen) )    # optimize for strings
	{
		$keyGen = sub { $_[0] };
		$compare = sub { my ( $a, $b ) = @_; $a eq $b };
	}
	else
	{
		$compare = sub {
			my $a = shift;
			my $b = shift;
			&$keyGen( $a, @_ ) eq &$keyGen( $b, @_ );
		};
	}

	my ( $aStart, $aFinish, $bStart, $bFinish, $matchVector ) =
	  ( 0, $#$a, 0, $#$b, [] );

	# First we prune off any common elements at the beginning
	while ( $aStart <= $aFinish
		and $bStart <= $bFinish
		and &$compare( $a->[$aStart], $b->[$bStart], @_ ) )
	{
		$matchVector->[ $aStart++ ] = $bStart++;
	}

	# now the end
	while ( $aStart <= $aFinish
		and $bStart <= $bFinish
		and &$compare( $a->[$aFinish], $b->[$bFinish], @_ ) )
	{
		$matchVector->[ $aFinish-- ] = $bFinish--;
	}

	# Now compute the equivalence classes of positions of elements
	my $bMatches =
	  _withPositionsOfInInterval( $b, $bStart, $bFinish, $keyGen, @_ );
	my $thresh = [];
	my $links  = [];

	my ( $i, $ai, $j, $k );
	for ( $i = $aStart ; $i <= $aFinish ; $i++ )
	{
		$ai = &$keyGen( $a->[$i], @_ );
		if ( exists( $bMatches->{$ai} ) )
		{
			$k = 0;
			for $j ( @{ $bMatches->{$ai} } )
			{

				# optimization: most of the time this will be true
				if ( $k and $thresh->[$k] > $j and $thresh->[ $k - 1 ] < $j )
				{
					$thresh->[$k] = $j;
				}
				else
				{
					$k = _replaceNextLargerWith( $thresh, $j, $k );
				}

				# oddly, it's faster to always test this (CPU cache?).
				if ( defined($k) )
				{
					$links->[$k] =
					  [ ( $k ? $links->[ $k - 1 ] : undef ), $i, $j ];
				}
			}
		}
	}

	if (@$thresh)
	{
		for ( my $link = $links->[$#$thresh] ; $link ; $link = $link->[0] )
		{
			$matchVector->[ $link->[1] ] = $link->[2];
		}
	}

	return wantarray ? @$matchVector : $matchVector;
}

sub traverse_sequences
{
	my $a                 = shift;                                  # array ref
	my $b                 = shift;                                  # array ref
	my $callbacks         = shift || {};
	my $keyGen            = shift;
	my $matchCallback     = $callbacks->{'MATCH'} || sub { };
	my $discardACallback  = $callbacks->{'DISCARD_A'} || sub { };
	my $finishedACallback = $callbacks->{'A_FINISHED'};
	my $discardBCallback  = $callbacks->{'DISCARD_B'} || sub { };
	my $finishedBCallback = $callbacks->{'B_FINISHED'};
	my $matchVector = _longestCommonSubsequence( $a, $b, $keyGen, @_ );

	# Process all the lines in @$matchVector
	my $lastA = $#$a;
	my $lastB = $#$b;
	my $bi    = 0;
	my $ai;

	for ( $ai = 0 ; $ai <= $#$matchVector ; $ai++ )
	{
		my $bLine = $matchVector->[$ai];
		if ( defined($bLine) )    # matched
		{
			&$discardBCallback( $ai, $bi++, @_ ) while $bi < $bLine;
			&$matchCallback( $ai,    $bi++, @_ );
		}
		else
		{
			&$discardACallback( $ai, $bi, @_ );
		}
	}

	# The last entry (if any) processed was a match.
	# $ai and $bi point just past the last matching lines in their sequences.

	while ( $ai <= $lastA or $bi <= $lastB )
	{

		# last A?
		if ( $ai == $lastA + 1 and $bi <= $lastB )
		{
			if ( defined($finishedACallback) )
			{
				&$finishedACallback( $lastA, @_ );
				$finishedACallback = undef;
			}
			else
			{
				&$discardBCallback( $ai, $bi++, @_ ) while $bi <= $lastB;
			}
		}

		# last B?
		if ( $bi == $lastB + 1 and $ai <= $lastA )
		{
			if ( defined($finishedBCallback) )
			{
				&$finishedBCallback( $lastB, @_ );
				$finishedBCallback = undef;
			}
			else
			{
				&$discardACallback( $ai++, $bi, @_ ) while $ai <= $lastA;
			}
		}

		&$discardACallback( $ai++, $bi, @_ ) if $ai <= $lastA;
		&$discardBCallback( $ai, $bi++, @_ ) if $bi <= $lastB;
	}

	return 1;
}

sub traverse_balanced
{
	my $a                 = shift;                                  # array ref
	my $b                 = shift;                                  # array ref
	my $callbacks         = shift || {};
	my $keyGen            = shift;
	my $matchCallback     = $callbacks->{'MATCH'} || sub { };
	my $discardACallback  = $callbacks->{'DISCARD_A'} || sub { };
	my $discardBCallback  = $callbacks->{'DISCARD_B'} || sub { };
	my $changeCallback    = $callbacks->{'CHANGE'};
	my $matchVector = _longestCommonSubsequence( $a, $b, $keyGen, @_ );

	# Process all the lines in match vector
	my $lastA = $#$a;
	my $lastB = $#$b;
	my $bi    = 0;
	my $ai    = 0;
	my $ma    = -1;
	my $mb;

	while (1)
	{

		# Find next match indices $ma and $mb
		do { $ma++ } while ( $ma <= $#$matchVector && !defined $matchVector->[$ma] );

		last if $ma > $#$matchVector;    # end of matchVector?
		$mb = $matchVector->[$ma];

		# Proceed with discard a/b or change events until
		# next match
		while ( $ai < $ma || $bi < $mb )
		{

			if ( $ai < $ma && $bi < $mb )
			{

				# Change
				if ( defined $changeCallback )
				{
					&$changeCallback( $ai++, $bi++, @_ );
				}
				else
				{
					&$discardACallback( $ai++, $bi, @_ );
					&$discardBCallback( $ai, $bi++, @_ );
				}
			}
			elsif ( $ai < $ma )
			{
				&$discardACallback( $ai++, $bi, @_ );
			}
			else
			{

				# $bi < $mb
				&$discardBCallback( $ai, $bi++, @_ );
			}
		}

		# Match
		&$matchCallback( $ai++, $bi++, @_ );
	}

	while ( $ai <= $lastA || $bi <= $lastB )
	{
		if ( $ai <= $lastA && $bi <= $lastB )
		{

			# Change
			if ( defined $changeCallback )
			{
				&$changeCallback( $ai++, $bi++, @_ );
			}
			else
			{
				&$discardACallback( $ai++, $bi, @_ );
				&$discardBCallback( $ai, $bi++, @_ );
			}
		}
		elsif ( $ai <= $lastA )
		{
			&$discardACallback( $ai++, $bi, @_ );
		}
		else
		{

			# $bi <= $lastB
			&$discardBCallback( $ai, $bi++, @_ );
		}
	}

	return 1;
}

sub LCS
{
	my $a = shift;                                           # array ref
	my $matchVector = _longestCommonSubsequence( $a, @_ );
	my @retval;
	my $i;
	for ( $i = 0 ; $i <= $#$matchVector ; $i++ )
	{
		if ( defined( $matchVector->[$i] ) )
		{
			push ( @retval, $a->[$i] );
		}
	}
	return wantarray ? @retval : \@retval;
}

sub diff
{
	my $a      = shift;    # array ref
	my $b      = shift;    # array ref
	my $retval = [];
	my $hunk   = [];
	my $discard = sub { push ( @$hunk, [ '-', $_[0], $a->[ $_[0] ] ] ) };
	my $add = sub { push ( @$hunk, [ '+', $_[1], $b->[ $_[1] ] ] ) };
	my $match = sub { push ( @$retval, $hunk ) if scalar(@$hunk); $hunk = [] };
	traverse_sequences( $a, $b,
		{ MATCH => $match, DISCARD_A => $discard, DISCARD_B => $add }, @_ );
	&$match();
	return wantarray ? @$retval : $retval;
}

sub sdiff
{
	my $a      = shift;    # array ref
	my $b      = shift;    # array ref
	my $retval = [];
	my $discard = sub { push ( @$retval, [ '-', $a->[ $_[0] ], "" ] ) };
	my $add = sub { push ( @$retval, [ '+', "", $b->[ $_[1] ] ] ) };
	my $change = sub {
		push ( @$retval, [ 'c', $a->[ $_[0] ], $b->[ $_[1] ] ] );
	};
	my $match = sub {
		push ( @$retval, [ 'u', $a->[ $_[0] ], $b->[ $_[1] ] ] );
	};
	traverse_balanced(
		$a,
		$b,
		{
			MATCH     => $match,
			DISCARD_A => $discard,
			DISCARD_B => $add,
			CHANGE    => $change,
		},
		@_
	);
	return wantarray ? @$retval : $retval;
}

1;
}
import Algorithm::Diff qw(traverse_sequences);
# End of inserted block for stand-alone version

use Getopt::Long ;
use strict ;
use warnings;
use utf8 ;

my ($algodiffversion)=split(/ /,$Algorithm::Diff::VERSION);


my ($versionstring)=<<EOF ;
This is LATEXDIFF 1.0.2  (Algorithm::Diff $Algorithm::Diff::VERSION, Perl $^V)
  (c) 2004-2012 F J Tilmann
EOF

# Configuration variables: these have to be visible from the subroutines
my $MINWORDSBLOCK=3; # minimum number of tokens to form an independent block
                     # shorter identical blocks will be merged to the previous word
my $FLOATENV='(?:figure|table|plate)[\w\d*@]*' ;   # Environments in which FL variants of defined commands are used
my $PICTUREENV='(?:picture|DIFnomarkup)[\w\d*@]*' ;   # Environments in which all change markup is removed
my $MATHENV='(?:equation[*]?|displaymath|DOLLARDOLLAR)[*]?' ;           # Environments turning on display math mode (code also knows about \[ and \])
my $MATHREPL='displaymath';  # Environment introducing deleted maths blocks
my $MATHARRENV='(?:eqnarray|align|alignat|gather|multline|flalign)[*]?' ;           # Environments turning on eqnarray math mode
my $MATHARRREPL='eqnarray*';  # Environment introducing deleted maths blocks
my $ARRENV='(?:array|[pbvBV]matrix)'; # Environments making arrays in math mode.  The underlining style does not cope well with those - as a result in-text math environments are surrounded by \mbox{ } if any of these commands is used in an inline math block
my $COUNTERCMD='(?:footnote|part|chapter|section|subsection|subsubsection|paragraph|subparagraph)';  # textcmds which are associated with a counter
                                        # If any of these commands occur in a deleted block
                                        # they will be succeeded by an \addtocounter{...}{-1}
                                        # for the associated counter such that the overall numbers
                                        # should be the same as in the new file
my $CITECMD=0 ;  # \cite-type commands which need to be protected within an mbox in UNDERLINE and other modes using ulem; pattern simply designed to never match; will be overwritten later for selected styles
my $CITE2CMD=0;  # \cite-type commands which should be reinstated in deleted blocks



# Markup strings
# If at all possible, do not change these as parts of the program
# depend on the actual name (particularly post-processing)
# At the very least adapt subroutine postprocess to new tokens.
my $ADDMARKOPEN='\DIFaddbegin ';   # Token to mark begin of appended text
my $ADDMARKCLOSE='\DIFaddend ';   # Token to mark end of appended text
my $ADDOPEN='\DIFadd{';  # To mark begin of added text passage
my $ADDCLOSE='}';        # To mark end of added text passage
my $ADDCOMMENT='DIF > ';   # To mark added comment line
my $DELMARKOPEN='\DIFdelbegin ';   # Token to mark begin of deleted text
my $DELMARKCLOSE='\DIFdelend ';   # Token to mark end of deleted text
my $DELOPEN='\DIFdel{';  # To mark begin of deleted text passage
my $DELCLOSE='}';        # To mark end of deleted text passage
my $DELCMDOPEN='%DIFDELCMD < ';  # To mark begin of deleted commands (must begin with %, i.e., be a comment
my $DELCMDCLOSE="%%%\n";    # To mark end of deleted commands (must end with a new line)
my $AUXCMD='%DIFAUXCMD' ; #  follows auxiliary commands put in by latexdiff to make difference file legal
                          # auxiliary commands must be on a line of their own
my $DELCOMMENT='DIF < ';   # To mark deleted comment line


# main local variables:
my @TEXTCMDLIST=();  # array containing patterns of commands with text arguments
my @TEXTCMDEXCL=();  # array containing patterns of commands without text arguments (if a pattern
                     # matches both TEXTCMDLIST and TEXTCMDEXCL it is excluded)
my @CONTEXT1CMDLIST=();  # array containing patterns of commands with text arguments (subset of text commands),
                         # but which cause confusion if used out of context (e.g. \caption). 
                         # In deleted passages, the command will be disabled but its argument is marked up
                         # Otherwise they behave exactly like TEXTCMD's 
my @CONTEXT1CMDEXCL=();  # exclude list for above, but always empty
my @CONTEXT2CMDLIST=();  # array containing patterns of commands with text arguments, but which fail or cause confusion
                         # if used out of context (e.g. \title). They and their arguments will be disabled in deleted
                         # passages
my @CONTEXT2CMDEXCL=();  # exclude list for above, but always empty
my @MATHTEXTCMDLIST=();  # treat like textcmd.  If a textcmd is in deleted or added block, just wrap the
                         # whole content with \DIFadd or \DIFdel irrespective of content.  This functionality 
                         # is useful for pseudo commands \MATHBLOCK.. into which math environments are being
                         # transformed 
my @MATHTEXTCMDEXCL=();  # 

# Note I need to declare this with "our" instead of "my" because later in the code I have to "local"ise these  
our @SAFECMDLIST=();  # array containing patterns of safe commands (which do not break when in the argument of DIFadd or DIFDEL)
our @SAFECMDEXCL=();

my ($i,$j,$l);
my ($old,$new);
my ($line);
my ($newpreamble,$oldpreamble);
my (@newpreamble,@oldpreamble,@diffpreamble,@diffbody);
my ($latexdiffpreamble);
my ($oldbody, $newbody, $diffbo);
my ($oldpost, $newpost);
my ($diffall);
# Option names
my ($type,$subtype,$floattype,$config,$preamblefile,$encoding,$nolabel,$visiblelabel,
    $showpreamble,$showsafe,$showtext,$showconfig,$showall,
    $replacesafe,$appendsafe,$excludesafe,
    $replacetext,$appendtext,$excludetext,
    $replacecontext1,$appendcontext1,
    $replacecontext2,$appendcontext2,
    $help,$verbose,$driver,$version,$ignorewarnings,
    $enablecitmark,$disablecitmark,$allowspaces,$flatten,$debug);  ###$disablemathmark,
# MNEMNONICS for mathmarkup
my $mathmarkup;
use constant {
  OFF => 0,
  WHOLE => 1,
  COARSE => 2,
  FINE => 3
};


my (@configlist,@labels,
    @appendsafelist,@excludesafelist,
    @appendtextlist,@excludetextlist,
    @appendcontext1list,@appendcontext2list,
    @packagelist);
my ($assign,@config);
# Hash where keys corresponds to the names of  all included packages (including the documentclass as another package
# the optional arguments to the package are the values of the hash elements
my ($pkg,%packages);
# Defaults
$type='UNDERLINE';
$subtype='SAFE';
$floattype='FLOATSAFE';
$mathmarkup=COARSE;

$verbose=0;
# output debug and intermediate files, set to 0 in final distribution
$debug=0; 
# define character properties
sub IsNonAsciiPunct { return <<'END'    # Unicode punctuation but excluding ASCII punctuation
+utf8::IsPunct
-utf8::IsASCII
END
}
sub IsNonAsciiS { return <<'END'       # Unicode symbol but excluding ASCII
+utf8::IsS
-utf8::IsASCII
END
}


my %verbhash;

Getopt::Long::Configure('bundling');
GetOptions('type|t=s' => \$type, 
	   'subtype|s=s' => \$subtype, 
	   'floattype|f=s' => \$floattype, 
	   'config|c=s' => \@configlist,
	   'preamble|p=s' => \$preamblefile,
	   'encoding|e=s' => \$encoding,
	   'label|L=s' => \@labels,
	   'no-label' => \$nolabel,
	   'visible-label' => \$visiblelabel,
	   'exclude-safecmd|A=s' => \@excludesafelist,
	   'replace-safecmd=s' => \$replacesafe,
	   'append-safecmd|a=s' => \@appendsafelist,
	   'exclude-textcmd|X=s' => \@excludetextlist,
	   'replace-textcmd=s' => \$replacetext,
	   'append-textcmd|x=s' => \@appendtextlist,
	   'replace-context1cmd=s' => \$replacecontext1,
	   'append-context1cmd=s' => \@appendcontext1list,
	   'replace-context2cmd=s' => \$replacecontext2,
	   'append-context2cmd=s' => \@appendcontext2list,
	   'show-preamble' => \$showpreamble,
	   'show-safecmd' => \$showsafe,
	   'show-textcmd' => \$showtext,
	   'show-config' => \$showconfig,
	   'show-all' => \$showall,
           'packages=s' => \@packagelist,
	   'allow-spaces' => \$allowspaces,
           'math-markup=s' => \$mathmarkup,
           'enable-citation-markup' => \$enablecitmark,
           'disable-citation-markup' => \$disablecitmark,
	   'verbose|V' => \$verbose,
	   'ignore-warnings' => \$ignorewarnings,
	   'driver=s'=> \$driver,
	   'flatten' => \$flatten,
	   'version' => \$version,
	   'help|h|H' => \$help);

if ( $help ) {
  usage() ;
}


if ( $version ) {
  die $versionstring ; 
}

print STDERR $versionstring if $verbose; 

if (defined($showall)){
  $showpreamble=$showsafe=$showtext=$showconfig=1;
}

if (defined($mathmarkup)) {
  $mathmarkup=~tr/a-z/A-Z/;
  if ( $mathmarkup eq 'OFF' ){
    $mathmarkup=OFF;
  } elsif ( $mathmarkup eq 'WHOLE' ){ 
    $mathmarkup=WHOLE;
  } elsif ( $mathmarkup eq 'COARSE' ){
    $mathmarkup=COARSE;
  } elsif ( $mathmarkup eq 'FINE' ){
    $mathmarkup=FINE;
  } elsif ( $mathmarkup !~ m/^[0123]$/ ) {
    die "Illegal value: ($mathmarkup)  for option--math-markup. Possible values: OFF,WHOLE,COARSE,FINE,0- ";
  }
  # else use numerical value
}

# setting extra preamble commands
if (defined($preamblefile)) {
  $latexdiffpreamble=join "\n",(extrapream($preamblefile),"");
} else {
  $latexdiffpreamble=join "\n",(extrapream($type,$subtype,$floattype),"");
}

if ( defined($driver) ) {
  # for changebar only
  $latexdiffpreamble=~s/\[dvips\]/[$driver]/sg;
}
# setting up @SAFECMDLIST and @SAFECMDEXCL
if (defined($replacesafe)) {
  init_regex_arr_ext(\@SAFECMDLIST,$replacesafe);
} else {
  init_regex_arr_data(\@SAFECMDLIST, "SAFE COMMANDS");
}
foreach $appendsafe ( @appendsafelist ) {
  init_regex_arr_ext(\@SAFECMDLIST, $appendsafe);
}
foreach $excludesafe ( @excludesafelist ) {
  init_regex_arr_ext(\@SAFECMDEXCL, $excludesafe);
}

# Special: treat all cite commands as safe except in UNDERLINE and FONTSTRIKE mode
# (there is a conflict between citation and ulem package, see
# package documentation)
# Use post-processing

if ( uc($type) ne "UNDERLINE" && uc($type) ne "FONTSTRIKE" && uc($type) ne "CULINECHBAR" ) {
  push (@SAFECMDLIST, qr/^cite.*$/);
} else {
  ### Experimental: disable text and emph commands
  push (@SAFECMDLIST, qr/^cite.*$/) unless $disablecitmark;
  push(@SAFECMDEXCL, qr/^emph$/, qr/^text..$/);
  # replace \cite{..} by \mbox{\cite{..}} in added or deleted blocks in post-processing
  if ( uc($subtype) eq "COLOR" or uc($subtype) eq "DVIPSCOL" ) {
    # remove \cite command again from list of safe commands
    pop @SAFECMDLIST;
    # deleted cite commands
    $CITE2CMD='(?:cite\w*|nocite)' unless $disablecitmark ; # \cite-type commands which should be reinstated in deleted blocks
  } else {
    $CITECMD='(?:cite\w*|nocite)' unless $disablecitmark ; # \cite commands which need to be protected within an mbox in UNDERLINE and other modes using ulem
  }
}
$CITECMD='(?:cite\w*|nocite)' if $enablecitmark ; # as above for explicit selection

# setting up @TEXTCMDLIST and @TEXTCMDEXCL
if (defined($replacetext)) {
  init_regex_arr_ext(\@TEXTCMDLIST,$replacetext);
} else {
  init_regex_arr_data(\@TEXTCMDLIST, "TEXT COMMANDS");
}
foreach $appendtext ( @appendtextlist ) {
  init_regex_arr_ext(\@TEXTCMDLIST, $appendtext);
}
foreach $excludetext ( @excludetextlist ) {
  init_regex_arr_ext(\@TEXTCMDEXCL, $excludetext);
}


# setting up @CONTEXT1CMDLIST ( @CONTEXT1CMDEXCL exist but is always empty )
if (defined($replacecontext1)) {
  init_regex_arr_ext(\@CONTEXT1CMDLIST,$replacecontext1);
} else {
  init_regex_arr_data(\@CONTEXT1CMDLIST, "CONTEXT1 COMMANDS");
}
foreach $appendcontext1 ( @appendcontext1list ) {
  init_regex_arr_ext(\@CONTEXT1CMDLIST, $appendcontext1);
}


# setting up @CONTEXT2CMDLIST ( @CONTEXT2CMDEXCL exist but is always empty )
if (defined($replacecontext2)) {
  init_regex_arr_ext(\@CONTEXT2CMDLIST,$replacecontext2);
} else {
  init_regex_arr_data(\@CONTEXT2CMDLIST, "CONTEXT2 COMMANDS");
}
foreach $appendcontext2 ( @appendcontext2list ) {
  init_regex_arr_ext(\@CONTEXT2CMDLIST, $appendcontext2);
}

# setting configuration variables
@config=();
foreach $config ( @configlist ) {
  if (-f $config ) {
    open(FILE,$config) or die ("Couldn't open configuration file $config: $!");
    while (<FILE>) {
      chomp;
      next if /^\s*#/ || /^\s*%/ || /^\s*$/ ;
      push (@config,$_);
    }
    close(FILE);
  }
  else {
#    foreach ( split(",",$config) ) {
#      push @config,$_;
#    }
     push @config,split(",",$config)
  }
}
foreach $assign ( @config ) {
  $assign=~ m/\s*(\w*)\s*=\s*(\S*)\s*$/ or die "Illegal assignment $assign in configuration list (must be variable=value)";  
  if ( $1 eq "MINWORDSBLOCK" ) { $MINWORDSBLOCK = $2; }
  elsif ( $1 eq "FLOATENV" ) { $FLOATENV = $2 ; }
  elsif ( $1 eq "PICTUREENV" ) { $PICTUREENV = $2 ; }
  elsif ( $1 eq "MATHENV" ) { $MATHENV = $2 ; }
  elsif ( $1 eq "MATHREPL" ) { $MATHREPL = $2 ; }
  elsif ( $1 eq "MATHARRENV" ) { $MATHARRENV = $2 ; }
  elsif ( $1 eq "MATHARRREPL" ) { $MATHARRREPL = $2 ; }
  elsif ( $1 eq "ARRENV" ) { $ARRENV = $2 ; }
  elsif ( $1 eq "COUNTERCMD" ) { $COUNTERCMD = $2 ; }
  else { die "Unknown variable $1 in assignment.";}
}

if ( $mathmarkup == COARSE || $mathmarkup == WHOLE ) {
  push(@MATHTEXTCMDLIST,qr/^MATHBLOCK(?:$MATHENV|$MATHARRENV|SQUAREBRACKET)$/);
}



foreach $pkg ( @packagelist ) {
  map { $packages{$_}="" } split(/,/,$pkg) ;
}

if ($showpreamble) {
  print "\nPreamble commands:\n";
  print $latexdiffpreamble ;
}

if ($showsafe) {
  print "\nCommands safe within scope of $ADDOPEN $ADDCLOSE and $DELOPEN $DELCLOSE (unless excluded):\n";
  print_regex_arr(@SAFECMDLIST);
  print "\nCommands not safe within scope of $ADDOPEN $ADDCLOSE and $DELOPEN $DELCLOSE :\n";
  print_regex_arr(@SAFECMDEXCL);
}

if ($showtext) {
  print "\nCommands with last argument textual (unless excluded) and safe in every context:\n";
  print_regex_arr(@TEXTCMDLIST);
  print "\nContext1 commands (last argument textual, command will be disabled in deleted passages, last argument will be shown as plain text):\n";
  print_regex_arr(@CONTEXT1CMDLIST);
  print "\nContext2 commands (last argument textual, command and its argument will be disabled in deleted passages):\n";
  print_regex_arr(@CONTEXT2CMDLIST);  
  print "\nExclude list of Commands with last argument not textual (overrides patterns above):\n";
  print_regex_arr(@TEXTCMDEXCL);
}


if ($showconfig) {
  print "Configuration variables:\n";
  print "MINWORDSBLOCK=$MINWORDSBLOCK\n";
  print "FLOATENV=$FLOATENV\n";
  print "PICTUREENV=$PICTUREENV\n";
  print "MATHENV=$MATHENV\n";
  print "MATHREPL=$MATHREPL\n";
  print "MATHARRENV=$MATHARRENV\n";
  print "MATHARRREPL=$MATHARRREPL\n";
  print "ARRENV=$ARRENV\n";
  print "COUNTERCMD=$COUNTERCMD\n";
}
if ($showconfig || $showtext || $showsafe || $showpreamble) {
  exit 0; }
if ( @ARGV != 2 ) { 
  print STDERR "2 and only 2 non-option arguments required.  Write latexdiff -h to get help\n";
  exit(2);
}

# Are extra spaces between command arguments permissible?
my $extraspace;
if ($allowspaces) {
  $extraspace='\s*'; 
} else {
  $extraspace='';
}

# append context lists to text lists (as text property is implied)
push @TEXTCMDLIST, @CONTEXT1CMDLIST;
push @TEXTCMDLIST, @CONTEXT2CMDLIST;

push @TEXTCMDLIST, @MATHTEXTCMDLIST if $mathmarkup==COARSE;

# internal additions to SAFECMDLIST
push(@SAFECMDLIST, qr/^QLEFTBRACE$/, qr/^QRIGHTBRACE$/);


# Patterns. These are used by some of the subroutines, too
# I can only define them down here because value of extraspace depends on an option
  my $pat0 = '(?:[^{}])*';
  my $pat1 = '(?:[^{}]|\{'.$pat0.'\})*';
  my $pat2 = '(?:[^{}]|\{'.$pat1.'\})*';
  my $pat3 = '(?:[^{}]|\{'.$pat2.'\})*';
  my $pat4 = '(?:[^{}]|\{'.$pat3.'\})*';
  my $pat5 = '(?:[^{}]|\{'.$pat4.'\})*';
  my $pat6 = '(?:[^{}]|\{'.$pat5.'\})*';
  my $brat0 = '(?:[^\[\]]|\\\[|\\\])*'; 

  my $quotemarks = '(?:\'\')|(?:\`\`)';
  my $punct='[0.,\/\'\`:;\"\?\(\)\[\]!~\p{IsNonAsciiPunct}\p{IsNonAsciiS}]';
  my $number='-?\d*\.\d*';
  my $mathpunct='[+=<>\-\|]';
  my $and = '&';
  my $coords= '[\-.,\s\d]*';
# word: sequence of letters or accents followed by letter
  my $word='(?:[-\w\d*]|\\\\[\"\'\`~^][A-Za-z\*])+';
  my $cmdleftright='\\\\(?:left|right|[Bb]igg?[lrm]?|middle)\s*(?:[()\[\]|]|\\\\(?:[|{}]|\w+))';

  my $cmdoptseq='\\\\[\w\d\*]+'.$extraspace.'(?:(?:\['.$brat0.'\]|\{'. $pat6 . '\}|\(' . $coords .'\))'.$extraspace.')*';
  my $backslashnl='\\\\\n';
  my $oneletcmd='\\\\.\*?(?:\['.$brat0.'\]|\{'. $pat6 . '\})*';
  my $math='\$(?:[^$]|\\\$)*?\$|\\\\[(].*?\\\\[)]';
## the current maths command cannot cope with newline within the math expression

  my $comment='%.*?\n';
  my $pat=qr/(?:\A\s*)?(?:${and}|${quotemarks}|${number}|${word}|$cmdleftright|${cmdoptseq}|${math}|${backslashnl}|${oneletcmd}|${comment}|${punct}|${mathpunct}|\{|\})\s*/ ;



# now we are done setting up and can start working   
my ($oldfile, $newfile) = @ARGV;
# check for existence of input files
if ( ! -e $oldfile ) {
  die "Input file $oldfile does not exist.";
}
if ( ! -e $newfile ) {
  die "Input file $newfile does not exist.";
}


# set the labels to be included into the file
my ($oldtime,$newtime,$oldlabel,$newlabel);
if (defined($labels[0])) {
  $oldlabel=$labels[0] ;
} else {
  $oldtime=localtime((stat($oldfile))[9]); 
  $oldlabel="$oldfile   " . " "x(length($newfile)-length($oldfile)) . $oldtime;
}
if (defined($labels[1])) {
  $newlabel=$labels[1] ;
} else {
  $newtime=localtime((stat($newfile))[9]);
  $newlabel="$newfile   " . " "x(length($oldfile)-length($newfile)) . $newtime;
}

$encoding=guess_encoding($newfile) unless defined($encoding);

$encoding = "utf8" if $encoding =~ m/^utf8/i ;
if (lc($encoding) eq "utf8" ) {
  binmode(STDOUT, ":utf8");
  binmode(STDERR, ":utf8");
}

$old=read_file_with_encoding($oldfile,$encoding);
$new=read_file_with_encoding($newfile,$encoding);




# reset time
exetime(1);
($oldpreamble,$oldbody,$oldpost)=splitdoc($old,'\\\\begin\{document\}','\\\\end\{document\}');


($newpreamble,$newbody,$newpost)=splitdoc($new,'\\\\begin\{document\}','\\\\end\{document\}');


if ($flatten) {
  $oldbody=flatten($oldbody,$oldpreamble,$oldfile,$encoding);
  $newbody=flatten($newbody,$newpreamble,$newfile,$encoding);
}

my @auxlines;
if ( length $oldpreamble && length $newpreamble ) {
  # pre-process preamble by looking for commands used in \maketitle (title, author, date etc commands) 
  # and marking up content with latexdiff markup
  @auxlines=preprocess_preamble($oldpreamble,$newpreamble);

  @oldpreamble = split /\n/, $oldpreamble;
  @newpreamble = split /\n/, $newpreamble;

  # If a command is defined in the preamble of the new file, and only uses safe commands, then it can be considered to be safe) (contribution S. Gouezel)
  # Base this assessment on the new preamble
  add_safe_commands($newpreamble);

  %packages=list_packages(@newpreamble) unless %packages;
  if (defined $packages{"hyperref"} ) {
    print STDERR "hyperref package detected.\n" if $verbose ;
    $latexdiffpreamble =~ s/\{\\DIFadd\}/{\\DIFaddtex}/g;
    $latexdiffpreamble =~ s/\{\\DIFdel\}/{\\DIFdeltex}/g;
    $latexdiffpreamble .= join "\n",(extrapream("HYPERREF"),"");
  }
  print STDERR "Differencing preamble.\n" if $verbose;

  # insert dummy first line such that line count begins with line 1 (rather than perl's line 0) - just so that line numbers inserted by linediff are correct
  unshift @newpreamble,'';
  unshift @oldpreamble,'';
  @diffpreamble = linediff(\@oldpreamble, \@newpreamble);
  # remove dummy line again
  shift @diffpreamble; 
  # add filenames, modification time and latexdiff mark
  defined($nolabel) or splice @diffpreamble,1,0,
      "%DIF LATEXDIFF DIFFERENCE FILE",
      ,"%DIF DEL $oldlabel",
      "%DIF ADD $newlabel";
  if ( @auxlines ) {
    push @diffpreamble,"%DIF DELETED TITLE COMMANDS FOR MARKUP";
    push @diffpreamble,join("\n",@auxlines);
  }
  push @diffpreamble,$latexdiffpreamble;
  push @diffpreamble,'\begin{document}';
}
elsif ( !length $oldpreamble && !length $newpreamble ) {
  @diffpreamble=();
} else {
  print STDERR "Either both texts must have preamble or neither text must have the preamble.\n";
  exit(2);
}

if (defined $packages{"amsmath"}  or defined $packages{"amsart"} or defined $packages{"amsbook"} ) {
  print STDERR "amsmath package detected.\n" if $verbose ;
  $MATHARRREPL='align*';
}

print STDERR "Preprocessing body.  " if $verbose;
my ($oldleadin,$newleadin)=preprocess($oldbody,$newbody);


# run difference algorithm
@diffbody=bodydiff($oldbody, $newbody);
$diffbo=join("",@diffbody);
if ( $debug ) {
    open(RAWDIFF,">","latexdiff.debug.bodydiff");
    print RAWDIFF $diffbo;
    close(RAWDIFF);
}
print STDERR "(",exetime()," s)\n","Postprocessing body. \n " if $verbose;
postprocess($diffbo);
$diffall =join("\n",@diffpreamble) ;
# add visible labels
if (defined($visiblelabel)) {
  # Give information right after \begin{document} (or at the beginning of the text for files without preamble
  ### if \date command is used, add information to \date argument, otherwise give right after \begin{document}
  ###  $diffall=~s/(\\date$extraspace(?:\[$brat0\])?$extraspace)\{($pat6)\}/$1\{$2 \\ LATEXDIFF comparison \\ Old: $oldlabel \\ New: $newlabel \}/  or
  $diffbo = "\\begin{verbatim}LATEXDIFF comparison\nOld: $oldlabel\nNew: $newlabel\\end{verbatim}\n$diffbo"   ;
}

$diffall .= "$newleadin$diffbo" ;
$diffall .= "\\end{document}$newpost" if length $newpreamble ;
if ( lc($encoding) ne "utf8" && lc($encoding) ne "ascii" ) {
  print STDERR "Encoding output file to $encoding\n" if $verbose;
  $diffall=Encode::encode($encoding,$diffall);
  binmode STDOUT;
}
print $diffall;


print STDERR "(",exetime()," s)\n","Done.\n" if $verbose;



## guess_encoding(filename)
## reads the first 20 lines of filename and looks for call of inputenc package
## if found, return the option of this package (encoding), otherwise return ascii
sub guess_encoding {
  my ($filename)=@_;
  my ($i,$enc);
  open (FH, $filename) or die("Couldn't open $filename: $!");
  $i=0;
  while (<FH>) {
    next if /^\s*%/;    # skip comment lines
    if (m/\\usepackage\[(\w*?)\]\{inputenc\}/) {
      close(FH);
      return($1);
    }
    last if (++$i > 20 ); # scan at most 20 non-comment lines
  }
  close(FH);
  return("ascii");
}


sub read_file_with_encoding {
  my ($output);
  my ($filename, $encoding) = @_;

  if (lc($encoding) eq "utf8" ) {
    open (FILE, "<:utf8",$filename) or die("Couldn't open $filename: $!");
    local $/ ; # locally set record operator to undefined, ie. enable whole-file mode
    $output=<FILE>;
  } elsif ( lc($encoding) eq "ascii") {
    open (FILE, $filename) or die("Couldn't open $filename: $!");
    local $/ ; # locally set record operator to undefined, ie. enable whole-file mode
    $output=<FILE>;
  } else {
    require Encode;
    open (FILE, "<",$filename) or die("Couldn't open $filename: $!");
    local $/ ; # locally set record operator to undefined, ie. enable whole-file mode
    $output=<FILE>;
    print STDERR "Converting $filename from $encoding to utf8\n" if $verbose;
    $output=Encode::decode($encoding,$output);
  }
  close FILE;
  if ($^O eq "linux" ) {
    $output =~ s/\r\n/\n/g ;
  }
  return $output;
}

# %packages=list_packages(@preamble)
# scans the arguments for \documentclass and \usepackage statements and constructs a hash
# whose keys are the included packages, and whose values are the associated optional arguments
sub list_packages {
  my (@preamble)=@_;
  my %packages=();
  foreach $line ( @preamble ) {
    # get rid of comments
    $line=~s/(?<!\\)%.*$// ;
    if ( $line =~ m/\\(?:documentclass|usepackage)(?:\[(.+?)\])?\{(.*?)\}/ ) {
#      print STDERR "Found something: |$line|\n";
      if (defined($1)) {
	$packages{$2}=$1;
      } else {
	$packages{$2}="";
      }
    }
  }
  return (%packages);
}

# Subroutine add_safe_commands modified from version provided by S. Gouezel
# add_safe_commands($preamble)
# scans the argument for \newcommand and \DeclareMathOperator,
# and adds the created commands which are clearly safe to @SAFECMDLIST
sub add_safe_commands {
  my ($preamble)=@_;
  my $added_command = 1;

  $preamble=~s/(?<!\\)%.*$//mg ;

  while ($added_command) { 
    $added_command  = 0;
      # get rid of comments
    my $to_test = "";
      # test for \DeclareMathOperator{\foo}{myoperator}
    while ( $preamble =~ m/\DeclareMathOperator\s*\{\\(\w*?)\}/s) {
      $to_test=$1;
      if ($to_test ne "" and not iscmd($to_test,\@SAFECMDLIST,\@SAFECMDEXCL) and not iscmd($to_test, \@SAFECMDEXCL, []))  {
        # one should add $to_test to the list of safe commands.
        init_regex_arr_ext(\@SAFECMDLIST, $to_test);
        $added_command = 1;
        print STDERR "Adding $to_test to the list of safe commands\n" if $verbose;
      }
    }

    while ( $preamble =~ m/\\(?:|re|provide)newcommand\s*{\\(\w*)\}(?:|\[\d*\])\s*\{(${pat6})\}/osg ) {
      my $maybe_to_test  = $1;
      my $should_be_safe = $2;
      my $success = 0;
      # test if all latex commands inside it are safe
      $success = 1;
      if ($should_be_safe =~ m/\\\\/) {
	$success = 0;
      } else {
	while ($should_be_safe =~ m/\\(\w+)/g) {
	  $success = 0 unless iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL); ### or $1 eq "";
	}
      }
      ###      }
      $to_test = $maybe_to_test if $success;
      
      if ($to_test ne "" and not iscmd($to_test,\@SAFECMDLIST,\@SAFECMDEXCL) and not iscmd($to_test, \@SAFECMDEXCL, []))  {
#        # one should add $to_test to the list of safe commands.
        init_regex_arr_ext(\@SAFECMDLIST, $to_test);
        $added_command = 1;
        print STDERR "Adding $to_test to the list of safe commands\n" if $verbose;
      }
    }
  }
}



# flatten($text,$preamble,$filename,$encoding)
# expands \input and \include commands within text
# preamble is scanned for includeonly commands
# encoding is the encoding
sub flatten {
  my ($text,$preamble,$filename,$encoding)=@_;
  my ($includeonly,$dirname,$fname,$newpage,$replacement,$begline);
  require File::Basename ; 
  require File::Spec ; 
  $dirname = File::Basename::dirname($filename);

  if ( ($includeonly) = ($preamble =~ m/\\includeonly{(.*?)}/ ) ) {
    $includeonly =~ s/,/|/g;
  } else {
    $includeonly = '.*?';
  }

  print STDERR "DEBUG: includeonly $includeonly\n" if $debug;

  $text=~s/(^(?:[^%\n]|\\%)*)\\input{(.*?)}|\\include{(${includeonly}(?:\.tex)?)}/{ 
	    $fname = $2 if defined($2) ;
	    $fname = $3 if defined($3) ;       
            #      # add tex extension unless there is a three letter extension already 
            $fname .= ".tex" unless $fname =~ m|\.\w{3}|;
            print STDERR "DEBUG Beg of line match |$1|\n" if defined($1) && $debug ;
            print STDERR "Include file $fname\n" if $verbose;
            print STDERR "DEBUG looking for file ",File::Spec->catfile($dirname,$fname), "\n" if $debug;
            # content of file becomes replacement value (use recursion), add \newpage if the command was include
            ###$replacement=read_file_with_encoding(File::Spec->catfile($dirname,$fname), $encoding) or die "Couldn't find file ",File::Spec->catfile($dirname,$fname),": $!";
	    $replacement=flatten(read_file_with_encoding(File::Spec->catfile($dirname,$fname), $encoding), $preamble,$filename,$encoding) or die "Couldn't find file ",File::Spec->catfile($dirname,$fname),": $!";
	    # \include always starts a new page; use explicit \newpage command to simulate this
	    $begline=(defined($1)? $1 : "") ;
	    $newpage=(defined($3)? " \\newpage " : "") ;
	    "$begline$newpage$replacement$newpage";
          }/exgm;

  return($text);
}


# print_regex_arr(@arr)
# prints regex array without x-ism expansion put in by pearl to stdout
sub print_regex_arr {
  my $dumstring;
  $dumstring = join(" ",@_);     # PERL generates string (?-xism:^ref$) for quoted refex ^ref$
  $dumstring =~ s/\(\?-xism:\^(.*?)\$\)/$1/g;   # remove string and ^,$ marks before output
  print $dumstring,"\n";
}


# @lines=extrapream($type)
# reads line from appendix (end of file after __END__ token)
sub extrapream {
  my $type;
  my @retval=("%DIF PREAMBLE EXTENSION ADDED BY LATEXDIFF") ;
  my ($copy);

  while (@_) {
    $copy=0;
    $type=shift ;
    if ( -f $type ) {
      open (FILE,$type) or die "Cannot open preamble file $type: $!";
      print STDERR "Reading preamble file $type\n" if $verbose ;
      while (<FILE>) {
	chomp ;
	if ( $_ =~ m/%DIF PREAMBLE/ ) {
	  push (@retval,"$_"); 
	} else {
	  push (@retval,"$_ %DIF PREAMBLE"); 
	}
      }
    } 
    else {    # not (-f $type)
      $type=uc($type);   # upcase argument
      print STDERR "Preamble Internal Type $type\n" if $verbose;
      while (<DATA>) {
	if ( m/^%DIF $type/ ) {
	  $copy=1; }
	elsif ( m/^%DIF END $type/ ) {
	  last; }
	chomp;
	push (@retval,"$_ %DIF PREAMBLE") if $copy;
      }
      if ( $copy == 0 ) {
	print STDERR "\nPreamble style $type not implemented.\n";
        print STDERR "Write latexdiff -h to get help with available styles\n";
        exit(2);
      }
      seek DATA,0,0;    # rewind DATA handle to file begin
    }
  }
  push (@retval,"%DIF END PREAMBLE EXTENSION ADDED BY LATEXDIFF")  ;
  return @retval;
}


# ($part1,$part2,$part3)=splitdoc($text,$word1,$word2)
# splits $text into 3 parts at $word1 and $word2.
# if neither $word1 nor $word2 exist, $part1 and $part3 are empty, $part2 is $text
# If only $word1 or $word2 exist but not the other, output an error message.

# NB this version avoids $` and $' for performance reason although it only makes a tiny difference
# (in one test gain a tenth of a second for a 30s run)
sub splitdoc {
  my ($text,$word1,$word2)=@_;
  my ($part1,$part2,$part3)=("","","");
  my ($rest,$pos);

  if ( $text =~ m/(^[^%]*)($word1)/mg ) {
    $pos=pos $text;
    $part1=substr($text,0,$pos-length($2));
    $rest=substr($text,$pos);
    if ( $rest =~ m/(^[^%]*)($word2)/mg ) {
      $pos=pos $rest;
      $part2=substr($rest,0,$pos-length($2));
      $part3=substr($rest,$pos);
    } 
    else {
      die "$word1 and $word2 not in the correct order or not present as a pair." ;
    }
  } else {
    $part2=$text;
    die "$word2 present but not $word1." if ( $text =~ m/(^[^%]*)$word2/ms );
  }
  return ($part1,$part2,$part3);
}





# bodydiff($old,$new)
sub bodydiff {
  my ($oldwords, $newwords) = @_;
  my @retwords;

  print STDERR "(",exetime()," s)\n","Splitting into latex tokens \n" if $verbose;
  print STDERR "Parsing $oldfile \n" if $verbose;
  my @oldwords = splitlatex($oldwords);
  print STDERR "Parsing $newfile \n" if $verbose;
  my @newwords = splitlatex($newwords);

  if ( $debug ) {
    open(TOKENOLD,">","latexdiff.debug.tokenold");
    print TOKENOLD join("***\n",@oldwords);
    close(TOKENOLD);
    open(TOKENNEW,">","latexdiff.debug.tokennew");
    print TOKENNEW join("***\n",@newwords);
    close(TOKENNEW);
  }

  print STDERR "(",exetime()," s)\n","Pass 1: Expanding text commands and merging isolated identities with changed blocks  " if $verbose;
  pass1(\@oldwords, \@newwords);


  print STDERR "(",exetime()," s)\n","Pass 2: inserting DIF tokens and mark up.  " if $verbose;
  if ( $debug ) {
    open(TOKENOLD,">","latexdiff.debug.tokenold2.tex");
    print TOKENOLD join("***\n",@oldwords);
    close(TOKENOLD);
    open(TOKENNEW,">","latexdiff.debug.tokennew2.tex");
    print TOKENNEW join("***\n",@newwords);
    close(TOKENNEW);
  }

  @retwords=pass2(\@oldwords, \@newwords);

  return(@retwords);
}




# @words=splitlatex($string)
# split string according to latex rules
# Each element of words is either
# a word (including trailing spaces and punctuation)
# a latex command
sub splitlatex {
  my ($string) = @_ ;
  # if input is empty, return empty list
  length($string)>0 or return ();

  my @retval=($string =~ m/$pat/osg);  

  if (length($string) != length(join("",@retval))) {
    print STDERR "\nWARNING: Inconsistency in length of input string and parsed string:\n     This often indicates faulty or non-standard latex code.\n     In many cases you can ignore this and the following warning messages.\n Note that character numbers in the following are counted beginning after \\begin{document} and are only approximate." unless $ignorewarnings;
    print STDERR "DEBUG Original length ",length($string),"  Parsed length ",length(join("",@retval)),"\n" if $debug;
    print STDERR "DEBUG Input string:  |$string|\n" if (length($string)<500) && $debug;
    print STDERR "DEBUG Token parsing: |",join("+",@retval),"|\n" if (length($string)<500) && $debug ;
    @retval=();
    # slow way only do this if other m//sg method fails
    my $last = 0;
    while ( $string =~ m/$pat/osg ) {
      my $match=$&;
      if ($last + length $& != pos $string  ) {
	my $pos=pos($string);
	my $offset=30<$last ? 30 : $last;
	my $dum=substr($string,$last-$offset,$pos-$last+2*$offset);
	my $dum1=$dum;
	my $cnt=$#retval;
	my $i;
	$dum1 =~ s/\n/ /g;
	unless ($ignorewarnings) {
	  print STDERR "\n$dum1\n";
	  print STDERR " " x 30,"^" x ($pos-$last)," " x 30,"\n";
	  print STDERR "Missing characters near word " . (scalar @retval) . " character index: " . $last . "-" .  pos($string) . " Length: " . length($match) . " Match: |$match| (expected match marked above).\n";
	}
	  # put in missing characters `by hand'
	push (@retval, substr($dum,$offset,$pos-$last-length($match)));
#       Note: there seems to be a bug in substr with utf8 that made the following line output substr which were too long,
#             using dum instead appears to work
#	push (@retval, substr($string,$last, pos($string)-$last-length($match)));
      }
      push (@retval, $match);
      $last=pos $string;
    }

  }
  return @retval;
}


# pass1( \@seq1,\@seq2)
# Look for differences between seq1 and seq2.
# Where an common-subsequence block is flanked by deleted or appended blocks, 
# and is shorter than $MINWORDSBLOCK words it is appended
# to the last deleted or appended word.  If the block contains tokens other than words 
# or punctuation it is not merged.
# Deleted or appended block consisting of words and safe commands only are
# also merged, to prevent break-up in pass2 (after previous isolated words have been removed)
# If there are commands with textual arguments (e.g. \caption) both in corresponding 
# appended and deleted blocks split them such that the command and opening bracket 
# are one token, then the rest is split up following standard rules, and the closing 
# bracket is a separate token, ie. turn
# "\caption{This is a textual argument}" into 
# ("\caption{","This ","is ","a ","textual ","argument","}")
# No return value.  Destructively changes sequences
sub pass1 {
  my $seq1 = shift ;
  my $seq2 = shift ;

  my $len1 = scalar @$seq1;
  my $len2 = scalar @$seq2;
  my $wpat=qr/^(?:[a-zA-Z.,'`:;?()!]*)[\s~]*$/;   #'

  my ($last1,$last2)=(-1,-1) ;
  my $cnt=0;
  my $block=[];
  my $addblock=[];
  my $delblock=[];
  my $todo=[];
  my $instruction=[];
  my $i;
  my (@delmid,@addmid,@dummy);

  my ($addcmds,$delcmds,$matchindex);
  my ($addtextblocks,$deltextblocks);
  my ($addtokcnt,$deltokcnt,$mattokcnt)=(0,0,0);
  my ($addblkcnt,$delblkcnt,$matblkcnt)=(0,0,0);

  my $adddiscard = sub {
                      if ($cnt > 0 ) {
			$matblkcnt++;
			# just after an unchanged block 
#			print STDERR "Unchanged block $cnt, $last1,$last2 \n";
                        if ($cnt < $MINWORDSBLOCK 
			    && $cnt==scalar (
				     grep { /^$wpat/ || ( /^\\([\w\d\*]+)((?:\[$brat0\]|\{$pat6\})*)/o 
							   && iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL) 
							   && scalar(@dummy=split(" ",$2))<3 ) }
					     @$block) )  {
			  # merge identical blocks shorter than $MINWORDSBLOCK 
			  # and only containing ordinary words
			  # with preceding different word
			  # We cannot carry out this merging immediately as this
			  # would change the index numbers of seq1 and seq2 and confuse
			  # the algorithm, instead we store in @$todo where we have to merge
                          push(@$todo, [ $last1,$last2,$cnt,@$block ]);
			}
			$block = []; 
			$cnt=0; $last1=-1; $last2=-1;
		      }
		    };
  my $discard=sub { $deltokcnt++;
                    &$adddiscard; #($_[0],$_[1]);
		    push(@$delblock,[ $seq1->[$_[0]],$_[0] ]);
		    $last1=$_[0] };		      

  my $add =   sub { $addtokcnt++;
                    &$adddiscard; #($_[0],$_[1]);
		    push(@$addblock,[ $seq2->[$_[1]],$_[1] ]);
		    $last2=$_[1] };		      

  my $match = sub { $mattokcnt++;
                    if ($cnt==0) {   # first word of matching sequence after changed sequence or at beginning of word sequence
		      $deltextblocks = extracttextblocks($delblock); 
		      $delblkcnt++ if scalar @$delblock;
		      $addtextblocks = extracttextblocks($addblock);
		      $addblkcnt++ if scalar @$addblock;

		      $delcmds = extractcommands($delblock);
      		      $addcmds = extractcommands($addblock);
		      # keygen(third argument of _longestCommonSubsequence) implies to sort on command (0th elements of $addcmd elements)
		      # the calling format for longestCommonSubsequence has changed between versions of
		      # Algorithm::Diff so we need to check which one we are using
		      if ( $algodiffversion  > 1.15 ) {
			### Algorithm::Diff 1.19
			$matchindex=Algorithm::Diff::_longestCommonSubsequence($delcmds,$addcmds, 0, sub { $_[0]->[0] } );
		      } else {
			### Algorithm::Diff 1.15	
			$matchindex=Algorithm::Diff::_longestCommonSubsequence($delcmds,$addcmds, sub { $_[0]->[0] } );
		      }

		      for ($i=0 ; $i<=$#$matchindex ; $i++) {
			if (defined($matchindex->[$i])){
			  $j=$matchindex->[$i];
			  @delmid=splitlatex($delcmds->[$i][3]);
			  @addmid=splitlatex($addcmds->[$j][3]);
			  while (scalar(@$deltextblocks)  && $deltextblocks->[0][0]<$delcmds->[$i][1]) {
			    my ($index,$block,$cnt)=@{ shift(@$deltextblocks) };
			    push(@$todo, [$index,-1,$cnt,@$block]);
			  }
			  push(@$todo, [ $delcmds->[$i][1],-1,-1,$delcmds->[$i][2],@delmid,$delcmds->[$i][4]]);

			  while (scalar(@$addtextblocks) && $addtextblocks->[0][0]<$addcmds->[$j][1]) {
			    my ($index,$block,$cnt)=@{ shift(@$addtextblocks) };
			    push(@$todo, [-1,$index,$cnt,@$block]);
			  }
			  push(@$todo, [ -1,$addcmds->[$j][1],-1,$addcmds->[$j][2],@addmid,$addcmds->[$j][4]]);
			}
		      }
		      # mop up remaining textblocks
		      while (scalar(@$deltextblocks)) {
			my ($index,$block,$cnt)=@{ shift(@$deltextblocks) } ;
			push(@$todo, [$index,-1,$cnt,@$block]);
		      }
		      while (scalar(@$addtextblocks)) {
			my ($index,$block,$cnt)=@{ shift(@$addtextblocks) };
			push(@$todo, [-1,$index,$cnt,@$block]);
		      }
		      
		      $addblock=[];
		      $delblock=[];
		    }
		    push(@$block,$seq2->[$_[1]]);  
		    $cnt++  };

  my $keyfunc = sub { join("  ",split(" ",shift())) };

  traverse_sequences($seq1,$seq2, { MATCH=>$match, DISCARD_A=>$discard, DISCARD_B=>$add }, $keyfunc );


  # now carry out the merging/splitting.  Refer to elements relative from 
  # the end (with negative indices) as these offsets don't change before the instruction is executed
  # cnt>0: merged small unchanged groups with previous changed blocks
  # cnt==-1: split textual commands into components
  foreach $instruction ( @$todo) {
    ($last1,$last2,$cnt,@$block)=@$instruction ;
    if ($cnt>=0) {
      splice(@$seq1,$last1-$len1,1+$cnt,join("",$seq1->[$last1-$len1],@$block)) if $last1>=0;
      splice(@$seq2,$last2-$len2,1+$cnt,join("",$seq2->[$last2-$len2],@$block)) if $last2>=0;
    } else {
      splice(@$seq1,$last1-$len1,1,@$block) if $last1>=0;
      splice(@$seq2,$last2-$len2,1,@$block) if $last2>=0;
    }
  }

  if ($verbose) { 
    print STDERR "\n";
    print STDERR "  $mattokcnt matching  tokens in $matblkcnt blocks.\n";
    print STDERR "  $deltokcnt discarded tokens in $delblkcnt blocks.\n";
    print STDERR "  $addtokcnt appended  tokens in $addblkcnt blocks.\n";
  }
}


# extracttextblocks(\@blockindex)
# $blockindex has the following format 
# [ [ token1, index1 ], [token2, index2],.. ] 
# where index refers to the index in the original old or new word sequence 
# Returns: reference to an array of the form  
# [[ $index, $textblock, $cnt ], ..
# where $index index of block to be merged
#       $textblock contains all the words to be merged with the word at $index (but does not contain this word)
#       $cnt   is length of block
#
# requires: iscmd
#
sub extracttextblocks { 
  my $block=shift;
  my ($i,$token,$index);
  my $textblock=[];
  my $last=-1;
  my $wpat=qr/^(?:[a-zA-Z.,'`:;?()!]*)[\s~]*$/;  #'
  my $retval=[];

  for ($i=0;$i< scalar @$block;$i++) {
    ($token,$index)=@{ $block->[$i] };
    # store pure text blocks
    if ($token =~ /$wpat/ ||  ( $token =~/^\\([\w\d\*]+)((?:${extraspace}\[$brat0\]${extraspace}|${extraspace}\{$pat6\})*)/o 
				&& iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL) 
				&& !iscmd($1,\@TEXTCMDLIST,\@TEXTCMDEXCL))) {
      # we have text or a command which can be treated as text
      if ($last<0) {
	# new pure-text block
	$last=$index;
      } else {
	# add to pure-text block
	push(@$textblock, $token); 
      }
    } else {
      # it is not text
      if (scalar(@$textblock)) {
	push(@$retval,[ $last, $textblock, scalar(@$textblock) ]);
      }
      $textblock=[];
      $last=-1;
    }
  }
  # finish processing a possibly unfinished block before returning
  if (scalar(@$textblock)) {
    push(@$retval,[ $last, $textblock, scalar(@$textblock) ]);
  }
  return($retval)
}



# extractcommands( \@blockindex )
# $blockindex has the following format 
# [ [ token1, index1 ], [token2, index2],.. ] 
# where index refers to the index in the original old or new word sequence 
# Returns: reference to an array of the form  
# [ [ "\cmd1", index, "\cmd1[optarg]{arg1}{", "arg2" ,"} " ],.. 
# where index is just taken from input array 
# command must have a textual argument as last argument 
# 
# requires: iscmd 
# 
sub extractcommands { 
  my $block=shift;
  my ($i,$token,$index,$cmd,$open,$mid,$closing);
  my $retval=[];

  for ($i=0;$i< scalar @$block;$i++) {
    ($token,$index)=@{ $block->[$i] };
    # check if token is an alphanumeric command sequence with at least one non-optional argument
    # \cmd[...]{...}{last argument}  
    # Capturing in the following results in these associations
    # $1: \cmd[...]{...}{
    # $2: \cmd
    # $3: last argument
    # $4: }  + trailing spaces
    if ( ( $token =~ m/^(\\([\w\d\*]+)(?:${extraspace}\[$brat0\]|${extraspace}\{$pat6\})*${extraspace}\{)($pat6)(\}\s*)$/so )
	 && iscmd($2,\@TEXTCMDLIST,\@TEXTCMDEXCL) ) {
      #      push(@$retval,[ $2,$index,$1,$3,$4 ]);
      ($cmd,$open,$mid,$closing) = ($2,$1,$3,$4) ;
      $closing =~ s/\}/\\RIGHTBRACE/ ;
      push(@$retval,[ $cmd,$index,$open,$mid,$closing ]);
    }
  }
  return $retval;
}

# iscmd($cmd,\@regexarray,\@regexexcl) checks
# return 1 if $cmd matches any of the patterns in the 
# array $@regexarray, and none of the patterns in \@regexexcl, otherwise return 0
sub iscmd {
  my ($cmd,$regexar,$regexexcl)=@_;
  my ($ret)=0;
  foreach $pat ( @$regexar ) {
    if ( $cmd =~ m/^${pat}$/ ) {
      $ret=1 ; 
      last;
    }
  }
  return 0 unless $ret;
  foreach $pat ( @$regexexcl ) {
    return 0 if ( $cmd =~ m/^${pat}$/ );
  }
  return 1;
}


# pass2( \@seq1,\@seq2)
# Look for differences between seq1 and seq2.  
# Mark begin and end of deleted and appended sequences with tags $DELOPEN and $DELCLOSE
# and $ADDOPEN and $ADDCLOSE, respectively, however exclude { } & and all comands, unless
# they match an element of the whitelist (SAFECMD)
# For words in TEXTCMD but not in SAFECMD, enclose interior with $ADDOPEN and $ADDCLOSE brackets
# Deleted comment lines are marked with %DIF < 
# Added comment lines are marked with %DIF > 
sub pass2 {
  my $seq1 = shift ;
  my $seq2 = shift ;

  my ($addtokcnt,$deltokcnt,$mattokcnt)=(0,0,0);
  my ($addblkcnt,$delblkcnt,$matblkcnt)=(0,0,0);

  my $retval = [];
  my $delhunk   = [];
  my $addhunk   = [];

  my $discard = sub { $deltokcnt++;
                      push ( @$delhunk, $seq1->[$_[0]]) };

  my $add = sub { $addtokcnt++;
                  push ( @$addhunk, $seq2->[$_[1]]) };

  my $match = sub { $mattokcnt++;
		    if ( scalar @$delhunk ) {
                      $delblkcnt++;
		      # mark up changes, but comment out commands
                      push @$retval,marktags($DELMARKOPEN,$DELMARKCLOSE,$DELOPEN,$DELCLOSE,$DELCMDOPEN,$DELCMDCLOSE,$DELCOMMENT,$delhunk);
		      $delhunk = [];
		    }
                    if ( scalar @$addhunk ) {
                      $addblkcnt++;
                      # we mark up changes, but simply quote commands
                      push @$retval,marktags($ADDMARKOPEN,$ADDMARKCLOSE,$ADDOPEN,$ADDCLOSE,"","",$ADDCOMMENT,$addhunk);
		      $addhunk = [];
		    }
		    push(@$retval,$seq2->[$_[1]]) };
 
  my $keyfunc = sub { join("  ",split(" ",shift())) };

  traverse_sequences($seq1,$seq2, { MATCH=>$match, DISCARD_A=>$discard, DISCARD_B=>$add }, $keyfunc );
  # clear up unprocessed hunks
  push @$retval,marktags($DELMARKOPEN,$DELMARKCLOSE,$DELOPEN,$DELCLOSE,$DELCMDOPEN,$DELCMDCLOSE,$DELCOMMENT,$delhunk) if scalar @$delhunk;
  push @$retval,marktags($ADDMARKOPEN,$ADDMARKCLOSE,$ADDOPEN,$ADDCLOSE,"","",$ADDCOMMENT,$addhunk) if scalar @$addhunk;


  if ($verbose) { 
    print STDERR "\n";
    print STDERR "  $mattokcnt matching  tokens. \n";
    print STDERR "  $deltokcnt discarded tokens in $delblkcnt blocks.\n";
    print STDERR "  $addtokcnt appended  tokens in $addblkcnt blocks.\n";
  }

  return(@$retval);
}

# marktags($openmark,$closemark,$open,$close,$opencmd,$closecmd,$comment,\@block)
# returns ($openmark,$open,$block,$close,$closemark) if @block only contains no commands (except white-listed ones),
# braces, ampersands, or comments
# mark comments with $comment
# exclude all other exceptions from scope of open, close like this
# ($openmark, $open,...,$close, $opencmd,command, command,$closecmd, $open, ..., $close, $closemark)
# If $opencmd begins with "%" marktags assumes it is operating on a deleted block, otherwise on an added block
sub marktags {
  my ($openmark,$closemark,$open,$close,$opencmd,$closecmd,$comment,$block)=@_;
  my $word;
  my (@argtext);
  my $retval=[];
  my $noncomment=0;
  my $cmd=-1;    # -1 at beginning 0: last token written is a ordinary word 
                 # 1: last token written is a command
                # for keeping track whether we are just in a command sequence or in a word sequence
  my $cmdcomment= ($opencmd =~ m/^%/);  # Flag to indicate whether opencmd is a comment (i.e. if we intend to simply comment out changed commands)
  my ($command,$commandword,$closingbracket) ; # temporary variables needed below to remember sub-pattern matches

# split this block to flatten out sequences joined in pass1
  @$block=splitlatex(join "",@$block);
  foreach (@$block) {
    $word=$_; 
    if ( $word =~ s/^%/%$comment/ ) {
      # a comment
      if ($cmd==1) {
	push (@$retval,$closecmd) ;
	$cmd=-1;
      }
      push (@$retval,$word); 
      next;
    }
    if (! $noncomment) {
      push (@$retval,$openmark); 
      $noncomment=1;
    }
    # negative lookahead pattern (?!) in second clause is put in to avoid mathcing \( .. \) patterns
    # also note that second pattern will match \\
    # Note: the second pattern should really be $word =~ /^\\(?!\()(\\|[\w*@]+)/, ie * replaced by +
    # and then all commands \" \' etc declared safe. But as I don't have a complete list of one letter 
    # commands, and nobody has complained so far, I will eave this as is
    if ( $word =~ /^[&{}\[\]]/ || ( $word =~ /^\\(?!\()(\\|[\w*@]*)/ &&  !iscmd($1,\@SAFECMDLIST,\@SAFECMDEXCL)) ) {
      # word is a command or other significant token (not in SAFECMDLIST)
	## same conditions as in subroutine extractcommand:
	# check if token is an alphanumeric command sequence with at least one non-optional argument
	# \cmd[...]{...}{last argument}  
	# Capturing in the following results in these associations
	# $1: \cmd[...]{...}{
	# $2: cmd
	# $3: last argument
	# $4: }  + trailing spaces
	### pre-0.3    if ( ( $token =~ m/^(\\([\w\d\*]+)(?:\[$brat0\]|\{$pat6\})*\{)($pat6)(\}\s*)$/so )
      if ( ( $word =~ m/^(\\([\w\d\*]+)(?:${extraspace}\[$brat0\]|${extraspace}\{$pat6\})*${extraspace}\{)($pat6)(\}\s*)$/so )
	   && (iscmd($2,\@TEXTCMDLIST,\@TEXTCMDEXCL)|| iscmd($2,\@MATHTEXTCMDLIST,\@MATHTEXTCMDEXCL))
           && ( !$cmdcomment || !iscmd($2,\@CONTEXT2CMDLIST, \@CONTEXT2CMDEXCL) )  ) {
	# Condition 1: word is a command? - if yes, $1,$2,.. will be set as above
        # Condition 2: word is a text command - we mark up the interior of the word. There is a separate check for MATHTEXTCMDLIST
        #              because for $mathmarkup=WHOLE, the commands should not be split in pass1 (ie. math mode commands are not in
        #              TEXTCMDLIST, but the interior of MATHTEXT commands should be highlighted in both deleted and added blocks
        # Condition 3: But if we are in a deleted block ($cmdcomment=1) and
        #            $2 (the command) is in context2, just treat it as an ordinary command (i.e. comment it open with $opencmd)
        # Because we do not want to disable this command
	# here we do not use $opencmd and $closecmd($opencmd is empty) 
	if ($cmd==1) {
	  push (@$retval,$closecmd) ;
	} elsif ($cmd==0) { 
	  push (@$retval,$close) ;
	}
        $command=$1; $commandword=$2; $closingbracket=$4;
	@argtext=splitlatex($3);   # split textual argument into tokens
	# and mark it up (but we do not need openmark and closemark)
        # insert command with initial arguments, marked-up final argument, and closing bracket
	if ( $cmdcomment && iscmd($commandword,\@CONTEXT1CMDLIST, \@CONTEXT1CMDEXCL) ) {
	  # context1cmd in a deleted environment; delete command itself but keep last argument, marked up
	  push (@$retval,$opencmd);
	  $command =~ s/\n/\n${opencmd}/sg ; # repeat opencmd at the beginning of each line
	  # argument, note that the additional comment character is included
          # to suppress linebreak after opening parentheses, which is important
          # for latexrevise
          push (@$retval,$command,"%\n{$AUXCMD\n",marktags("","",$open,$close,$opencmd,$closecmd,$comment,\@argtext),$closingbracket);
        } elsif ( iscmd($commandword,,\@MATHTEXTCMDLIST, \@MATHTEXTCMDEXCL) ) {
	  # MATHBLOCK pseudo command: consider all commands safe, except & and \\	
	  # Keep these commands even in deleted blocks, hence set $opencmd and $closecmd (5th and 6th argument of marktags) to 
	  # ""
	  local @SAFECMDLIST=(".*"); 
	  local @SAFECMDEXCL=('\\','\\\\');
	  push(@$retval,$command,marktags("","",$open,$close,"","",$comment,\@argtext)#@argtext
                       ,$closingbracket);
        } else {
	  # normal textcmd or context1cmd in an added block
	  push (@$retval,$command,marktags("","",$open,$close,$opencmd,$closecmd,$comment,\@argtext),$closingbracket);  
	}
	push (@$retval,$AUXCMD,"\n") if $cmdcomment ;
	$cmd=-1 ;
      } else {
	# ordinary command
	push (@$retval,$opencmd) if $cmd==-1 ;
	push (@$retval,$close,$opencmd) if $cmd==0 ;
	$word =~ s/\n/\n${opencmd}/sg if $cmdcomment ;   # if opencmd is a comment, repeat this at the beginning of every line
	push (@$retval,$word);
	$cmd=1;
      }
    } else {
      # just an ordinary word or word in SAFECMD
      push (@$retval,$open) if $cmd==-1 ;
      push (@$retval,$closecmd,$open) if $cmd==1 ;
      push (@$retval,$word);
      $cmd=0;
    }
  }
  push (@$retval,$close) if $cmd==0;
  push (@$retval,$closecmd) if $cmd==1;

  push (@$retval,$closemark) if ($noncomment);
  return @$retval;
}

# preprocess($string, ..)
# carry out the following pre-processing steps for all arguments:
# 1. Remove leading white-space
#    Change \{ to \LEFTBRACE and \} to \RIGHTBRACE
# #. change begin and end commands  within comments to BEGINDIF, ENDDIF
#    so they don't disturb the pattern matching (if there are several \begin or \end in one line
# 2. mark all first empty line (in block of several) with \PAR tokens
# 3. Convert all '\%' into '\PERCENTAGE ' to make parsing regular expressions easier
# 4. Convert all \verb|some verbatim text| commands (where | can be an arbitrary character)
#    into \verb{hash}
# 5. Convert \begin{verbatim} some verbatim text \end{verbatim} into \verbatim{hash}
# 6. Convert _n into \SUBSCRIPTNB{n} and _{nnn} into \SUBSCRIPT{nn}
# 7. Convert ^n into \SUPERSCRIPTNB{n} and ^{nnn} into \SUPERSCRIPT{nn}
# 8. a. Convert $$ $$ into \begin{DOLLARDOLLAR} \end{DOLLARDOLLAR}
#    b. Convert \[ \] into \begin{SQUAREBRACKET} \end{SQUAREBRACKET}
# 9. Convert all picture environmentent (\begin{PICTUREENV} .. \end{PICTUREENV} \PICTUREBLOCKenv
#     For --block-math-markup option -convert all \begin{MATH} .. \end{MATH}
#    into \MATHBLOCKmath{...} commands, where MATH/math is any valid math environment

# 10. Add final token STOP to the very end.  This is put in because the algorithm works better if the last token is identical.  This is removed again in postprocessing.
#
# NB: step 6 and 7 is likely to  convert some "_" inappropriately, e.g. in file
#     names or labels but it does not matter because they are converted back in the postprocessing step
# Returns: leading white space removed in step 1
sub preprocess {
  my @leadin=() ;
  for (@_) { 
    s/^(\s*)//s;
    push(@leadin,$1);
    #    Change \{ to \QLEFTBRACE and \} to \QRIGHTBRACE
    s/(?<!\\)\\{/\\QLEFTBRACE /sg;
    s/(?<!\\)\\}/\\QRIGHTBRACE /sg;
    # change begin and end commands  within comments such that they
    # don't disturb the pattern matching (if there are several \begin or \end in one line
    # this substitution is insufficient but that appears unlikely)
    s/(%.*)\\begin\{(.*)$/$1\\BEGINDIF\{$2/mg ;
    s/(%.*)\\end\{(.*)$/$1\\ENDDIF\{$2/mg ;

    s/\n(\s*?)\n((?:\s*\n)*)/\n$1\\PAR\n$2/g ;
    s/(?<!\\)\\%/\\PERCENTAGE /g ;  # (?<! is negative lookbehind assertion to prevent \\% from being converted
    s/(\\verb\*?)(\S)(.*?)\2/"${1}{". tohash(\%verbhash,"${2}${3}${2}") ."}"/esg;
    s/\\begin\{(verbatim\*?)\}(.*?)\\end\{\1\}/"\\${1}{". tohash(\%verbhash,"${2}") . "}"/esg;
    # Convert _n or _\cmd into \SUBSCRIPTNB{n} or \SUBSCRIPTNB{\cmd} and _{nnn} into \SUBSCRIPT{nn}
    1 while s/_([^{\\]|\\\w+)/\\SUBSCRIPTNB{$1}/g ;
    1 while s/_{($pat6)}/\\SUBSCRIPT{$1}/g ;
    # Convert ^n into \SUPERSCRIPTNB{n} and ^{nnn} into \SUPERSCRIPT{nn}
    1 while s/\^([^{\\]|\\\w+)/\\SUPERSCRIPTNB{$1}/g ;
    1 while s/\^{($pat6)}/\\SUPERSCRIPT{$1}/g ;
    # Convert $$ $$ into \begin{DOLLARDOLLAR} \end{DOLLARDOLLAR}
    s/\$\$(.*?)\$\$/\\begin{DOLLARDOLLAR}$1\\end{DOLLARDOLLAR}/sg;
    # Convert \[ \] into \begin{SQUAREBRACKET} \end{SQUAREBRACKET}
    s/(?<!\\)\\\[/\\begin{SQUAREBRACKET}/sg;
    s/\\\]/\\end{SQUAREBRACKET}/sg;
    # Convert all picture environmentent (\begin{PICTUREENV} .. \end{PICTUREENV} \PICTUREBLOCKenv
    s/\\begin{($PICTUREENV)}(.*?)\\end{\1}/\\PICTUREBLOCK$1\{$2\}/sg;
    #    For --block-math-markup option -convert all \begin{MATH} .. \end{MATH}
    #    into \MATHBLOCKMATH{...} commands, where MATH is any valid math environment
    #    Also convert all array environments into ARRAYBLOCK environments
    if ( $mathmarkup != FINE ) {
      s/\\begin{($ARRENV)}(.*?)\\end{\1}/\\ARRAYBLOCK$1\{$2\}/sg;
      s/\\begin{($MATHENV|$MATHARRENV|SQUAREBRACKET)}(.*?)\\end{\1}/\\MATHBLOCK$1\{$2\}/sg;
    }
    # add final token " STOP"
    $_ .= " STOP"
  }
  return(@leadin);
}

#hashstring=tohash(\%hash,$string)
# creates a hash value based on string and stores in %hash
sub tohash {
  my ($hash,$string)=@_;
  my (@arr,$val);
  my ($sum,$i)=(0,1);
  my ($hstr);

  @arr=unpack('c*',$string);

  foreach $val (@arr) {
    $sum += $i*$val;
    $i++;
  }
  $hstr= "$sum";
  if (defined($hash->{$hstr}) && $string ne $hash->{$hstr}) {
    warn "Repeated hash value for verbatim mode in spite of different content.";
    $hstr="-$hstr";
  }
  $hash->{$hstr}=$string;
  return($hstr);
}

#string=fromhash(\%hash,$fromstring)
# restores string value stored in hash
#string=fromhash(\%hash,$fromstring,$prependstring)
# additionally begins each line with prependstring
sub fromhash {
  my ($hash,$hstr)=($_[0],$_[1]);
  my $retstr=$hash->{$hstr};
  if ( $#_ >= 2) {
    $retstr =~ s/^/$_[2]/mg;
  }
  return $retstr;
}


# postprocess($string, ..)
# carry out the following post-processing steps for all arguments:
# * Remove STOP token from the end
# * Replace \RIGHTBRACE by }
# *  change citation commands within comments to protect from processing (using marker CITEDIF)
# 1. Check all deleted blocks: 
#    a.where a deleted block contains a matching \begin and
#      \end environment (these will be disabled by a %DIFDELCMD statements), for selected environments enable
#      these commands again (such that for example displayed math in a deleted equation
#      is properly within math mode.  For math mode environments replace numbered equation
#      environments with their display only variety (so that equation numbers in new file and
#      diff file are identical).  Where the correct type of math environment cannot be determined
#      use a place holder MATHMODE
#    b.where one of the commands matching $COUNTERCMD is used as a DIFAUXCMD, add a statement
#      subtracting one from the respective counter to keep numbering consistent with new file
#    Replace all MATHMODE environment commands by the correct environment to achieve matching
#    pairs
#    c. Convert MATHBLOCKmath commands to their uncounted numbers (e.g. convert equation -> displaymath
#       (environments defined in $MATHENV will be replaced by $MATHREPL, and  environments in $MATHARRENV
#       will be replaced by $MATHARRREPL
#    d. If in-line math mode contains array environment, enclose the whole environment in \mbox'es
#    d. place \cite commands in mbox'es (for UNDERLINE style)
#
#   For added blocks:
#    c. If in-line math mode contains array environment, enclose the whole environment in \mbox'es
#    d. place \cite commands in mbox'es (for UNDERLINE style)
#     
# 2.   If --block-math-markup option set: Convert \MATHBLOCKmath{..} commands back to environments
#
#      Convert all PICTUREblock{..} commands back to the appropriate environments
# 3. Convert DIFadd, DIFdel, DIFFaddbegin , ... into FL varieties
#    within floats (currently recognised float environments: plate,table,figure
#    plus starred varieties).
# 4. Remove empty %DIFDELCMD < lines 
# 4. Convert \begin{SQUAREBRACKET} \end{SQUAREBRACKET} into \[ \]
#    Convert \begin{DOLLARDOLLAR} \end{DOLLARDOLLAR} into $$ $$
# 5. Convert  \SUPERSCRIPTNB{n} into ^n  and  \SUPERSCRIPT{nn} into ^{nnn}
# 6. Convert  \SUBSCRIPTNB{n} into _n  and  \SUBCRIPT{nn} into _{nnn}
# 7. Expand hashes of verb and verbatim environments
# 8. Convert '\PERCENTAGE ' back into '\%'
# 9.. remove all \PAR tokens
# 10.  package specific processing:  endfloat: make sure \begin{figure} and \end{figure} are always
#      on a line by themselves, similarly for table environment
#  4, undo renaming of the \begin and \end in comments
#    Change \QLEFTBRACE, \QRIGHTBRACE to \{,\}
#
# Note have to manually synchronize substitution commands below and 
# DIF.. command names in the header
sub postprocess {
  my ($begin,$len,$cnt,$float,$delblock,$addblock);
  # second level blocks
  my ($begin2,$cnt2,$len2,$eqarrayblock,$mathblock);

  for (@_) { 

    # change $'s in comments to something harmless
    1 while s/(%.*)\$/$1DOLLARDIF/mg ;

    # Remove final STOP token
    s/ STOP$//;
    # Replace \RIGHTBRACE by }    
    s/\\RIGHTBRACE/}/g;

    # change citation commands within comments to protect from processing
    if ($CITECMD){
      1 while s/(%.*)\\($CITECMD)/$1\\CITEDIF$2/m ;
    }
    # Check all deleted blocks: where a deleted block contains a matching \begin and
    #    \end environment (these will be disabled by a %DIFDELCMD statements), enable
    #    these commands again (such that for example displayed math in a deleted equation
    #    is properly within math mode.  For math mode environments replace numbered equation
    #    environments with their display only variety (so that equation numbers in new file and
    #    diff file are identical
    while ( m/\\DIFdelbegin.*?\\DIFdelend/sg ) {
      $cnt=0;
      $len=length($&);
      $begin=pos($_) - $len;
      $delblock=$&;


      ### (.*?[^\n]?)\n? construct is necessary to avoid empty lines in math mode, which result in
      ### an error
      # displayed math environments
      if ($mathmarkup == FINE ) {
	$delblock=~ s/(\%DIFDELCMD < \s*\\begin\{((?:$MATHENV)|SQUAREBRACKET)\}.*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(\%DIFDELCMD < \s*\\end\{\2\})/\\begin{$MATHREPL}$AUXCMD\n$1$3\n\\end{$MATHREPL}$AUXCMD\n$4/sg;
	# also transform the opposite pair \end{displaymath} .. \begin{displaymath} but we have to be careful not to interfere with the results of the transformation in the line directly above
	### pre-0.42 obsolete version which did not work on eqnarray test      $delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{($MATHENV)\}\s*?\n)(.*?[^\n]?)\n?(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{\2\})/$1\\end{$MATHREPL}$AUXCMD\n$3\n\\begin{$MATHREPL}$AUXCMD\n$4/sg;
	###0.5:      $delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{((?:$MATHENV)|SQUAREBRACKET)\}\s*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{\2\})/\\end{MATHMODE}$AUXCMD\n$1$3\n\\begin{MATHMODE}$AUXCMD\n$4/sg;
	$delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{((?:$MATHENV)|SQUAREBRACKET)\}.*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{\2\})/\\end{MATHMODE}$AUXCMD\n$1$3\n\\begin{MATHMODE}$AUXCMD\n$4/sg;
  
        # now look for unpaired %DIFDELCMD < \begin{MATHENV}; if found add \begin{$MATHREPL} and insert \end{$MATHREPL} 
        # just before end of block; again we use look-behind assertion to avoid matching constructions which have already been converted
        if ($delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{((?:$MATHENV)|SQUAREBRACKET)\}\s*?(?:$DELCMDCLOSE|\n))/$1\\begin{$MATHREPL}$AUXCMD\n/sg ) {
	  $delblock =~ s/(\\DIFdelend$)/\\end{$MATHREPL}$AUXCMD\n$1/s ;
        }
        # now look for unpaired %DIFDELCMD < \end{MATHENV}; if found add \end{MATHMODE} and insert \begin{MATHMODE} 
        # just before end of block; again we use look-behind assertion to avoid matching constructions which have already been converted
        if ($delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{((?:$MATHENV)|SQUAREBRACKET)\}\s*?(?:$DELCMDCLOSE|\n))/$1\\end{MATHMODE}$AUXCMD\n/sg ) {
	  $delblock =~ s/(\\DIFdelend$)/\\begin{MATHMODE}$AUXCMD\n$1/s ;
	}


	### pre-0.42      # same as above for special case \[.\] (latex abbreviation for displaymath)
        ### pre-0.42      $delblock=~ s/(\%DIFDELCMD < \s*\\\[\s*?\n())(.*?[^\n]?)\n?(\%DIFDELCMD < \s*\\\])/$1\\\[$AUXCMD\n$3\n\\\]$AUXCMD\n$4/sg;
        ### pre-0.42      $delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\\]\s*?\n())(.*?[^\n]?)\n?(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\\[)/$1\\\]$AUXCMD\n$3\n\\\[$AUXCMD\n$4/sg;
        # equation array environment
        ###pre-0.3      $delblock=~ s/(\%DIFDELCMD < \s*\\begin\{($MATHARRENV)\}\s*?\n)(.*?)(\%DIFDELCMD < \s*\\end\{\2\})/$1\\begin{$MATHARRREPL}$AUXCMD\n$3\n\\end{$MATHARRREPL}$AUXCMD\n$4/sg;
        ###0.5      $delblock=~ s/(\%DIFDELCMD < \s*\\begin\{($MATHARRENV)\}\s*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(\%DIFDELCMD < \s*\\end\{\2\})/\\begin{$MATHARRREPL}$AUXCMD\n$1$3\n\\end{$MATHARRREPL}$AUXCMD\n$4/sg;
        $delblock=~ s/(\%DIFDELCMD < \s*\\begin\{($MATHARRENV)\}.*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(\%DIFDELCMD < \s*\\end\{\2\})/\\begin{$MATHARRREPL}$AUXCMD\n$1$3\n\\end{$MATHARRREPL}$AUXCMD\n$4/sg;
        ###  pre-0.42 obsolete version which did not work on eqnarray test     $delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{($MATHARRENV)\}\s*?\n)(.*?[^\n]?)\n?(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{\2\})/$1\\end{$MATHARRREPL}$AUXCMD\n$3\n\\begin{$MATHARRREPL}$AUXCMD\n$4/sg;
        $delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{($MATHARRENV)\}\s*?(?:$DELCMDCLOSE|\n))(.*?[^\n]?)\n?(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{\2\})/\\end{MATHMODE}$AUXCMD\n$1$3\n\\begin{MATHMODE}$AUXCMD\n$4/sg;

        # now look for unpaired %DIFDELCMD < \begin{MATHARRENV}; if found add \begin{$MATHARRREPL} and insert \end{$MATHARRREPL} 
        # just before end of block; again we use look-behind assertion to avoid matching constructions which have already been converted
        if ($delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\begin\{($MATHARRENV)\}\s*?(?:$DELCMDCLOSE|\n))/$1\\begin{$MATHARRREPL}$AUXCMD\n/sg ) {
           $delblock =~ s/(\\DIFdelend$)/\\end{$MATHARRREPL}$AUXCMD\n$1/s ;
        }
        # now look for unpaired %DIFDELCMD < \end{MATHENV}; if found add \end{MATHMODE} and insert \begin{MATHMODE} 
        # just before end of block; again we use look-behind assertion to avoid matching constructions which have already been converted
        if ($delblock=~ s/(?<!${AUXCMD}\n)(\%DIFDELCMD < \s*\\end\{($MATHARRENV)\}\s*?(?:$DELCMDCLOSE|\n))/$1\\end{MATHMODE}$AUXCMD\n/sg ) {
	  $delblock =~ s/(\\DIFdelend$)/\\begin{MATHMODE}$AUXCMD\n$1/s ;
        }

      # parse $delblock for deleted and reinstated eqnarray* environments - within those reinstate \\ and & commands
        while ( $delblock =~ m/\\begin\Q{$MATHARRREPL}$AUXCMD\E\n.*?\n\\end\Q{$MATHARRREPL}$AUXCMD\E\n/sg ) {
	  $cnt2=0;
	  $len2=length($&);
	  $begin2=pos($delblock) - $len2;
	  $eqarrayblock=$&;
	  # reinstate deleted & and \\ commands
	  $eqarrayblock=~ s/(\%DIFDELCMD < \s*(\&|\\\\)\s*?(?:$DELCMDCLOSE|\n))/$1$2$AUXCMD\n/sg ;
	  
	  substr($delblock,$begin2,$len2)=$eqarrayblock;
	  pos($delblock) = $begin2 + length($eqarrayblock);
	}
      } elsif ( $mathmarkup == COARSE || $mathmarkup == WHOLE ) {
#       Convert MATHBLOCKmath commands to their uncounted numbers (e.g. convert equation -> displaymath
#       (environments defined in $MATHENV will be replaced by $MATHREPL, and  environments in $MATHARRENV
#       will be replaced by $MATHARRREPL
	$delblock=~ s/\\MATHBLOCK($MATHENV)\{($pat6)\}/\\MATHBLOCK$MATHREPL\{$2\}/sg;
	$delblock=~ s/\\MATHBLOCK($MATHARRENV)\{($pat6)\}/\\MATHBLOCK$MATHARRREPL\{$2\}/sg;
      }


#    b.where one of the commands matching $COUNTERCMD is used as a DIFAUXCMD, add a statement
#      subtracting one from the respective counter to keep numbering consistent with new file
      $delblock=~ s/\\($COUNTERCMD)((?:${extraspace}\[$brat0\]${extraspace}|${extraspace}\{$pat6\})*\s*${AUXCMD}\n)/\\$1$2\\addtocounter{$1}{-1}${AUXCMD}\n/sg ;


#     c. If in-line math mode contains array environment, enclose the whole environment in \mbox'es
      while ( $delblock =~ m/($math)(\s*)/sg ) {
	$cnt2=0;
	$len2=length($&);
	$begin2=pos($delblock) - $len2;
	$mathblock="%\n\\mbox{$AUXCMD\n$1\n}$AUXCMD\n";
        next unless $mathblock =~ m/\{$ARRENV\}/ ;
	substr($delblock,$begin2,$len2)=$mathblock;
	pos($delblock) = $begin2 + length($mathblock);
      }
      if ($CITE2CMD) {
	$delblock=~s/($DELCMDOPEN\s*\\($CITE2CMD)(.*)$DELCMDCLOSE)/
	  # Replacement code 
	  {my ($aux,$all);
	   $aux=$all=$1;
	   $aux=~s#\n?($DELCMDOPEN|$DELCMDCLOSE)##g;
	   $all."$aux$AUXCMD\n";}/sge;
      }
      # or protect \cite commands with \mbox
      if ($CITECMD) {
	$delblock=~s/(\\($CITECMD)${extraspace}(?:\[$brat0\]${extraspace}){0,2}\{$pat6\})(\s*)/\\mbox{$AUXCMD\n$1\n}$AUXCMD\n/msg ;
      } 
#     splice in modified delblock
      substr($_,$begin,$len)=$delblock;
      pos = $begin + length($delblock);
    }
    # make the array modification in added blocks
    while ( m/\\DIFaddbegin.*?\\DIFaddend/sg ) {
      $cnt=0;
      $len=length($&);
      $begin=pos($_) - $len;
      $addblock=$&;
      while ( $addblock =~ m/($math)(\s*)/sg ) {
	$cnt2=0;
	$len2=length($&);
	$begin2=pos($addblock) - $len2;
	$mathblock="%\n\\mbox{$AUXCMD\n$1\n}$AUXCMD\n";
        next unless $mathblock =~ m/\{$ARRENV\}/ ;
	substr($addblock,$begin2,$len2)=$mathblock;
	pos($addblock) = $begin2 + length($mathblock);
      }
      if ($CITECMD) {
	my $addblockbefore=$addblock;
	$addblock=~ s/(\\($CITECMD)${extraspace}(?:\[$brat0\]${extraspace}){0,2}\{$pat2\})(\s*)/\\mbox{$AUXCMD\n$1\n}$AUXCMD\n/msg ;
      }
#     splice in modified addblock
      substr($_,$begin,$len)=$addblock;
      pos = $begin + length($addblock);
    }


    ### old place for BEGINDIF, ENDDIF replacement
    # change begin and end commands  within comments such that they
    # don't disturb the pattern matching (if there are several \begin or \end in one line
    # this substitution is insufficient but that appears unlikely)
    # This needs to be repeated here to also get rid of DIFdelcmd-protected environments
    s/(%.*)\\begin\{(.*)$/$1\\BEGINDIF\{$2/mg ;
    s/(%.*)\\end\{(.*)$/$1\\ENDDIF\{$2/mg ;

    # Replace MATHMODE environments from step 1a above by the correct Math environment

    # The next line is complicated.  The negative look-ahead insertion makes sure that no \end{$MATHENV} (or other mathematical
    # environments) are between the \begin{$MATHENV} and \end{MATHMODE} commands. This is necessary as the minimal matching 
    # is not globally minimal but only 'locally' (matching is beginning from the left side of the string)
    if ( $mathmarkup == FINE ) {
      1 while s/\\begin{((?:$MATHENV)|(?:$MATHARRENV)|SQUAREBRACKET)}((?:.(?!(?:\\end{(?:(?:$MATHENV)|(?:$MATHARRENV)|SQUAREBRACKET)}|\\begin{MATHMODE})))*?)\\end{MATHMODE}/\\begin{$1}$2\\end{$1}/s;
      1 while s/\\begin{MATHMODE}((?:.(?!\\end{MATHMODE}))*?)\\end{((?:$MATHENV)|(?:$MATHARRENV)|SQUAREBRACKET)}/\\begin{$2}$1\\end{$2}/s;
      # convert remaining \begin{MATHMODE} \end{MATHMODE} (and not containing & or \\ )into MATHREPL environments
      s/\\begin{MATHMODE}((?:(.(?!(?<!\\)\&|\\\\))*)?)\\end{MATHMODE}/\\begin{$MATHREPL}$1\\end{$MATHREPL}/sg;
      # others into MATHARRREPL
      s/\\begin{MATHMODE}(.*?)\\end{MATHMODE}/\\begin{$MATHARRREPL}$1\\end{$MATHARRREPL}/sg;

      # now look for AUXCMD math-mode pairs which have only comments (or empty lines between them), and remove the added commands
      s/\\begin{((?:$MATHENV)|(?:$MATHARRENV)|SQUAREBRACKET)}$AUXCMD\n((?:\s*%.[^\n]*\n)*)\\end{\1}$AUXCMD\n/$2/sg;       
    } else {
      #   math modes OFF,WHOLE,COARSE: Convert \MATHBLOCKmath{..} commands back to environments
      s/\\MATHBLOCK($MATHENV|$MATHARRENV|SQUAREBRACKET)\{($pat6)\}/\\begin{$1}$2\\end{$1}/sg;
      # convert ARRAYBLOCK.. commands back to environments
      s/\\ARRAYBLOCK($ARRENV)\{($pat6)\}/\\begin{$1}$2\\end{$1}/sg;
    }
    #  Convert all PICTUREblock{..} commands back to the appropriate environments
    s/\\PICTUREBLOCK($PICTUREENV)\{($pat6)\}/\\begin{$1}$2\\end{$1}/sg;
#0.5:    # Remove all mark up within picture environments
#     while ( m/\\begin\{($PICTUREENV)\}.*?\\end\{\1\}/sg ) {
#       $cnt=0;
#       $len=length($&);
#       $begin=pos($_) - $len;
#       $float=$&;
#       $float =~ s/\\DIFaddbegin //g;
#       $float =~ s/\\DIFaddend //g;
#       $float =~ s/\\DIFadd\{($pat6)\}/$1/g;
#       $float =~ s/\\DIFdelbegin //g;
#       $float =~ s/\\DIFdelend //g;
#       $float =~ s/\\DIFdel\{($pat6)\}//g;
#       $float =~ s/$DELCMDOPEN.*//g;
#       substr($_,$begin,$len)=$float;
#       pos = $begin + length($float);
#     }
    # Convert DIFadd, DIFdel, DIFFaddbegin , ... into  varieties
    #    within floats (currently recognised float environments: plate,table,figure
    #    plus starred varieties).
    while ( m/\\begin\{($FLOATENV)\}.*?\\end\{\1\}/sg ) {
      $cnt=0;
      $len=length($&);
      $begin=pos($_) - $len;
      $float=$&;
      $float =~ s/\\DIFaddbegin /\\DIFaddbeginFL /g;
      $float =~ s/\\DIFaddend /\\DIFaddendFL /g;
      $float =~ s/\\DIFadd\{/\\DIFaddFL{/g;
      $float =~ s/\\DIFdelbegin /\\DIFdelbeginFL /g;
      $float =~ s/\\DIFdelend /\\DIFdelendFL /g;
      $float =~ s/\\DIFdel\{/\\DIFdelFL{/g;
      substr($_,$begin,$len)=$float;
      pos = $begin + length($float);
    }
    ### former location of undo renaming of \begin and \end in comments

    # remove empty DIFCMD < lines
    s/^\Q${DELCMDOPEN}\E\n//msg;

    # Expand hashes of verb and verbatim environments (note negative look behind assertion to not leak out of DIFDELCMD comments
    s/(\\verb\*?)\{([-\d]*?)\}/"${1}". fromhash(\%verbhash,$2)/esg;
    s/${DELCMDOPEN}\\(verbatim\*?)\{([-\d]*?)\}/"${DELCMDOPEN}\\begin{${1}}".fromhash(\%verbhash,$2,$DELCMDOPEN)."${DELCMDOPEN}\\end{${1}}"/esg;
    s/\\(verbatim\*?)\{([-\d]*?)\}/"\\begin{${1}}".fromhash(\%verbhash,$2)."\\end{${1}}"/esg;
    # Convert '\PERCENTAGE ' back into '\%'			       
    s/\\PERCENTAGE /\\%/g;
    # remove all \PAR tokens (taking care to properly keep commented out PAR's
    # from introducing uncommented newlines - next line)
    s/(%DIF < )([^\n]*?)\\PAR\n/$1$2\n$1\n/sg;
    # convert PAR commands which are on a line by themselves
    s/\n(\s*?)\\PAR\n/\n\n/sg;
    # convert remaining PAR commands (which are preceded by non-white space characters, usually "}" ($ADDCLOSE)
    s/\\PAR\n/\n\n/sg;

    #  package specific processing: 
    if ( defined($packages{"endfloat"})) {
      #endfloat: make sure \begin{figure} and \end{figure} are always
      #      on a line by themselves, similarly for table environment
      print STDERR "endfloat package detected.\n" if $verbose ;
      # eliminate whitespace before and after
      s/^(\s*)(\\(?:begin|end)\{(?:figure|table)\})(\s*)$/$2/mg;
      # split lines with remaining characters before float enviroment conmmand
      s/^(.+)(\\(?:begin|end)\{(?:figure|table)\})/$1\n$2/mg;
      # split lines with remaining characters after float enviroment conmmand
      s/(\\(?:begin|end)\{(?:figure|table)\})(.+)$/$1\n$2/mg;
    }
    # undo renaming of the \begin and \end  and dollars in comments 
    s/(%.*)\\BEGINDIF\{(.*)$/$1\\begin\{$2/mg ;
    s/(%.*)\\ENDDIF\{(.*)$/$1\\end\{$2/mg ;
    1 while s/(%.*)DOLLARDIF/$1\$/mg ;
    # undo renaming of the \cite.. commands in comments 
    if ( $CITECMD ) {
      1 while s/(%.*)\\CITEDIF($CITECMD)/$1\\$2/mg ;
    }
#   Convert \begin{SQUAREBRACKET} \end{SQUAREBRACKET} into \[ \]
    s/\\end{SQUAREBRACKET}/\\\]/sg;
    s/\\begin{SQUAREBRACKET}/\\\[/sg;
# 4. Convert \begin{DOLLARDOLLAR} \end{DOLLARDOLLAR} into $$ $$
    s/\\begin\{DOLLARDOLLAR\}(.*?)\\end\{DOLLARDOLLAR\}/\$\$$1\$\$/sg;
# 5. Convert  \SUPERSCRIPTNB{n} into ^n  and  \SUPERSCRIPT{nn} into ^{nnn}
    1 while s/\\SUPERSCRIPTNB{($pat0)}/^$1/g ;
    1 while s/\\SUPERSCRIPT{($pat6)}/^{$1}/g ;
    # Convert  \SUBSCRIPNB{n} into _n  and  \SUBCRIPT{nn} into _{nnn}
    1 while s/\\SUBSCRIPTNB{($pat0)}/_$1/g ;
    1 while s/\\SUBSCRIPT{($pat6)}/_{$1}/g ;
#    Change \QLEFTBRACE, \QRIGHTBRACE to \{,\}
    s/\\QLEFTBRACE /\\{/sg;
    s/\\QRIGHTBRACE /\\}/sg;

  return;
  }
}


# @auxlines=preprocess_preamble($oldpreamble,$newpreamble);
  # pre-process preamble by looking for commands used in \maketitle (title, author, date etc commands) 
  # if found then use a bodydiff to mark up content, and replace the corresponding commands 
  # in both preambles by marked up version to 'fool' the linediff (such that only body is marked
  # up.
  # A special case are e.g. author commands being added (or removed)
  # 1. If commands are added, then the entire content is marked up as new, but also the lines are marked as new in the linediff
  # 2. If commands are removed, then the linediff will mark the line as deleted.  The program returns 
  #    with $auxlines a text to be appended at the end of the preamble, which shows the respective fields as deleted
sub preprocess_preamble {
  my ($oldpreambleref,$newpreambleref)=(\$_[0],\$_[1]) ;
  my @auxlines=();
  # Remember to use $$oldpreambleref to refer to oldpreamble
  my ($titlecmd,$titlecmdpat);
  my (@oldtitlecommands,@newtitlecommands );
  my  %oldhash  = ();
  my  %newhash  = ();
  my ($line,$cmd,$optarg,$arg,$optargnew,$optargold,$optargdiff,$argold,$argnew,$argdiff,$auxline);

  # resuse context2cmdlist to define these commands to  look out for in preamble
  $titlecmd = "(?:".join("|",@CONTEXT2CMDLIST).")";
  # as context2cmdlist is stored as regex, e.g. ((?-xism:^title$), we need to remove ^- fo
  # resue in a more complex regex
  $titlecmd =~ s/[\$\^]//g; 
  # make sure to not match on comment lines:
  $titlecmdpat=qr/^(?:[^%\n]|\\%)*(\\($titlecmd)$extraspace(?:\[($brat0)\])?(?:\{($pat6)\}))/ms;
  @oldtitlecommands= ( $$oldpreambleref =~ m/$titlecmdpat/g );
  @newtitlecommands= ( $$newpreambleref =~ m/$titlecmdpat/g );


  while ( @oldtitlecommands ) {
    $line=shift @oldtitlecommands;
    $cmd=shift @oldtitlecommands;
    $optarg=shift @oldtitlecommands;
    $arg=shift @oldtitlecommands;
  
    if ( defined($oldhash{$cmd})) {
      warn "$cmd is used twice in preamble of old file. Reverting to pure line diff mode for preamble.\n";
      return;
    }
    $oldhash{$cmd}=[ $line, $optarg, $arg ];
  }
  while ( @newtitlecommands ) {
    $line=shift @newtitlecommands;
    $cmd=shift @newtitlecommands;
    $optarg=shift @newtitlecommands;
    $arg=shift @newtitlecommands;
  
    if ( defined($newhash{$cmd})) {
      warn "$cmd is used twice in preamble of new file. Reverting to pure line diff mode for preamble.\n";
      return;
    }
    $newhash{$cmd}=[ $line, $optarg, $arg ];
  }
  foreach $cmd ( keys %newhash ) {
    if ( defined($newhash{$cmd}->[1])) {
       $optargnew=$newhash{$cmd}->[1];
    } else {
      $optargnew="";
    }
    if ( defined($oldhash{$cmd}->[1])) {
       $optargold=$oldhash{$cmd}->[1];
    } else {
      $optargold="";
    }

    if ( defined($oldhash{$cmd}) ) {
      $argold=$oldhash{$cmd}->[2];
    } else {
      $argold="";
    }
    $argnew=$newhash{$cmd}->[2];
    $argdiff="{" . join("",bodydiff($argold,$argnew)) ."}";
    if ( length $optargnew ) {
      $optargdiff="[".join("",bodydiff($optargold,$optargnew))."]" ;
      $optargdiff =~ s/\\DIFaddbegin /\\DIFaddbeginFL /g;
      $optargdiff =~ s/\\DIFaddend /\\DIFaddendFL /g;
      $optargdiff =~ s/\\DIFadd\{/\\DIFaddFL{/g;
      $optargdiff =~ s/\\DIFdelbegin /\\DIFdelbeginFL /g;
      $optargdiff =~ s/\\DIFdelend /\\DIFdelendFL /g;
      $optargdiff =~ s/\\DIFdel\{/\\DIFdelFL{/g;
    } else {
      $optargdiff="";
    }
    ### print STDERR "DEBUG s/\\Q$newhash{$cmd}->[0]\\E/\\$cmd$optargdiff$argdiff/s\n";
    # Note: \Q and \E force literal interpretation of what it between them but allow 
    #      variable interpolation, such that e.g. \title matches just that and not TAB-itle
    $$newpreambleref=~s/\Q$newhash{$cmd}->[0]\E/\\$cmd$optargdiff$argdiff/s;
    # replace this in old preamble if necessary
    if ( defined($oldhash{$cmd}->[0])) {
      $$oldpreambleref=~s/\Q$oldhash{$cmd}->[0]\E/\\$cmd$optargdiff$argdiff/s ;
    }
    ### print STDERR "DEBUG NEW PRE ".$$newpreambleref."\n";
  }

  foreach $cmd ( keys %oldhash ) {
    # if this has already been dealt with above can just skip
    next if defined($newhash{$cmd}) ;
    if ( defined($oldhash{$cmd}->[1])) {
      $optargold=$oldhash{$cmd}->[1];
      $optargdiff="[".join("",bodydiff($optargold,""))."]" ;
      $optargdiff =~ s/\\DIFdelbegin /\\DIFdelbeginFL /g;
      $optargdiff =~ s/\\DIFdelend /\\DIFdelendFL /g;
      $optargdiff =~ s/\\DIFdel\{/\\DIFdelFL{/g;
    } else {
      $optargdiff="";
    }
    $argdiff="{" . join("",bodydiff($argold,"")) ."}";
    $auxline = "\\$cmd$optargdiff$argdiff";
    $auxline =~s/$/$AUXCMD/sg;
    push @auxlines,$auxline;
  }
  # add auxcmd comment to highlight added lines
  return(@auxlines);
}



# @diffs=linediff(\@seq1, \@seq2)
# mark up lines like this
#%DIF mm-mmdnn
#%< old deleted line(s)
#%DIF -------
#%DIF mmann-nn
#new appended line %< 
#%DIF -------
# Future extension: mark change explicitly
# Assumes: traverse_sequence traverses deletions before insertions in changed sequences
#          all line numbers relative to line 0 (first line of real file)
sub linediff {
  my $seq1 = shift ;
  my $seq2 = shift ;

  my $block = [];
  my $retseq = [];
  my @begin=('','',''); # dummy initialisation
  my $instring ; 

  my $discard = sub { @begin=('d',$_[0],$_[1]) unless scalar @$block ; 
                      push(@$block, "%DIF < " . $seq1->[$_[0]]) };
  my $add = sub { if (! scalar  @$block) {
		    @begin=('a',$_[0],$_[1]) ;}
		  elsif ( $begin[0] eq 'd' ) {
                    $begin[0]='c'; $begin[2]=$_[1];
		    push(@$block, "%DIF -------") }
                  push(@$block,  $seq2->[$_[1]] . " %DIF > " ) };
  my $match = sub { if ( scalar @$block ) {
                      if ( $begin[0] eq 'd' && $begin[1]!=$_[0]-1) {
			$instring = sprintf "%%DIF %d-%dd%d",$begin[1],$_[0]-1,$begin[2]; }
		      elsif ( $begin[0] eq 'a' && $begin[2]!=$_[1]-1) {
			$instring = sprintf "%%DIF %da%d-%d",$begin[1],$begin[2],$_[1]-1; }
		      elsif ( $begin[0] eq 'c' ) {
			$instring = sprintf "%%DIF %sc%s",
			                     ($begin[1]==$_[0]-1) ? "$begin[1]" : $begin[1]."-".($_[0]-1)  , 
			                     ($begin[2]==$_[1]-1) ? "$begin[2]" : $begin[2]."-".($_[1]-1)  ; }
		      else {
			$instring = sprintf "%%DIF %d%s%d",$begin[1],$begin[0],$begin[2]; }
		      push @$retseq, $instring,@$block, "%DIF -------" ; 
		      $block = []; 
		    }
		    push @$retseq, $seq2->[$_[1]]
		  };
  # key function: remove multiple spaces (such that insertion or deletion of redundant white space is not reported)
  my $keyfunc = sub { join("  ",split(" ",shift())) };

  traverse_sequences($seq1,$seq2, { MATCH=>$match, DISCARD_A=>$discard, DISCARD_B=>$add }, $keyfunc );
  push @$retseq, @$block if scalar @$block; 

  return wantarray ? @$retseq : $retseq ;
}



# init_regex_arr_data(\@array,"TOKEN INIT")
# scans DATA file handel for line "%% TOKEN INIT" line
# then appends each line not beginning with % into array (as a quoted regex)
sub init_regex_arr_data {
  my ($arr,$token)=@_;
  my ($copy);
  while (<DATA>) {
    if ( m/^%%BEGIN $token\s*$/ ) {
      $copy=1; }
    elsif ( m/^%%END $token\s*/ )  {
      last; }
    chomp;
    push (@$arr,qr/^$_$/) if ( $copy && !/^%/ ) ;
  }
  seek DATA,0,0;    # rewind DATA handle to file begin
}


# init_regex_arr_ext(\@array,$arg)
# fills array with regular expressions.
# if arg is a file name, then read in list of regular expressions from that file
# (one expression per line)
# Otherwise treat arg as a comma separated list of regular expressions
sub init_regex_arr_ext {
  my ($arr,$arg)=@_;
  my $regex;
  if ( -f $ arg ) {
    open(FILE,"$arg") or die ("Couldn't open $arg: $!");
    while (<FILE>) {
      chomp;
      next if /^\s*#/ || /^\s*%/ || /^\s*$/ ;
      push (@$arr,qr/^$_$/);
    }
    close(FILE);
  }
  else {
    # assume it is a comma-separated list of reg-ex
    foreach $regex (split(qr/(?<!\\),/,$arg)) {
      $regex =~ s/\\,/,/g;
      push (@$arr,qr/^$regex$/);
    }
  }
}

#exetime() returns time since last execution of this command
#exetime(1) resets this time
my $lasttime=-1;   # global variable for persistence
sub exetime {
  my $reset=0;
  my $retval;
  if ((scalar @_) >=1) {
    $reset=shift;
  }
  if ($reset) {
    $lasttime=times();
  }
  else {
    $retval=times()-$lasttime;
    $lasttime=$lasttime+$retval;
    return($retval);
  }
}


sub usage {
  die <<"EOF"; 
Usage: $0 [options] old.tex new.tex > diff.tex

Compares two latex files and writes tex code to stdout, which has the same
format as new.tex but has all changes relative to old.tex marked up or commented.

--type=markupstyle
-t markupstyle         Add code to preamble for selected markup style
                       Available styles: UNDERLINE CTRADITIONAL TRADITIONAL CFONT FONTSTRIKE INVISIBLE 
                                         CHANGEBAR CCHANGEBAR CULINECHBAR CFONTCBHBAR
                       [ Default: UNDERLINE ]

--subtype=markstyle
-s markstyle           Add code to preamble for selected style for bracketing
                       commands (e.g. to mark changes in  margin)
                       Available styles: SAFE MARGINAL DVIPSCOL COLOR
                       [ Default: SAFE ]

--floattype=markstyle
-f markstyle           Add code to preamble for selected style which 
                       replace standard marking and markup commands within floats
                       (e.g., marginal remarks cause an error within floats
                       so marginal marking can be disabled thus)
                       Available styles: FLOATSAFE IDENTICAL
                       [ Default: FLOATSAFE ]

--encoding=enc
-e enc                 Specify encoding of old.tex and new.tex. Typical encodings are
                       ascii, utf8, latin1, latin9.  A list of available encodings can be 
                       obtained by executing 
                       perl -MEncode -e 'print join ("\\n",Encode->encodings( ":all" )) ;'
                       [Default encoding is utf8 unless the first few lines of the preamble contain
                       an invocation "\\usepackage[..]{inputenc} in which case the 
                       encoding chosen by this command is asssumed. Note that ASCII (standard
                       latex) is a subset of utf8]

--preamble=file
-p file                Insert file at end of preamble instead of auto-generating
                       preamble.  The preamble must define the following commands
                       \\DIFaddbegin,\\DIFaddend,\\DIFadd{..},
                       \\DIFdelbegin,\\DIFdelend,\\DIFdel{..},
                       and varieties for use within floats
                       \\DIFaddbeginFL,\\DIFaddendFL,\\DIFaddFL{..},
                       \\DIFdelbeginFL,\\DIFdelendFL,\\DIFdelFL{..}
                       (If this option is set -t, -s, and -f options
                       are ignored.)

--exclude-safecmd=exclude-file
--exclude-safecmd="cmd1,cmd2,..."
-A exclude-file 
--replace-safecmd=replace-file
--append-safecmd=append-file
--append-safecmd="cmd1,cmd2,..."
-a append-file         Exclude from, replace or append to the list of regex
                       matching commands which are safe to use within the 
                       scope of a \\DIFadd or \\DIFdel command.  The file must contain
                       one Perl-RegEx per line (Comment lines beginning with # or % are
                       ignored). A literal comma within the comma-separated list must be
                       escaped thus "\\,",   Note that the RegEx needs to match the whole of 
                       the token, i.e., /^regex\$/ is implied and that the initial
                       "\\" of the command is not included. The --exclude-safecmd
                       and --append-safecmd options can be combined with the --replace-safecmd 
                       option and can be used repeatedly to add cumulatively to the lists.

--exclude-textcmd=exclude-file 
--exclude-textcmd="cmd1,cmd2,..."
-X exclude-file
--replace-textcmd=replace-file
--append-textcmd=append-file
--append-textcmd="cmd1,cmd2,..."
-x append-file         Exclude from, replace or append to the list of regex
                       matching commands whose last argument is text.  See
                       entry for --exclude-safecmd directly above for further details.

--replace-context1cmd=replace-file
--append-context1cmd=append-file
--append-context1cmd="cmd1,cmd2,..."
                       Replace or append to the list of regex matching commands
                       whose last argument is text but which require a particular
                       context to work, e.g. \\caption will only work within a figure
                       or table.  These commands behave like text commands, except when 
                       they occur in a deleted section, when they are disabled, but their
                       argument is shown as deleted text.

--replace-context2cmd=replace-file
--append-context2cmd=append-file
--append-context2cmd="cmd1,cmd2,..."
                       As corresponding commands for context1.  The only difference is that
                       context2 commands are completely disabled in deleted sections, including
                       their arguments.


--config var1=val1,var2=val2,...
-c var1=val1,..        Set configuration variables.
-c configfile           Available variables: 
                          MINWORDSBLOCK (integer)
                          FLOATENV (RegEx)
                          PICTUREENV (RegEx)
                          MATHENV (RegEx)
                          MATHREPL (String)
                          MATHARRENV (RegEx)
                          MATHARRREPL (String)
                          ARRENV (RegEx)
                          COUNTERCMD (RegEx)
                       This option can be repeated.


--packages=pkg1,pkg2,..
                       Tell latexdiff that .tex file is processed with the packages in list 
                       loaded.  This is normally not necessary if the .tex file includes the
                       preamble, as the preamble is automatically scanned for \\usepackage commands.
                       Use of the --packages option disables automatic scanning, so if for any
                       reason package specific parsing needs to be switched off, use --packages=none.
                       The following packages trigger special behaviour:
                       endfloat hyperref amsmath
                       [ Default: scan the preamble for \\usepackage commands to determine
                         loaded packages.]

--show-preamble        Print generated or included preamble commands to stdout.

--show-safecmd         Print list of regex matching and excluding safe commands.

--show-textcmd         Print list of regex matching and excluding commands with text argument.

--show-config          Show values of configuration variables

--show-all             Show all of the above

   NB For all --show commands, no old.tex or new.tex file needs to be given, and no 
      differencing takes place.

Other configuration options:

--allow-spaces         Allow spaces between bracketed or braced arguments to commands
                       [Default requires arguments to directly follow each other without 
                                intervening spaces]

--math-markup=level    Determine granularity of markup in displayed math environments:
                      Possible values for level are (both numerical and text labels are acceptable):
                      off or 0: suppress markup for math environments.  Deleted equations will not 
                               appear in diff file. This mode can be used if all the other modes 
                               cause invalid latex code.
                      whole or 1: Differencing on the level of whole equations. Even trivial changes
                               to equations cause the whole equation to be marked changed.  This 
                               mode can be used if processing in coarse or fine mode results in 
                               invalid latex code.
                      coarse or 2: Detect changes within equations marked up with a coarse
                               granularity; changes in equation type (e.g.displaymath to equation) 
                               appear as a change to the complete equation. This mode is recommended
                               for situations where the content and order of some equations are still
                               being changed. [Default]
                      fine or 3: Detect small change in equations and mark up and fine granularity.
                               This mode is most suitable, if only minor changes to equations are
                               expected, e.g. correction of typos. 

--disable-citation-markup  Suppress citation markup in styles using ulem (UNDERLINE, 
                       FONTSTRIKE, CULINECHBAR)
--enable-citation-markup   Protect citation commands in changed sections with \\mbox command
                       [i.e. use default behaviour for ulem package for other packages]

Miscelleneous options

--label=label
-L label               Sets the labels used to describe the old and new files.  The first use
                       of this option sets the label describing the old file and the second
                       use of the option sets the label for the new file.
                       [Default: use the filename and modification dates for the label]

--no-label             Suppress inclusion of old and new file names as comment in output file

--visble-label         Include old and new filenames (or labels set with --label option) as 
                       visible output

--flatten              Replace \\input and \\include commands within body by the content
                       of the files in their argument.  If \\includeonly is present in the
                       preamble, only those files are expanded into the document. However, 
                       no recursion is done, i.e. \\input and \\include commands within 
                       included sections are not expanded.  The included files are assumed to 
                       be located in the same directories as the old and new master files,
                       respectively, making it possible to organise files into old and new directories.
                       --flatten is applied recursively, so inputted files can contain further
                       \\input statements.

--help
-h                     Show this help text.

--ignore-warnings      Suppress warnings about inconsistencies in length between input
                       and parsed strings and missing characters. 

--verbose
-V                     Output various status information to stderr during processing.
                       Default is to work silently.

--version              Show version number.

For further information, consult   http://latexdiff.berlios.de
EOF
}

=head1 NAME

latexdiff - determine and markup differences between two latex files

=head1 SYNOPSIS

B<latexdiff> [ B<OPTIONS> ] F<old.tex> F<new.tex> > F<diff.tex>

=head1 DESCRIPTION

Briefly, I<latexdiff> is a utility program to aid in the management of
revisions of latex documents. It compares two valid latex files, here
called C<old.tex> and C<new.tex>, finds significant differences
between them (i.e., ignoring the number of white spaces and position
of line breaks), and adds special commands to highlight the
differences.  Where visual highlighting is not possible, e.g. for changes
in the formatting, the differences are
nevertheless marked up in the source.

The program treats the preamble differently from the main document.
Differences between the preambles are found using line-based
differencing (similarly to the Unix diff command, but ignoring white
spaces).  A comment, "S<C<%DIF E<gt>>>" is appended to each added line, i.e. a 
line present in C<new.tex> but not in C<old.tex>.  Discarded lines 
 are deactivated by prepending "S<C<%DIF E<lt>>>". Changed blocks are preceded  by
comment lines giving information about line numbers in the original files.  Where there are insignificant
differences, the resulting file C<diff.tex> will be similar to
C<new.tex>.  At the end of the preamble, the definitions for I<latexdiff> markup commands are inserted.
In differencing the main body of the text, I<latexdiff> attempts to
satisfy the following guidelines (in order of priority):

=over 3

=item 1

If both C<old.tex> and C<new.tex> are valid LaTeX, then the resulting
C<diff.tex> should also be valid LateX. (NB If a few plain TeX commands
are used within C<old.tex> or C<new.tex> then C<diff.tex> is not
guaranteed to work but usually will).

=item 2

Significant differences are determined on the level of
individual words. All significant differences, including differences
between comments should be clearly marked in the resulting source code
C<diff.tex>.

=item 3

If a changed passage contains text or text-producing commands, then
running C<diff.tex> through LateX should produce output where added
and discarded passages are highlighted.

=item 4

Where there are insignificant differences, e.g. in the positioning of
line breaks, C<diff.tex> should follow the formatting of C<new.tex>

=back

For differencing the same algorithm as I<diff> is used but words
instead of lines are compared.  An attempt is made to recognize
blocks which are completely changed such that they can be marked up as a unit.
Comments are differenced line by line
but the number of spaces within comments is ignored. Commands including
all their arguments are generally compared as one unit, i.e., no mark-up
is inserted into the arguments of commands.  However, for a selected
number of commands (for example, C<\caption> and all sectioning
commands) the last argument is known to be text. This text is
split into words and differenced just as ordinary text (use options to
show and change the list of text commands, see below). As the
algorithm has no detailed knowledge of LaTeX, it assumes all pairs of
curly braces immediately following a command (i.e. a sequence of
letters beginning with a backslash) are arguments for that command.
As a restriction to condition 1 above it is thus necessary to surround
all arguments with curly braces, and to not insert
extraneous spaces.  For example, write 

  \section{\textem{This is an emphasized section title}}

and not

  \section {\textem{This is an emphasized section title}}

or

  \section\textem{This is an emphasized section title}

even though all varieties are the same to LaTeX (but see
B<--allow-spaces> option which allows the second variety).

For environments whose content does not conform to standard LaTeX or
where graphical markup does not make sense all markup commands can be
removed by setting the PICTUREENV configuration variable, set by
default to C<picture> and C<DIFnomarkup> environments; see B<--config>
option).  The latter environment (C<DIFnomarkup>) can be used to
protect parts of the latex file where the markup results in illegal
markup. You have to surround the offending passage in both the old and
new file by C<\begin{DIFnomarkup}> and C<\end{DIFnomarkup}>. You must
define the environment in the preambles of both old and new
documents. I prefer to define it as a null-environment,

C<\newenvironment{DIFnomarkup}{}{}>

but the choice is yours.  Any markup within the environment will be
removed, and generally everything within the environment will just be
taken from the new file.

It is also possible to difference files which do not have a preamble. 
 In this case, the file is processed in the main document
mode, but the definitions of the markup commands are not inserted.

All markup commands inserted by I<latexdiff> begin with "C<\DIF>".  Added
blocks containing words, commands or comments which are in C<new.tex>
but not in C<old.tex> are marked by C<\DIFaddbegin> and C<\DIFaddend>.
Discarded blocks are marked by C<\DIFdelbegin> and C<\DIFdelend>.
Within added blocks all text is highlighted with C<\DIFadd> like this:
C<\DIFadd{Added text block}>
Selected `safe' commands can be contained in these text blocks as well
(use options to show and change the list of safe commands, see below).
All other commands as well as braces "{" and "}" are never put within
the scope of C<\DIFadd>.  Added comments are marked by prepending
"S<C<%DIF E<gt> >>".

Within deleted blocks text is highlighted with C<\DIFdel>.  Deleted
comments are marked by prepending "S<C<%DIF E<lt> >>".  Non-safe command
and curly braces within deleted blocks are commented out with 
"S<C<%DIFDELCMD E<lt> >>".



=head1 OPTIONS

=head2 Preamble

The following options determine the visual markup style by adding the appropriate
command definitions to the preamble. See the end of this section for a description of 
available styles.

=over 4

=item B<--type=markupstyle> or
B<-t markupstyle>

Add code to preamble for selected markup style. This option defines
C<\DIFadd> and C<\DIFdel> commands.
Available styles: 

C<UNDERLINE CTRADITIONAL TRADITIONAL CFONT FONTSTRIKE INVISIBLE 
CHANGEBAR CCHANGEBAR CULINECHBAR CFONTCBHBAR>

[ Default: C<UNDERLINE> ]

=item B<--subtype=markstyle> or
B<-s markstyle> 

Add code to preamble for selected style for bracketing
commands (e.g. to mark changes in  margin). This option defines
C<\DIFaddbegin>, C<\DIFaddend>, C<\DIFdelbegin> and C<\DIFdelend> commands.
Available styles: C<SAFE MARGINAL COLOR DVIPSCOL>

[ Default: C<SAFE> ]

=item B<--floattype=markstyle> or
B<-f markstyle>

Add code to preamble for selected style which 
replace standard marking and markup commands within floats
(e.g., marginal remarks cause an error within floats
so marginal marking can be disabled thus). This option defines all 
C<\DIF...FL> commands.
Available styles: C<FLOATSAFE TRADITIONALSAFE IDENTICAL>

[ Default: C<FLOATSAFE> ]

=item B<--encoding=enc> or 
B<-e enc>

Specify encoding of old.tex and new.tex. Typical encodings are
C<ascii>, C<utf8>, C<latin1>, C<latin9>.  A list of available encodings can be 
obtained by executing 

C<perl -MEncode -e 'print join ("\n",Encode->encodings( ":all" )) ;' >

[Default encoding is utf8 unless the first few lines of the preamble contain
an invocation C<\usepackage[..]{inputenc}> in which case the 
encoding chosen by this command is asssumed. Note that ASCII (standard
latex) is a subset of utf8]

=item B<--preamble=file> or
B<-p file>

Insert file at end of preamble instead of generating
preamble.  The preamble must define the following commands
C<\DIFaddbegin, \DIFaddend, \DIFadd{..},
\DIFdelbegin,\DIFdelend,\DIFdel{..},>
and varieties for use within floats
C<\DIFaddbeginFL, \DIFaddendFL, \DIFaddFL{..},
\DIFdelbeginFL, \DIFdelendFL, \DIFdelFL{..}>
(If this option is set B<-t>, B<-s>, and B<-f> options
are ignored.)

=item B<--packages=pkg1,pkg2,..> 

Tell latexdiff that .tex file is processed with the packages in list
loaded.  This is normally not necessary if the .tex file includes the
preamble, as the preamble is automatically scanned for C<\usepackage> commands.
Use of the B<--packages> option disables automatic scanning, so if for any
reason package specific parsing needs to be switched off, use B<--packages=none>.
The following packages trigger special behaviour:

=over 8

=item C<amsmath> 

Configuration variable amsmath is set to C<align*> (Default: C<eqnarray*>)

=item C<endfloat> 

Ensure that C<\begin{figure}> and C<\end{figure}> always appear by themselves on a line.

=item C<hyperref>

Change name of C<\DIFadd> and C<\DIFdel> commands to C<\DIFaddtex> and C<\DIFdeltex> and 
define new C<\DIFadd> and C<\DIFdel> commands, which provide a wrapper for these commands,
using them for the text but not for the link defining command (where any markup would cause
errors).

=back

[ Default: scan the preamble for C<\\usepackage> commands to determine
  loaded packages.]



=item B<--show-preamble>

Print generated or included preamble commands to stdout.

=back

=head2 Configuration

=over 4

=item B<--exclude-safecmd=exclude-file> or
B<-A exclude-file> or  B<--exclude-safecmd="cmd1,cmd2,...">

=item B<--replace-safecmd=replace-file>

=item B<--append-safecmd=append-file> or 
B<-a append-file> or B<--append-safecmd="cmd1,cmd2,...">

Exclude from, replace or append to the list of regular expressions (RegEx)
matching commands which are safe to use within the 
scope of a C<\DIFadd> or C<\DIFdel> command.  The file must contain
one Perl-RegEx per line (Comment lines beginning with # or % are
ignored).  Note that the RegEx needs to match the whole of 
the token, i.e., /^regex$/ is implied and that the initial
"\" of the command is not included. 
The B<--exclude-safecmd> and B<--append-safecmd> options can be combined with the -B<--replace-safecmd> 
option and can be used repeatedly to add cumulatively to the lists.
 B<--exclude-safecmd>
and B<--append-safecmd> can also take a comma separated list as input. If a
comma for one of the regex is required, escape it thus "\,". In most cases it
will be necessary to protect the comma-separated list from the shell by putting
it in quotation marks.

=item B<--exclude-textcmd=exclude-file> or
B<-X exclude-file> or B<--exclude-textcmd="cmd1,cmd2,...">

=item B<--replace-textcmd=replace-file>

=item B<--append-textcmd=append-file> or 
B<-x append-file> or B<--append-textcmd="cmd1,cmd2,...">

Exclude from, replace or append to the list of regular expressions
matching commands whose last argument is text.  See
entry for B<--exclude-safecmd> directly above for further details.


=item B<--replace-context1cmd=replace-file> 

=item B<--append-context1cmd=append-file> or
=item B<--append-context1cmd="cmd1,cmd2,...">

Replace or append to the list of regex matching commands
whose last argument is text but which require a particular
context to work, e.g. \caption will only work within a figure
or table.  These commands behave like text commands, except when 
they occur in a deleted section, when they are disabled, but their
argument is shown as deleted text.

=item B<--replace-context2cmd=replace-file> 

=item B<--append-context2cmd=append-file> or
=item B<--append-context2cmd="cmd1,cmd2,...">
As corresponding commands for context1.  The only difference is that
context2 commands are completely disabled in deleted sections, including
their arguments.



=item B<--config var1=val1,var2=val2,...> or B<-c var1=val1,..>

=item B<-c configfile>

Set configuration variables.  The option can be repeated to set different
variables (as an alternative to the comma-separated list).
Available variables (see below for further explanations): 

C<MINWORDSBLOCK> (integer)

C<FLOATENV> (RegEx)

C<PICTUREENV> (RegEx)

C<MATHENV> (RegEx)

C<MATHREPL> (String)

C<MATHARRENV> (RegEx)

C<MATHARRREPL> (String)

C<ARRENV> (RegEx)

C<COUNTERCMD> (RegEx)

=item B<--show-safecmd>

Print list of RegEx matching and excluding safe commands.

=item B<--show-textcmd>

Print list of RegEx matching and excluding commands with text argument.

=item B<--show-config>

Show values of configuration variables.

=item B<--show-all>

Combine all --show commands.

NB For all --show commands, no C<old.tex> or C<new.tex> file needs to be specified, and no 
differencing takes place.

=back

=head2 Other configuration options:

=over 4

=item B<--allow-spaces>

Allow spaces between bracketed or braced arguments to commands.  Note
that this option might have undesirable side effects (unrelated scope
might get lumpeded with preceding commands) so should only be used if the
default produces erroneous results.  (Default requires arguments to
directly follow each other without intervening spaces).

=item B<--math-markup=level>   

Determine granularity of markup in displayed math environments:               
Possible values for level are (both numerical and text labels are acceptable):

C<off> or C<0>: suppress markup for math environments.  Deleted equations will not 
appear in diff file. This mode can be used if all the other modes 
cause invalid latex code.

C<whole> or C<1>: Differencing on the level of whole equations. Even trivial changes
to equations cause the whole equation to be marked changed.  This 
mode can be used if processing in coarse or fine mode results in 
invalid latex code.

C<coarse> or C<2>: Detect changes within equations marked up with a coarse
granularity; changes in equation type (e.g.displaymath to equation) 
appear as a change to the complete equation. This mode is recommended
for situations where the content and order of some equations are still
being changed. [Default]

C<fine> or C<3>: Detect small change in equations and mark up at fine granularity.
This mode is most suitable, if only minor changes to equations are
expected, e.g. correction of typos. 

=item B<--disable-citation-markup>

Suppress citation markup in styles using ulem (UNDERLINE, 
FONTSTRIKE, CULINECHBAR)

=item B<--enable-citation-markup>

Protect citation commands in changed sections with \\mbox command [i.e. use default behaviour for ulem package for other packages]

=back

=head2 Miscellaneous

=over 4
=item B<--verbose> or B<-V>

Output various status information to stderr during processing.
Default is to work silently.

=item B<--driver=type>

Choose driver for changebar package (only relevant for styles using
   changebar: CCHANGEBAR CFONTCHBAR CULINECHBAR CHANGEBAR). Possible
drivers are listed in changebar manual, e.g. pdftex,dvips,dvitops
  [Default: dvips]

=item B<--ignore-warnings>

Suppress warnings about inconsistencies in length between input and
parsed strings and missing characters.  These warning messages are
often related to non-standard latex or latex constructions with a
syntax unknown to C<latexdiff> but the resulting difference argument
is often fully functional anyway, particularly if the non-standard
latex only occurs in parts of the text which have not changed.

=item B<--label=label> or
B<-L label>

Sets the labels used to describe the old and new files.  The first use
of this option sets the label describing the old file and the second
use of the option sets the label for the new file, i.e. set both
labels like this C<-L labelold -L labelnew>.
[Default: use the filename and modification dates for the label]

=item B<--no-label>

Suppress inclusion of old and new file names as comment in output file

=item B<--visble-label>

Include old and new filenames (or labels set with --label option) as 
visible output.

=item B<--flatten>

Replace C<\input> and C<\include> commands within body by the content
of the files in their argument.  If C<\includeonly> is present in the
preamble, only those files are expanded into the document. However, 
no recursion is done, i.e. C<\input> and C<\include> commands within 
included sections are not expanded.  The included files are assumed to 
 be located in the same directories as the old and new master files,
respectively, making it possible to organise files into old and new directories. 
--flatten is applied recursively, so inputted files can contain further
C<\input> statements.

Use of this option might result in prohibitive processing times for
larger documents, and the resulting difference document
no longer reflects the structure of the input documents.

=item B<--help> or
B<-h>

Show help text

=item B<--version>

Show version number

=back



=head2 Predefined styles 

=head2 Major types

The major type determine the markup of plain text and some selected latex commands outside floats by defining the markup commands C<\DIFadd{...}> and C<\DIFdel{...}> .

=over 10

=item C<UNDERLINE>

Added text is wavy-underlined and blue, discarded text is struck out and red
(Requires color and ulem packages).  Overstriking does not work in displayed math equations such that deleted parts of equation are underlined, not struck out (this is a shortcoming inherent to the ulem package).

=item C<CTRADITIONAL>

Added text is blue and set in sans-serif, and a red footnote is created for each discarded 
piece of text. (Requires color package)

=item C<TRADITIONAL>

Like C<CTRADITIONAL> but without the use of color.

=item C<CFONT>

Added text is blue and set in sans-serif, and discarded text is red and very small size.

=item C<FONTSTRIKE>

Added tex is set in sans-serif, discarded text small and struck out

=item C<CCHANGEBAR>

Added text is blue, and discarded text is red.  Additionally, the changed text is marked with a bar in the margin (Requires color and changebar packages).

=item C<CFONTCHBAR>

Like C<CFONT> but with additional changebars (Requires color and changebar packages).

=item C<CULINECHBAR>

Like C<UNDERLINE> but with additional changebars (Requires color, ulem and changebar packages).

=item C<CHANGEBAR>

No mark up of text, but mark margins with changebars (Requires changebar package).

=item C<INVISIBLE>

No visible markup (but generic markup commands will still be inserted.

=back

=head2 Subtypes

The subtype defines the commands that are inserted at the begin and end of added or discarded blocks, irrespectively of whether these blocks contain text or commands (Defined commands: C<\DIFaddbegin, \DIFaddend, \DIFdelbegin, \DIFdelend>) 

=over 10

=item C<SAFE>

No additional markup (Recommended choice)

=item C<MARGIN>

Mark beginning and end of changed blocks with symbols in the margin nearby (using
the standard C<\marginpar> command - note that this sometimes moves somewhat
from the intended position.

=item C<COLOR>

An alternative way of marking added passages in blue, and deleted ones in red.
(It is recommeneded to use instead the main types to effect colored markup,
although in some cases coloring with dvipscol can be more complete, for example 
with citation commands).

=item C<DVIPSCOL>

An alternative way of marking added passages in blue, and deleted ones in red. Note
that C<DVIPSCOL> only works with the dvips converter, e.g. not pdflatex.
(it is recommeneded to use instead the main types to effect colored markup,
although in some cases coloring with dvipscol can be more complete).

=back

=head2 Float Types

Some of the markup used in the main text might cause problems when used within 
floats (e.g. figures or tables).  For this reason alternative versions of all
markup commands are used within floats. The float type defines these alternative commands.

=over 10

=item C<FLOATSAFE>

Use identical markup for text as in the main body, but set all commands marking the begin and end of changed blocks to null-commands.  You have to choose this float type if your subtype is C<MARGIN> as C<\marginpar> does not work properly within floats.

=item C<TRADITIONALSAFE>

Mark additions the same way as in the main text.  Deleted environments are marked by angular brackets \[ and \] and the deleted text is set in scriptscript size. This float type should always be used with the C<TRADITIONAL> and  C<CTRADITIONAL> markup types as the \footnote command does not work properly in floating environments.

=item C<IDENTICAL>

Make no difference between the main text and floats.

=back


=head2 Configuration Variables

=over 10

=item C<MINWORDSBLOCK>

Minimum number of tokens required to form an independent block. This value is
used in the algorithm to detect changes of complete blocks by merging identical text parts of less than C<MINWORDSBLOCK> to the preceding added and discarded parts.

[ Default: 3 ]

=item C<FLOATENV>

Environments whose name matches the regular expression in C<FLOATENV> are 
considered floats.  Within these environments, the I<latexdiff> markup commands
are replaced by their FL variaties.

[ Default: S<C<(?:figure|table|plate)[\w\d*@]*> >]

=item C<PICTUREENV>

Within environments whose name matches the regular expression in C<PICTUREENV>
all latexdiff markup is removed (in pathologic cases this might lead to
 inconsistent markup but this situation should be rare).

[ Default: S<C<(?:picture|DIFnomarkup)[\w\d*@]*> >]

=item C<MATHENV>,C<MATHREPL>

If both \begin and \end for a math environment (environment name matching C<MATHENV>
or \[ and \])
are within the same deleted block, they are replaced by a \begin and \end commands for C<MATHREPL>
rather than being commented out.

[ Default: C<MATHENV>=S<C<(?:displaymath|equation)> >, C<MATHREPL>=S<C<displaymath> >]

=item C<MATHARRENV>,C<MATHARRREPL>

as C<MATHENV>,C<MATHREPL> but for equation arrays

[ Default: C<MATHARRENV>=S<C<eqnarray\*?> >, C<MATHREPL>=S<C<eqnarray> >]

=item C<ARRENV>

If a match to C<ARRENV> is found within an inline math environment within a deleted or added block, then the inlined math 
is surrounded by C<\mbox{>...C<}>.  This is necessary as underlining does not work within inlined array environments.

[ Default: C<ARRENV>=S<C<(?:array|[pbvBV]matrix)> >

=item C<COUNTERCMD>

If a command in a deleted block which is also in the textcmd list matches C<COUNTERCMD> then an
additional command C<\addtocounter{>F<cntcmd>C<}{-1}>, where F<cntcmd> is the matching command, is appended in the diff file such that the numbering in the diff file remains synchronized with the
numbering in the new file.

[ Default: C<COUNTERCMD>=C<(?:footnote|part|section|subsection> ...

C<|subsubsection|paragraph|subparagraph)>  ]

=back

=head1 COMMON PROBLEMS

=over 10

=item Citations result in overfull boxes

There is an incompatibility between the C<ulem> package, which C<latexdiff> uses for underlining and striking out in the UNDERLINE style,
the default style. In order to be able to mark up citations properly, they are placed with an C<\mbox> command in post-processing. As mboxes
cannot be broken across lines, this procedure frequently results in overfull boxes, possibly obscuring the content as it extends beyond the right margin. If this is a problem, you have two possibilities:

1. Use C<COLOR> or C<DVIPSCOL> subtype markup (option C<-s COLOR>): If this markup is chosen, then changed citations are no longer marked up
with the wavy line (additions) or struck out (deletions), but are still highlighted in the appropriate color.

2. Choose option C<--disable-citation-markup> which turns off the marking up of citations: deleted citations are no longer shown, and
added ctations are shown without markup. (This was the default behaviour of latexdiff at versions 0.6 and older)

=item Changes in complicated mathematical equations result in latex processing errors

Try options C<--math-markup=whole>.   If even that fails, you can turn off mark up for equations with C<--math-markup=off>.

=back

=head1 BUGS

Option allow-spaces not implemented entirely consistently. It breaks
the rules that number and type of white space does not matter, as
different numbers of inter-argument spaces are treated as significant.

Please submit bug reports on the latexdiff project page I<http://latexdiff.berlios.de>, 
send them to user discussion list C<latexdiff-users@lists.berlios,de> (prior subscription 
to list required, also on project webpage)
or send them to I<tilmann@gfz-potsdam.de>.  Include the serial number of I<latexdiff>
(from comments at the top of the source or use B<--version>).  If you come across latex
files that are error-free and conform to the specifications set out
above, and whose differencing still does not result in error-free
latex, please send me those files, ideally edited to only contain the
offending passage as long as that still reproduces the problem. If your 
file relies on non-standard class files, you must include those.  I will not
look at examples where I have trouble to latex the original files.

=head1 SEE ALSO

L<latexrevise>, L<latexdiff-vc>

=head1 PORTABILITY

I<latexdiff> does not make use of external commands and thus should run
on any platform  supporting Perl 5.6 or higher.  If files with encodings 
other than ASCII or UTF-8 are processed, Perl 5.8 or higher is required.

The standard version of I<latexdiff> requires installation of the Perl package
C<Algorithm::Diff> (available from I<www.cpan.org> - 
I<http://search.cpan.org/~nedkonz/Algorithm-Diff-1.15>) but a stand-alone
version, I<latexdiff-so>, which has this package inlined, is available, too.
I<latexdiff-fast> requires the I<diff> command to be present.

=head1 AUTHOR

Version 1.0.2
Copyright (C) 2004-2012 Frederik Tilmann

This program is free software; you can redistribute it and/or modify
it under the terms of the GNU General Public License Version 3

Contributors of fixes and additions: V. Kuhlmann, J. Paisley, N. Becker, T. Doerges, K. Huebner, 
T. Connors, Sebastian Gouezel and many others.
Thanks to the many people who send in bug reports, feature suggestions, and other feedback.

=cut

__END__
%%BEGIN SAFE COMMANDS
% Regex matching commands which can safely be in the
% argument of a \DIFadd or \DIFdel command (leave out the \)
arabic
dashbox
emph
fbox
framebox
hspace
math.*
makebox
mbox
pageref
ref
symbol
raisebox
rule
text.*
shortstack
usebox
dag
ddag
copyright
pounds
S
P
oe
OE
ae
AE
aa
AA
o
O
l
L
frac
ss
sqrt
ldots
cdots
vdots
ddots
alpha
beta
gamma
delta
epsilon
varepsilon
zeta
eta
theta
vartheta
iota
kappa
lambda
mu
nu
xi
pi
varpi
rho
varrho
sigma
varsigma
tau
upsilon
phi
varphi
chi
psi
omega
Gamma
Delta
Theta
Lambda
Xi
Pi
Sigma
Upsilon
Phi
Psi
Omega
ps
mp
times
div
ast
star
circ
bullet
cdot
cap
cup
uplus
sqcap
vee
wedge
setminus
wr
diamond
(?:big)?triangle.*
lhd
rhd
unlhd
unrhd
oplus
ominus
otimes
oslash
odot
bigcirc
d?dagger
amalg
leq
prec
preceq
ll
(?:sq)?su[bp]set(?:eq)?
in
vdash
geq
succ(?:eq)?
gg
ni
dashv
equiv
sim(?:eq)?
asymp
approx
cong
neq
doteq
propto
models
perp
mid
parallel
bowtie
Join
smile
frown
.*arrow
(?:long)?mapsto
.*harpoon.*
leadsto
aleph
hbar
imath
jmath
ell
wp
Re
Im
mho
prime
emptyset
nabla
surd
top
bot
angle
forall
exists
neg
flat
natural
sharp
backslash
partial
infty
Box
Diamond
triangle
clubsuit
diamondsuit
heartsuit
spadesuit
sum
prod
coprod
int
oint
big(?:sq)?c[au]p
bigvee
bigwedge
bigodot
bigotimes
bigoplus
biguplus
(?:arc)?(?:cos|sin|tan|cot)h?
csc
arg
deg
det
dim
exp
gcd
hom
inf
ker
lg
lim
liminf
limsup
ln
log
max
min
Pr
sec
sup
(SUPER|SUB)SCRIPTNB
(SUPER|SUB)SCRIPT
%%END SAFE COMMANDS

%%BEGIN TEXT COMMANDS
% Regex matching commands with a text argument (leave out the \)
addcontents.*
cc
closing
chapter
dashbox
emph
encl
fbox
framebox
footnote
footnotetext
framebox
part
(sub){0,2}section\*?
(sub)?paragraph\*?
makebox
mbox
opening
parbox
raisebox
savebox
sbox
shortstack
signature
text.*
value
underline
sqrt
(SUPER|SUB)SCRIPT
%%END TEXT COMMANDS 

%%BEGIN CONTEXT1 COMMANDS
% Regex matching commands with a text argument (leave out the \), which will fail out of context, but whose argument should be printed as plain text
caption
%%END CONTEXT1 COMMANDS 

%%BEGIN CONTEXT2 COMMANDS
% Regex matching commands with a text argument (leave out the \), which will fail out of context, but whose argument should be printed as plain text
title
author
date
institute
%%END CONTEXT2 COMMANDS 


%% TYPES (Commands for highlighting changed blocks)

%DIF UNDERLINE PREAMBLE
\RequirePackage[normalem]{ulem}
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{{\protect\color{blue}\uwave{#1}}}
\providecommand{\DIFdel}[1]{{\protect\color{red}\sout{#1}}}                     
%DIF END UNDERLINE PREAMBLE

%DIF CTRADITIONAL PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\RequirePackage[stable]{footmisc}
\providecommand{\DIFadd}[1]{{\protect\color{blue} \sf #1}}
\providecommand{\DIFdel}[1]{{\protect\color{red} [..\footnote{removed: #1} ]}}
%DIF END CTRADITIONAL PREAMBLE

%DIF TRADITIONAL PREAMBLE
\RequirePackage[stable]{footmisc}
\providecommand{\DIFadd}[1]{{\sf #1}}
\providecommand{\DIFdel}[1]{{[..\footnote{removed: #1} ]}}
%DIF END TRADITIONAL PREAMBLE

%DIF CFONT PREAMBLE
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{{\protect\color{blue} \sf #1}}
\providecommand{\DIFdel}[1]{{\protect\color{red} \scriptsize #1}}
%DIF END CFONT PREAMBLE

%DIF FONTSTRIKE PREAMBLE
\RequirePackage[normalem]{ulem}
\providecommand{\DIFadd}[1]{{\sf #1}}
\providecommand{\DIFdel}[1]{{\footnotesize \sout{#1}}}
%DIF END FONTSTRIKE PREAMBLE

%DIF CCHANGEBAR PREAMBLE
\RequirePackage[dvips]{changebar}
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{\protect\cbstart{\protect\color{blue}#1}\protect\cbend}
\providecommand{\DIFdel}[1]{\protect\cbdelete{\protect\color{red}#1}\protect\cbdelete}
%DIF END CCHANGEBAR PREAMBLE

%DIF CFONTCHBAR PREAMBLE
\RequirePackage[dvips]{changebar}
\RequirePackage{color}\definecolor{RED}{rgb}{1,0,0}\definecolor{BLUE}{rgb}{0,0,1}
\providecommand{\DIFadd}[1]{\protect\cbstart{\protect\color{blue}\sf #1}\protect\cbend}
\providecommand{\DIFdel}[1]{\protect\cbdelete{\protect\color{red}\scriptsize #1}\protect\cbdelete}
%DIF END CFONTCHBAR PREAMBLE

%DIF CULINECHBAR PREAMBLE
\RequirePackage[normalem]{ulem}
\RequirePackage[dvips]{changebar}
\RequirePackage{color}
\providecommand{\DIFadd}[1]{\protect\cbstart{\protect\color{blue}\uwave{#1}}\protect\cbend}
\providecommand{\DIFdel}[1]{\protect\cbdelete{\protect\color{red}\sout{#1}}\protect\cbdelete}
%DIF END CULINECHBAR PREAMBLE

%DIF CHANGEBAR PREAMBLE
\RequirePackage[dvips]{changebar}
\providecommand{\DIFadd}[1]{\protect\cbstart{#1}\protect\cbend}
\providecommand{\DIFdel}[1]{\protect\cbdelete}
%DIF END CHANGEBAR PREAMBLE

%DIF INVISIBLE PREAMBLE
\providecommand{\DIFadd}[1]{#1}
\providecommand{\DIFdel}[1]{}
%DIF END INVISIBLE PREAMBLE


%% SUBTYPES (Markers for beginning and end of changed blocks)

%DIF SAFE PREAMBLE
\providecommand{\DIFaddbegin}{}
\providecommand{\DIFaddend}{}
\providecommand{\DIFdelbegin}{}
\providecommand{\DIFdelend}{}
%DIF END SAFE PREAMBLE

%DIF MARGIN PREAMBLE
\providecommand{\DIFaddbegin}{\protect\marginpar{a[}}
\providecommand{\DIFaddend}{\protect\marginpar{]}}
\providecommand{\DIFdelbegin}{\protect\marginpar{d[}}
\providecommand{\DIFdelend}{\protect\marginpar{]}}
%DIF END BRACKET PREAMBLE

%DIF DVIPSCOL PREAMBLE
%Note: only works with dvips converter
\RequirePackage{color}
\RequirePackage{dvipscol}
\providecommand{\DIFaddbegin}{\protect\nogroupcolor{blue}}
\providecommand{\DIFaddend}{\protect\nogroupcolor{black}}
\providecommand{\DIFdelbegin}{\protect\nogroupcolor{red}}
\providecommand{\DIFdelend}{\protect\nogroupcolor{black}}
%DIF END DVIPSCOL PREAMBLE

%DIF COLOR PREAMBLE
\RequirePackage{color}
\providecommand{\DIFaddbegin}{\protect\color{blue}}
\providecommand{\DIFaddend}{\protect\color{black}}
\providecommand{\DIFdelbegin}{\protect\color{red}}
\providecommand{\DIFdelend}{\protect\color{black}}
%DIF END COLOR PREAMBLE


%% FLOAT TYPES 

%DIF FLOATSAFE PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{}
\providecommand{\DIFaddendFL}{}
\providecommand{\DIFdelbeginFL}{}
\providecommand{\DIFdelendFL}{}
%DIF END FLOATSAFE PREAMBLE

%DIF IDENTICAL PREAMBLE
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdelFL}[1]{\DIFdel{#1}}
\providecommand{\DIFaddbeginFL}{\DIFaddbegin}
\providecommand{\DIFaddendFL}{\DIFaddend}
\providecommand{\DIFdelbeginFL}{\DIFdelbegin}
\providecommand{\DIFdelendFL}{\DIFdelend}
%DIF END IDENTICAL PREAMBLE

%DIF TRADITIONALSAFE PREAMBLE
% procidecommand color to make this work for TRADITIONAL and CTRADITIONAL
\providecommand{\color}[1]{}
\providecommand{\DIFaddFL}[1]{\DIFadd{#1}}
\providecommand{\DIFdel}[1]{{\protect\color{red}[..{\scriptsize {removed: #1}} ]}}
\providecommand{\DIFaddbeginFL}{}
\providecommand{\DIFaddendFL}{}
\providecommand{\DIFdelbeginFL}{}
\providecommand{\DIFdelendFL}{}
%DIF END FLOATSAFE PREAMBLE

%% SPECIAL PACKAGE PREAMBLE COMMANDS

% Standard \DIFadd and \DIFdel are redefined as \DIFaddtex and \DIFdeltex
% when hyperref package is included.
%DIF HYPERREF PREAMBLE
\providecommand{\DIFadd}[1]{\texorpdfstring{\DIFaddtex{#1}}{#1}}
\providecommand{\DIFdel}[1]{\texorpdfstring{\DIFdeltex{#1}}{}}
%DIF END HYPERREF PACKAGE


==> LHCbInternal/Scripts/trunk/python/lblatexdiff <==
#!/usr/bin/env python
# $Id: $
"""This script finds the difference between two LHCb documents"""
from sys import argv
from os import listdir, symlink, unlink
from os.path import join, abspath, expanduser
from optparse import OptionParser
from tempfile import mkdtemp
from subprocess import call
from shutil import copyfile, rmtree

def test():
    pass

import inspect, os.path
scriptpath =  os.path.dirname(inspect.getsourcefile(test))


class DiffLHCbError(Exception):
    """Exception class for DiffLHCb"""
    pass


class DiffLHCb:
    """Find differences between LHCb documents"""
    def __init__(self,options):
        self.options = options
        
        # Directory where diff will be located
        self.diffdirname = mkdtemp()

        # Setup old and new directories
        if self.options.svn:
            self._svn()
        else:
            self.olddirname=abspath(expanduser(self.options.old))
            self.newdirname=abspath(expanduser(self.options.new))

        for item in listdir(self.newdirname):
            symlink(join(self.newdirname,item), join(self.diffdirname,item))

        self.latexfile=self.options.name+'.tex'

    def _shell(self, command):
        """Execute shell command and throw exception if an error occurs"""
        rc = call(command, shell=True)
        if rc != 0:
            self._clean()
            err = "{0!r} failed with return code {1}."
            raise DiffLHCbError(err.format(command,rc)) 

    def _svn(self):
        """Check out documents from SVN if required"""
        svnhead=join('svn+ssh://svn.cern.ch/reps/lhcbdocs',self.options.svn)
        self.oldco=mkdtemp()
        self.newco=mkdtemp()

        self._shell('svn co '+ join(svnhead,self.options.old) + " " + 
                    self.oldco)
                  
        self._shell('svn co '+ join(svnhead,self.options.new) + " " + 
                    self.newco)
        
        self.olddirname=self.oldco
        self.newdirname=self.newco

    def _clean(self):
        
        if self.options.svn:
            for d in [self.oldco,self.newco]:
                rmtree(d)
        
    def diff(self):
        
        self.oldfname=join(self.olddirname,self.latexfile)
        self.newfname=join(self.newdirname,self.latexfile)

        self._shell('cd '+self.diffdirname+'; make clean')
        unlink(join(self.diffdirname,self.latexfile))

        self._shell(join(scriptpath,'latexdiff') + ' --flatten ' + 
                    self.oldfname+' '+self.newfname+
                    ' > ' + join(self.diffdirname,self.latexfile))

    def latex(self):
        self._shell('cd '+self.diffdirname+'; make')

        pdf = join(self.diffdirname,self.options.name)+'.pdf'
        print '*'*50
        print 'Difference PDF file is at : '+pdf

if __name__ == '__main__':

    import os,sys
    
    usage = """usage: %prog [options] old [new]

Find the difference between two versions of an LHCb document. If no
new location is given, the current directory is used. The location of
the old version can either be given as a directory or as a location in
SVN. The toplevel is by default taken as main.tex. See options for how
to change this.

Compare the version in the current directory with the one in the
draft3 directory given as a relative path

lblatexdiff ../../draft3/latex


Compare draft v1r3 to the latest version in SVN

lblatexdiff --svn=Publications/PAPER/2012/011 drafts/v1r3/latex  latest/latex
"""
    parser = OptionParser(usage=usage)

    parser.add_option("-s", "--svn", dest="svn",
                      default = None,
                      help="Document in lhcbdocs to make comparison for "+ \
                          "like Publications/PAPER/2012/011", 
                      metavar="DIR")

    options, args = parser.parse_args()

    if len(args)<1 or len(args)>2:
        print "{0} takes one or two arguments.\n".format(parser.get_prog_name())
        parser.print_help()
        sys.exit(0)

    options.name = 'main'

    options.old=args[0]
    if len(args) == 2:
        options.new=args[1]
    else:
        options.new='.'

    try:
        differ = DiffLHCb(options)
        differ.diff()
        differ.latex()
        differ._clean()
    except DiffLHCbError, detail:
        print detail
        print "Run with option --help to see syntax."


==> LHCbInternal/acknowledgements_template.tex <==
\section{Acknowledgements}
We thank Ian Moult, Kyle Lee, Bianka Me\c{c}aj, and Evan Craft for helpful discussions. We express our gratitude to our colleagues in the CERN accelerator departments for the excellent performance of the LHC. We thank the technical and administrative staff at the LHCb institutes.
We acknowledge support from CERN and from the national agencies:
ARC (Australia);
CAPES, CNPq, FAPERJ and FINEP (Brazil); 
MOST and NSFC (China); 
CNRS/IN2P3 and CEA (France);  % added CEA 26/02/2026
BMFTR, DFG and MPG (Germany);
INFN (Italy); 
NWO (Netherlands); 
MNiSW and NCN (Poland); 
MEC/IFA (Romania); 
%MSHE (Russia); 
MICIU and AEI (Spain);
SNSF and SER (Switzerland); 
NASU (Ukraine); 
STFC (United Kingdom); 
DOE NP and NSF (USA).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We acknowledge the computing resources that are provided by ARDC (Australia), 
CBPF (Brazil),
CERN, 
IHEP and LZU (China),
IN2P3 (France), 
KIT and DESY (Germany), 
INFN (Italy), 
SURF (Netherlands),
Polish WLCG (Poland),
IFIN-HH (Romania), % http://dx.doi.org/10.13039/100019931,"Institutul National de Cercetare-Dezvoltare pentru Fizica si Inginerie Nucleara 'Horia Hulubei'"
%RRCKI and Yandex LLC (Russia), 
PIC (Spain), CSCS (Switzerland), 
GridPP (United Kingdom),
and NSF (USA).  % added Feb2026
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
We are indebted to the communities behind the multiple open-source
software packages on which we depend.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Individual groups or members have received support from
% ARC and ARDC (Australia); % moved to national 16/01/2025
RTP (Australia), % added 06/03/2026
FWO Odysseus grant G0ASD25N (Belgium), % added 20/4/2026
Key Research Program of Frontier Sciences of CAS, CAS PIFI, CAS CCEPP (China); 
%Fundamental Research Funds for the Central Universities,  and Sci.\
%\& Tech.\ Program of Guangzhou (China); Removed 24/11/25
Minciencias (Colombia);
EPLANET, Marie Sk\l{}odowska-Curie Actions, ERC and NextGenerationEU (European Union);
A*MIDEX, ANR, IPhU and Labex P2IO, and R\'{e}gion Auvergne-Rh\^{o}ne-Alpes (France);
%RFBR, RSF and Yandex LLC (Russia);
Alexander-von-Humboldt Foundation (Germany);
ICSC (Italy); 
%GVA, XuntaGal, GENCAT, Inditex, InTalent and Prog.~Atracci\'on Talento, CM (Spain);
Severo Ochoa and Mar\'ia de Maeztu Units of Excellence, GVA, XuntaGal, GENCAT, InTalent-Inditex and Prog.~Atracci\'on Talento CM (Spain);
%XuntaGal --> Xunta de Galicia 
% SRC (Sweden);  % removed 27/02/2026 - end of grant
the Leverhulme Trust, the Royal Society and UKRI (United Kingdom).
\input{LHCb/acknowledgements}



==> LHCbInternal/lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script python listsymbols.py

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash belletwo} & \belletwo & \texttt{\textbackslash besiii} & \besiii & \texttt{\textbackslash cleo} & \cleo \\
\texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero & \texttt{\textbackslash aleph} & \aleph \\
\texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal & \texttt{\textbackslash lthree} & \lthree \\
\texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern & \texttt{\textbackslash lhc} & \lhc \\
\texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron & \texttt{\textbackslash bfactories} & \bfactories \\
\texttt{\textbackslash bfactory} & \bfactory & \texttt{\textbackslash upgradeone} & \upgradeone & \texttt{\textbackslash upgradetwo} & \upgradetwo \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash herschel} & \herschel \\
\texttt{\textbackslash spd} & \spd & \texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal \\
\texttt{\textbackslash hcal} & \hcal & \texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown \\
\texttt{\textbackslash ode} & \ode & \texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc \\
\texttt{\textbackslash ecs} & \ecs & \texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt \\
\texttt{\textbackslash hltone} & \hltone & \texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash emp} & \emp & \texttt{\textbackslash epem} & \epem \\
\texttt{\textbackslash muon} & \muon & \texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun \\
\texttt{\textbackslash mupm} & \mupm & \texttt{\textbackslash mump} & \mump & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash taupm} & \taupm & \texttt{\textbackslash taump} & \taump & \texttt{\textbackslash tautau} & \tautau \\
\texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm & \texttt{\textbackslash ellp} & \ellp \\
\texttt{\textbackslash ellpm} & \ellpm & \texttt{\textbackslash ellmp} & \ellmp & \texttt{\textbackslash ellell} & \ellell \\
\texttt{\textbackslash neu} & \neu & \texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue \\
\texttt{\textbackslash neueb} & \neueb & \texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb \\
\texttt{\textbackslash neut} & \neut & \texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul \\
\texttt{\textbackslash neulb} & \neulb &  \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim & \texttt{\textbackslash pipm} & \pipm \\
\texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson & \texttt{\textbackslash rhoz} & \rhoz \\
\texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom & \texttt{\textbackslash rhopm} & \rhopm \\
\texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon & \texttt{\textbackslash Kbar} & \Kbar \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash Vzero} & \Vzero & \texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz \\
\texttt{\textbackslash Kstarzb} & \Kstarzb & \texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb \\
\texttt{\textbackslash Kstarp} & \Kstarp & \texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm \\
\texttt{\textbackslash Kstarmp} & \Kstarmp & \texttt{\textbackslash KorKbarz} & \KorKbarz & \texttt{\textbackslash etaz} & \etaz \\
\texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz & \texttt{\textbackslash omegaz} & \omegaz \\
\end{tabular*}

\subsubsection{Charmed mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Dbar} & \Dbar & \texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db \\
\texttt{\textbackslash DorDbar} & \DorDbar & \texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb \\
\texttt{\textbackslash Dp} & \Dp & \texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm \\
\texttt{\textbackslash Dmp} & \Dmp & \texttt{\textbackslash DpDm} & \DpDm & \texttt{\textbackslash Dstar} & \Dstar \\
\texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz & \texttt{\textbackslash Dstarzb} & \Dstarzb \\
\texttt{\textbackslash theDstarz} & \theDstarz & \texttt{\textbackslash theDstarzb} & \theDstarzb & \texttt{\textbackslash Dstarp} & \Dstarp \\
\texttt{\textbackslash Dstarm} & \Dstarm & \texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp \\
\texttt{\textbackslash theDstarp} & \theDstarp & \texttt{\textbackslash theDstarm} & \theDstarm & \texttt{\textbackslash theDstarpm} & \theDstarpm \\
\texttt{\textbackslash theDstarmp} & \theDstarmp & \texttt{\textbackslash Ds} & \Ds & \texttt{\textbackslash Dsp} & \Dsp \\
\texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm & \texttt{\textbackslash Dsmp} & \Dsmp \\
\texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp & \texttt{\textbackslash Dssm} & \Dssm \\
\texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp & \texttt{\textbackslash DporDsp} & \DporDsp \\
\texttt{\textbackslash DmorDsm} & \DmorDsm & \texttt{\textbackslash DpmorDspm} & \DpmorDspm &  \\
\end{tabular*}

\subsubsection{Beauty mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash BdorBdbar} & \BdorBdbar \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb & \texttt{\textbackslash BsorBsbar} & \BsorBsbar \\
\texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp & \texttt{\textbackslash Bcm} & \Bcm \\
\texttt{\textbackslash Bcpm} & \Bcpm & \texttt{\textbackslash Bds} & \Bds & \texttt{\textbackslash Bdsb} & \Bdsb \\
\texttt{\textbackslash BdorBs} & \BdorBs & \texttt{\textbackslash BdorBsbar} & \BdorBsbar &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash psires} & \psires & \texttt{\textbackslash chic} & \chic \\
\texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone & \texttt{\textbackslash chictwo} & \chictwo \\
\texttt{\textbackslash chicJ} & \chicJ & \texttt{\textbackslash Upsilonres} & \Upsilonres & \texttt{\textbackslash OneS} & \OneS \\
\texttt{\textbackslash TwoS} & \TwoS & \texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS \\
\texttt{\textbackslash FiveS} & \FiveS & \texttt{\textbackslash chib} & \chib & \texttt{\textbackslash chibzero} & \chibzero \\
\texttt{\textbackslash chibone} & \chibone & \texttt{\textbackslash chibtwo} & \chibtwo & \texttt{\textbackslash chibJ} & \chibJ \\
\texttt{\textbackslash theX} & \theX &  \\
\end{tabular*}

\subsubsection{Light Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Lz} & \Lz & \texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar \\
\texttt{\textbackslash Lambdares} & \Lambdares & \texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares \\
\texttt{\textbackslash Sigmaz} & \Sigmaz & \texttt{\textbackslash Sigmap} & \Sigmap & \texttt{\textbackslash Sigmam} & \Sigmam \\
\texttt{\textbackslash Sigmaresbar} & \Sigmaresbar & \texttt{\textbackslash Sigmabarz} & \Sigmabarz & \texttt{\textbackslash Sigmabarp} & \Sigmabarp \\
\texttt{\textbackslash Sigmabarm} & \Sigmabarm & \texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiz} & \Xiz \\
\texttt{\textbackslash Xim} & \Xim & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Xibarz} & \Xibarz \\
\texttt{\textbackslash Xibarp} & \Xibarp & \texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar \\
\texttt{\textbackslash Omegam} & \Omegam & \texttt{\textbackslash Omegabarp} & \Omegabarp &  \\
\end{tabular*}

\subsubsection{Charmed Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar & \texttt{\textbackslash Sigmac} & \Sigmac \\
\texttt{\textbackslash Sigmacp} & \Sigmacp & \texttt{\textbackslash Sigmacz} & \Sigmacz & \texttt{\textbackslash Sigmacpp} & \Sigmacpp \\
\texttt{\textbackslash Sigmacbar} & \Sigmacbar & \texttt{\textbackslash Sigmacbarp} & \Sigmacbarp & \texttt{\textbackslash Sigmacbarz} & \Sigmacbarz \\
\texttt{\textbackslash Sigmacbarm} & \Sigmacbarm & \texttt{\textbackslash Xic} & \Xic & \texttt{\textbackslash Xicz} & \Xicz \\
\texttt{\textbackslash Xicp} & \Xicp & \texttt{\textbackslash Xicbar} & \Xicbar & \texttt{\textbackslash Xicbarz} & \Xicbarz \\
\texttt{\textbackslash Xicbarm} & \Xicbarm & \texttt{\textbackslash Omegac} & \Omegac & \texttt{\textbackslash Omegacbar} & \Omegacbar \\
\texttt{\textbackslash Xicc} & \Xicc & \texttt{\textbackslash Xiccbar} & \Xiccbar & \texttt{\textbackslash Xiccp} & \Xiccp \\
\texttt{\textbackslash Xiccpp} & \Xiccpp & \texttt{\textbackslash Xiccbarm} & \Xiccbarm & \texttt{\textbackslash Xiccbarmm} & \Xiccbarmm \\
\texttt{\textbackslash Omegacc} & \Omegacc & \texttt{\textbackslash Omegaccbar} & \Omegaccbar & \texttt{\textbackslash Omegaccc} & \Omegaccc \\
\texttt{\textbackslash Omegacccbar} & \Omegacccbar &  \\
\end{tabular*}

\subsubsection{Beauty Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Lb} & \Lb & \texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Sigmab} & \Sigmab \\
\texttt{\textbackslash Sigmabp} & \Sigmabp & \texttt{\textbackslash Sigmabz} & \Sigmabz & \texttt{\textbackslash Sigmabm} & \Sigmabm \\
\texttt{\textbackslash Sigmabpm} & \Sigmabpm & \texttt{\textbackslash Sigmabbar} & \Sigmabbar & \texttt{\textbackslash Sigmabbarp} & \Sigmabbarp \\
\texttt{\textbackslash Sigmabbarz} & \Sigmabbarz & \texttt{\textbackslash Sigmabbarm} & \Sigmabbarm & \texttt{\textbackslash Sigmabbarpm} & \Sigmabbarpm \\
\texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz & \texttt{\textbackslash Xibm} & \Xibm \\
\texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz & \texttt{\textbackslash Xibbarp} & \Xibbarp \\
\texttt{\textbackslash Omegab} & \Omegab & \texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsubsection{New Naming Scheme for Hadrons}
Since 2024 a new naming scheme for exotic hadrons previously known as $X, Y, Z$ states has been adopted by PDG. Please refer to Table 8.2 in ``Naming scheme for Hadrons'' review of Ref.~\cite{PDG2024}.

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BR} & \BR & \texttt{\textbackslash BRvis} & \BRvis \\
\texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to &  \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, \boldmath \CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash T} & \T & \texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar \\
\texttt{\textbackslash Vud} & \Vud & \texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd \\
\texttt{\textbackslash Vus} & \Vus & \texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts \\
\texttt{\textbackslash Vub} & \Vub & \texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb \\
\texttt{\textbackslash Vuds} & \Vuds & \texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds \\
\texttt{\textbackslash Vuss} & \Vuss & \texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss \\
\texttt{\textbackslash Vubs} & \Vubs & \texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\texttt{\textbackslash Cpipi} & \Cpipi & \texttt{\textbackslash Spipi} & \Spipi & \texttt{\textbackslash CKK} & \CKK \\
\texttt{\textbackslash SKK} & \SKK & \texttt{\textbackslash ADGKK} & \ADGKK &  \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash Bsee} & \Bsee & \texttt{\textbackslash Bdee} & \Bdee \\
\texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk &  \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsubsection{Units (these macros add a small space in front)}
\subsubsection{Energy and momentum }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevgev} & \gevgev \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevc} & \gevc & \texttt{\textbackslash mevcc} & \mevcc \\
\texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcc} & \gevgevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\end{tabular*}

\subsubsection{Distance and area (these macros add a small space)}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst & \texttt{\textbackslash lumi} & \lumi \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqfd} & \chisqfd & \texttt{\textbackslash chisqvs} & \chisqvs \\
\texttt{\textbackslash chisqvtx} & \chisqvtx & \texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv \\
\texttt{\textbackslash gsim} & \gsim & \texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} \\
\texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} & \texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag \\
\texttt{\textbackslash PDF} & \PDF & \texttt{\textbackslash sPlot} & \sPlot & \texttt{\textbackslash sFit} & \sFit \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash sqsnn} & \sqsnn \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash ptsq} & \ptsq & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt & \texttt{\textbackslash dpp} & \dpp \\
\texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx &  \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash murad} & \murad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash lamarr} & \lamarr & \texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig \\
\texttt{\textbackslash moore} & \moore & \texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos \\
\texttt{\textbackslash powheg} & \powheg & \texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos \\
\texttt{\textbackslash roofit} & \roofit & \texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice \\
\texttt{\textbackslash tensorflow} & \tensorflow & \texttt{\textbackslash urania} & \urania &  \texttt{\textbackslash hepml} & \hepml  \\
 \texttt{\textbackslash starlight} & \starlight & \texttt{\textbackslash superchic} & \superchic & & \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn & \texttt{\textbackslash git} & \git & \texttt{\textbackslash latex} & \latex \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbit} & \kbit & \texttt{\textbackslash kbps} & \kbps & \texttt{\textbackslash kbytes} & \kbytes \\
\texttt{\textbackslash kbyps} & \kbyps & \texttt{\textbackslash mbit} & \mbit & \texttt{\textbackslash mbps} & \mbps \\
\texttt{\textbackslash mbytes} & \mbytes & \texttt{\textbackslash mbyps} & \mbyps & \texttt{\textbackslash gbit} & \gbit \\
\texttt{\textbackslash gbps} & \gbps & \texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbyps} & \gbyps \\
\texttt{\textbackslash tbit} & \tbit & \texttt{\textbackslash tbps} & \tbps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbyps} & \tbyps & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsubsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}

\subsubsection{Helpful to align numbers in tables}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash phz} & \phz &  \\
\end{tabular*}



==> LHCbInternal/supplementary_template.tex <==
\section{Inclusion of supplementary material}
\label{sec:Supplementary}

Three types of supplementary material should be distinguished:
\begin{itemize}
\item{A regular appendix: lengthy equations or long tables are sometimes
better put in an appendix in order not to interrupt the main flow of a paper.
Appendices will appear in the final paper, on arXiv
and on the CDS record and should be considered integral
part of a paper, and are thus to be reviewed like the rest of the paper.
An example of an LHCb paper with an appendix is Ref.~\cite{LHCb-PAPER-2013-070}.
}
\item{Supplementary material for CDS: plots or tables that 
would make the paper exceed the page limit or are
not appropriate to include in the paper itself,
but are desirable to be shown in public
should be added to the paper drafts in an appendix, and
removed from the paper before submitting to arXiv or the journal.
See Appendix~\ref{sec:Supplementary-App} for further instructions.
Examples are: comparison plots of the new result with older results,
plots that illustrate cross-checks.
An example of an LHCb paper with supplementary material for CDS 
is Ref.~\cite{LHCb-PAPER-2013-035}.
Supplementary material for CDS cannot be referenced in the paper.
Supplementary material should be included in the draft paper to be
reviewed by the collaboration.
}
\item{Supplementary material for the paper. This is usually called ``supplemental material'', which distinguishes it from supplementary material for CDS only. Most journals allow
to submit files along with the paper that will not be part of the
text of the article, but will be stored on the journal server.
Examples are plain text files with numerical data corresponding to the plots
in the paper. 
The supplemental material should be cited in the paper by including a reference
which should say ``See supplemental material at [link] for [give brief description of material].''
The journal will insert a specific link for [link]. The arXiv version will usually include the supplemental material as part of the paper and so should not contain the words ``at [link]''.
Supplemental material should be included in the draft paper to be
reviewed by the collaboration.
An example of an LHCb paper with supplemental material 
is Ref.~\cite{LHCb-PAPER-2015-029}
}
\end{itemize}



==> LHCbInternal/wordcount.tex <==
\ProvidesFile{wordcount.tex}[2000/09/27 v1.5 Michael Downes]
% Copyright 2000 Michael John Downes
% This file has no restrictions on its use, distribution, or sale.
%
% If you run LaTeX on wordcount.tex it will prompt you for the name of a
% document to be counted. For most people, however, it will be more
% convenient to run the shell script wordcount.sh, giving the document
% name as the first argument. The comments in wordcount.sh
% give further information about the usage and limitations of this tool.

% The fundamental idea is to mark each character and interword space
% with a unique tag that will show up in TeX "showbox" output. Then
% arrange to make the output routine trigger a TeX overfull vbox message
% for the page box so that everything gets reported in the TeX log.
% Then run grep -c (or an equivalent text search utility, e.g., perl) on
% the log file to count the occurrences.
%
% In showbox output, a character is typically represented by a line of
% the form
%
%   ...\T1/cmr/m/n/10 e
%
% where "\T1/cmr/m/n/10" is the font name. We arrange things so that all
% characters are typeset in a font named "\3.08632". Furthermore, for
% interword spaces, which are normally represented in the output as
% something like
%
%   ...\glue 3.33333 plus 1.66666 minus 1.11111
%
% we use \spaceskip to ensure that it always appears as
%
%   ...\glue(\spaceskip) 3.08633 plus 9.0
%
% Then to count characters (including word spaces) we can
% grep for lines matching "3.0863", while to count words we
% count the number of lines in the log that match "3.08633" but not
% "3.08632".
%
% For an accurate count in multi-line paragraphs we also need
% to set rightskip to the flag value, since interword spaces are
% discarded at line breaks; and on the presumption that hyphenated
% compounds like "steady-state" should be counted as two words, we set
% \exhyphenpenalty to a value that ensures a line break at *every*
% explicit hyphen---then we will get a rightskip glue node between the
% two parts. (How about em-dashes? you may ask. Answer: it works all
% right, try it and see.)

\ifx\relax\?\def\wcQUIET{TT}\else\def\wcQUIET{TF}\fi

% We want accented letters to be represented by a single font char, to
% the extent possible:
\RequirePackage[T1]{fontenc}
\makeatletter
\thickmuskip=5.55555mu plus5.55555mu minus 2.22222mu
\let\@@thickmuskip\thickmuskip \newmuskip\thickmuskip
\let\@@spaceskip\spaceskip \xspaceskip=0pt
\newskip\@charfontname
% Ensure that these cannot be overridden.
\let\spaceskip\@charfontname \let\xspaceskip\spaceskip
\def\FreezeSpaces{%
  \setbox\z@\hbox{\mathsurround=\z@ $\mkern\@@thickmuskip$}%
  \@@spaceskip=\wd\z@ plus 9pt\relax
  % Setting rightskip to a slightly different value means that
  % end-of-line spaces can be distinguished if desired. (By default,
  % they are not.) Using fil units means there won't be any hyphenation
  % except for explicit hyphens.
  \dimen@\@@spaceskip \advance\dimen@ 1sp\relax
  \rightskip\z@ plus\strip@pt\dimen@ fil\relax
  % Prevent any further changes to \rightskip.
  \let\rightskip\spaceskip
  \@charfontname=\wd\z@ \advance\@charfontname -1sp\relax
  % Cancel all non-1000 sfcodes, which might otherwise affect the value
  % of inter-sentence spaces and keep them from being counted as
  % interword spaces.
  \def\do{\sfcode\fam\@m \advance\fam\@ne
    \ifnum\fam>\@cclv\expandafter\@gobble\fi \do
  }%
  \fam\z@ \do
  \let\frenchspacing\relax \let\nonfrenchspacing\relax
}
\def\DashPatch{%
  \exhyphenpenalty=-\@M \let\exhyphenpenalty\count@
  \hyphenpenalty\@M \let\hyphenpenalty\count@
  % LaTeX bug? Default definitions for these don't have \exhyphenpenalty
  % built in. Change them to just print a hyphen so that the penalties
  % will work.
  \def\textemdash{-}\def\textendash{-}%
}
% Here we set the font to ptmr8t (a T1 encoded font for which most
% people are likely to have a tfm file) and then make it difficult for
% the font to be changed ever again. We use two names for the font,
% \ptmr and \3.08632, the former being easier to use when resetting math
% fonts. The name that is defined last when TeX processes a document is
% the one that will be used in the log file.
\def\FreezeFont{%
  \expandafter\font
    \csname\strip@pt\@charfontname\endcsname
    =ptmr8t \relax
  \ptmr
  \check@mathfonts \let\check@mathfonts\relax
  \def\do{%
    \textfont\fam=\ptmr\scriptfont\fam=\ptmr\scriptscriptfont\fam=\ptmr
    \advance\fam\@ne \ifnum\fam<\sixt@@n \else\expandafter\@gobble\fi
    \do
  }%
  \fam=0 \do
}
\font\ptmr=ptmr8t \relax
\fontdimen22\ptmr=1sp % to permit use as math font 2
\let\selectfont\relax
\let\fontshape\@gobble \let\fontseries\@gobble \let\fontfamily\@gobble 
\let\fontencoding\@gobble \let\fontsize\@gobbletwo
\let\linespread\@gobble 
\let\try@load@fontshape\relax
\@namedef{U/msa/m/n}{}% disable special test in AMS documentclasses
\def\define@newfont{\expandafter\let\font@name=\ptmr}
\let\@@hfuzz\hfuzz \let\@@vfuzz\vfuzz
\newdimen\hfuzz \let\vfuzz\hfuzz
\def\QuietBoxes{%
  \@@hfuzz\maxdimen \@@vfuzz\maxdimen
}
\AtBeginDocument{\FreezeSpaces \FreezeFont \DashPatch \QuietBoxes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Halign patches
\def\ialign{\everycr{}\tabskip\@@spaceskip\halign} % initialized \halign
\def\extracolsep#1{\tabskip\@@spaceskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nofiles \let\makeindex\@empty % work-around for a natbib problem
% Seize control of the output routine to avoid extra clutter of dvi
% files. Handling \AtBeginDVI would take some extra work--for now I
% won't bother.
\def\showpagebox{%
  \showboxbreadth\maxdimen\showboxdepth99
  % This is a devious way of getting the box contents into the log file
  % without actually using \showbox (which typically results in a
  % nonzero exit code from the TeX run).
  \@@vfuzz\z@
  \setbox\z@\vbox to\z@{\box\@outputbox}%
  \setbox\z@\box\voidb@x
  \global \@colht \textheight
  \stepcounter{page}%
  \let\firstmark\botmark
}
\AtBeginDocument{\def\@outputpage{\showpagebox}}
\if\wcQUIET\else
\begingroup \def\msg^^J#1]^^J{\endgroup\message{#1]^^J^^J}}
\endlinechar=`\^^J \catcode`\ =12 \msg

The 'wordcount' utility provides a way of estimating the number of
words in a LaTeX document.

[Warning: The counting method uses a large log file as an intermediate
step. If your disk space is extremely low the counting process
may end prematurely for lack of space.]

\fi

% \typein has extraneous blank lines and slightly idiosyncratic prompt.
\begingroup \endlinechar=-1
\message{File name [press RETURN to cancel]: }
\def\do{%
  \let\do\@makeother \dospecials
  \global\read-1 to\wcFileName
  \endgroup
}
\do

\ifx\@empty\wcFileName
  \typeout{No file name given; quitting.}\expandafter\@@end\fi

\expandafter\filename@parse\expandafter{\wcFileName}
\edef\jobname{\filename@base}

\if\wcQUIET
  \message{\wcFileName}
\else
\typeout{^^JTo get a count of characters, run^^J^^J \space
%
  grep -c '3[.]0863[23]' wordcount.log^^J^^J%
%
or equivalent when processing is finished.^^J%
}
\fi

\typeout{Processing \wcFileName...^^J}

\IfFileExists{\wcFileName}{\batchmode}{\nonstopmode}
\edef\@tempa{\noexpand\makeatother
  \noexpand\input{\wcFileName}\noexpand\stop
}
\@tempa


==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) LHCbInternal/$(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' LHCbInternal/main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && sh LHCbInternal/wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) LHCbInternal/$(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl && $(LATEX) LHCbInternal/$(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex)  $(wildcard */*.tex) $(wildcard */*.bib) $(wildcard */*.bst)
FIGSOURCES = $(wildcard Figures/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) LHCbInternal/$(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl LHCbInternal/$(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm -f LHCbInternal/$(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

